Array Program Transformation with Loo.py by Example: High-Order Finite Elements

To concisely and effectively demonstrate the capabilities of our program transformation system Loo.py, we examine a transformation path from two real-world Fortran subroutines as found in a weather model to a single high-performance computational kernel suitable for execution on modern GPU hardware. Along the transformation path, we encounter kernel fusion, vectorization, prefetch- ing, parallelization, and algorithmic changes achieved by mechanized conversion between imperative and functional/substitution- based code, among a number more. We conclude with performance results that demonstrate the effects and support the effectiveness of the applied transformations.

==> tcbbreakable.code.tex <==
%% The LaTeX package tcolorbox - version 3.90 (2016/02/29)
%% tcbbreakable.code.tex: Code for breakable colorboxes
%%
%% -------------------------------------------------------------------------------------------
%% Copyright (c) 2006-2016 by Prof. Dr. Dr. Thomas F. Sturm <thomas dot sturm at unibw dot de>
%% -------------------------------------------------------------------------------------------
%%
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either version 1.3
%% of this license or (at your option) any later version.
%% The latest version of this license is in
%%   http://www.latex-project.org/lppl.txt
%% and version 1.3 or later is part of all distributions of LaTeX
%% version 2005/12/01 or later.
%%
%% This work has the LPPL maintenance status `author-maintained'.
%%
%% This work consists of all files listed in README
%%
\tcb@set@library@version{3.90}

\let\tcb@parboxrestore@true=\tcb@parboxrestore
\let\tcb@parboxrestore@false\tcb@parbox@false@settings

% total height for boxes smaller than 0.4375\maxdimen and 0.4375\maxdimen else (ca 2.5m)
\def\tcb@defToTotalHeightBreakable#1#2{%
  \ifnum\ht#2<0 %
    \edef#1{7168pt}%
  \else\ifnum\ht#2<469762048 %
    \tcbdimto#1{\ht#2+\dp#2}%
  \else%
    \edef#1{7168pt}%
  \fi\fi%
}

\newbox\tcb@testbox

% for oversized boxes height is detected as \textheight or larger
\def\tcb@defToTotalHeightUnlimited#1#2{%
  \tcb@defToTotalHeightBreakable#1#2%
  \ifdim\dimexpr#1<\textheight\relax%
    \edef\tcb@thevfuzz{\the\vfuzz}%
    \edef\tcb@thevbadness{\the\vbadness}%
    \vfuzz=\maxdimen\vbadness=10000%
    \splittopskip=0pt%
    \splitmaxdepth=0pt%
    \savingvdiscards=1%
    \setbox\tcb@testbox=\vsplit#2 to \textheight%
    \vbadness=\tcb@thevbadness\vfuzz=\tcb@thevfuzz%
    \ifdim\wd#2=0pt\relax%
      \tcb@swap{#2}{\tcb@testbox}%
      \tcbdimto#1{\ht#2+\dp#2}%
    \else%
      \setbox#2=\vbox{%
        \unvbox\tcb@testbox%
        \splitdiscards%
        \unvbox#2}%
      \edef#1{7168pt}%
    \fi%
    \savingvdiscards=0%
  \fi%
}


\def\tcb@vbox#1#2{%
  \edef\reserved@a{%
    \endgroup%
    \setbox#1\vbox{\hsize=#2%
      \begingroup\aftergroup}%
      \def\noexpand\@currenvir{\@currenvir}%
      \def\noexpand\@currenvline{\on@line}}%
  \reserved@a%
  \@endpefalse%
  \color@begingroup%
  \textwidth\hsize%
  \columnwidth\hsize%
  \csname tcb@parboxrestore@\kvtcb@parbox\endcsname%
  \def\@mpfn{mpfootnote}%
  \def\thempfn{\thempfootnote}%
  \c@mpfootnote\z@%
  \let\@footnotetext\@mpfootnotetext%
  \let\@listdepth\@mplistdepth \@mplistdepth\z@%
  \@setminipage\tcb@hyph@fix%
  \let\tcb@drawcolorbox\tcb@drawcolorbox@standalone%
  \let\FN@pp@footnote\@empty% disable perpage mode of 'footmisc' package
  \ignorespaces%
}

\def\endtcb@vbox{%
  \par%
  \unskip%
  \ifvoid\@mpfootins\else%
    \vskip\skip\@mpfootins%
    \normalcolor%
    \footnoterule%
    \unvbox\@mpfootins%
  \fi%
  \@minipagefalse%
  \color@endgroup}

% remaining height
\def\tcb@comp@h@page{%
  \tcb@breakat@next%
  \ifdim\tcb@breakat@dim>0pt\relax%
    \tcbdimto\tcb@h@page{\tcb@breakat@dim-\kvtcb@shrinkbreakgoal}%
  \else%
    \ifx\kvtcb@float\@empty%
      \iftcb@multicol%
        \tcbdimto\tcb@h@page{\textheight-\kvtcb@shrinkbreakgoal}%
      \else%
        \ifdim\pagegoal=16383.99998pt
          \tcbdimto\tcb@h@page{\vsize-\kvtcb@shrinkbreakgoal}% detects floating objects
        \else%
          \tcb@comp@compress%
          \tcbdimto\tcb@h@page{\pagegoal-\pagetotal+\tcb@compress@height-\kvtcb@shrinkbreakgoal}%
        \fi%
      \fi%
    \else%
      \tcbdimto\tcb@h@page{\textheight-\kvtcb@shrinkbreakgoal}%
    \fi%
  \fi%
}

\def\tcb@comp@h@total@standalone{%
  \tcbdimto\tcb@h@padding{\kvtcb@bbtop@stand+\kvtcb@bbbottom@stand+\kvtcb@top@rule@stand+\kvtcb@bottom@rule@stand+\kvtcb@boxsep*2+\kvtcb@top+\kvtcb@bottom}%
  \tcbdimto\tcb@h@total{\tcb@h@padding+\tcb@h@padtitle+\tcb@h@upper+\tcb@h@segment+\tcb@h@lower}%
}


\newif\iftcb@final@box

\def\tcb@check@for@final@box{%
  \ifdim\tcb@h@total>\tcb@h@page\relax%
    \iftcb@multicol%
      \tcb@final@boxfalse%
    \else%
      \ifdim\tcb@h@total>\dimexpr\tcb@h@page+\kvtcb@enlargepage@flex\relax%
        \tcb@final@boxfalse%
      \else%
        \tcbdimto\tcb@temp{\tcb@h@total-\tcb@h@page}%
        \enlargethispage*{\tcb@temp}%
        \tcbdimto\tcb@h@page{\tcb@h@page+\tcb@temp}%
        \tcb@final@boxtrue%
      \fi%
    \fi%
  \else%
    \tcb@final@boxtrue%
  \fi%
}

\def\tcb@following@title{%
  \ifx\kvtcb@followingtitle\@empty%
    \tcb@hasTitlefalse%
    \let\tcb@h@title=\tcb@zpt%
    \let\tcb@h@padtitle=\tcb@zpt%
  \else%
    \tcb@hasTitletrue%
    \tcbdimto\tcb@w@title{\tcb@innerwidth-\kvtcb@boxsep*2-\kvtcb@lefttitle-\kvtcb@righttitle}%
    \begin{tcb@savebox}{\tcb@titlebox}{\tcb@w@title}\color{tcbcol@title}\kvtcb@fonttitle\kvtcb@followingtitle\end{tcb@savebox}%
    \tcbdimto\tcb@h@title{\ht\tcb@titlebox+\dp\tcb@titlebox}%
    \tcbdimto\tcb@h@padtitle{\kvtcb@title@rule+\kvtcb@boxsep*2+\kvtcb@toptitle+\kvtcb@bottomtitle+\tcb@h@title}%
  \fi%
}

\newbox\tcb@totalupperbox
\newbox\tcb@totallowerbox
\newif\iftcb@break@allowed

\def\tcb@enlbreak@next@final{%
  \ifdim\dimexpr\tcb@enlbreak@dim=0pt\relax
  \else%
    \iftcb@multicol\else\enlargethispage{\tcb@enlbreak@dim}\fi%
  \fi%
}

\def\tcb@enlbreak@next@scan#1/#2@{%
  \def\temp@a{#2}%
  \tcbdimto\tcb@enlbreak@dim{#1}%
  \ifx\temp@a\@empty%
    \let\tcb@enlbreak@next=\tcb@enlbreak@next@final%
  \else%
     \edef\tcb@enlbreak@seq{\temp@a @}%
  \fi%
  \tcb@enlbreak@next@final%
}

\def\tcb@enlbreak@next@step{%
  \edef\tcb@temp{\noexpand\tcb@enlbreak@next@scan\tcb@enlbreak@seq}%
  \tcb@temp%
}

\def\tcb@enlbreak@init{%
  \edef\tcb@enlbreak@seq{\kvtcb@enlargepage/@}%
  \let\tcb@enlbreak@next=\tcb@enlbreak@next@step%
  \tcb@enlbreak@next%
}


\def\tcb@breakat@next@scan#1/#2@{%
  \def\temp@a{#2}%
  \tcbdimto\tcb@breakat@dim{#1}%
  \ifx\temp@a\@empty%
    \let\tcb@breakat@next=\@empty%
  \else%
     \edef\tcb@breakat@seq{\temp@a @}%
  \fi%
}

\def\tcb@breakat@next@step{%
  \edef\tcb@temp{\noexpand\tcb@breakat@next@scan\tcb@breakat@seq}%
  \tcb@temp%
}

\def\tcb@breakat@init{%
  \edef\tcb@breakat@seq{\kvtcb@breakatdim/@}%
  \let\tcb@breakat@next=\tcb@breakat@next@step%
}


\newif\iftcb@multicol
\newif\iftcb@vfillbeforefirst

\def\tcb@do@nobreak@warning{%
  \iftcb@ignorenobreak%
    \tcb@warning{Using nobreak failed. You should set `ignore nobreak=false' to avoid this}%
  \else%
    \tcb@warning{Using nobreak failed. Try to enlarge `lines before break' or set page breaks manually}%
  \fi%
}

\def\tcb@handle@nobreak{%
  \tcb@enlbreak@init%
  \tcb@breakat@init%
  \tcb@comp@h@page%
  \tcbdimto\tcb@h@page{\tcb@h@page-1.5\baselineskip-\parskip-\lineskip}% security surcharge
  \tcb@comp@h@total@standalone%
  \tcb@check@for@final@box%
  \iftcb@final@box%
  \else%
    \ifdim\dimexpr\tcb@h@page-\tcb@h@padding-\tcb@h@padtitle<\kvtcb@breakminlines\baselineskip\relax%
      \tcbdimto\tcb@h@page{\tcb@h@page+3.5\baselineskip+\parskip+\lineskip}%
      \vspace{\tcb@h@page}%
      {\parskip\z@\nointerlineskip\noindent}%
      \vspace{-\tcb@h@page}%
      \par%
    \fi%
  \fi%
}

\def\tcb@prepare@break@operation{%
  \setcounter{tcbbreakpart}{0}%
  \let\tcb@nobreak@warning\@empty%
  \@ifundefined{columnbreak}{\tcb@multicolfalse}{%
    \ifnum\doublecol@number>\z@ %
      \tcb@multicoltrue%
    \else%
      \tcb@multicolfalse%
    \fi}%
  \ifx\kvtcb@float\@empty%
    \iftcb@nobreak{%
      \let\tcb@nobreak@warning\tcb@do@nobreak@warning%
      \iftcb@ignorenobreak%
        \kvtcb@beforebox%
      \else%
        \tcb@handle@nobreak%
      \fi%
    }{\kvtcb@beforebox}%
    \def\kvtcb@beforebox{\parskip\z@\nointerlineskip\noindent}%
    \noindent% applies parskip
    \vskip\lineskip{\parskip\z@\par\vskip\z@}\bgroup\@nobreakfalse\addpenalty\z@\egroup% force update vertical list
    \tcb@break@allowedtrue%
    \tcb@enlbreak@init%
  \else%
    \tcb@break@allowedfalse%
  \fi%
}

\def\tcb@height@fill@unbroken#1{%
  \ifnum\c@tcblayer<2\relax%
    \tcb@ignorenobreaktrue%
    \tcb@prepare@break@operation%
    \tcb@breakat@init%
    \tcbset{compress page=#1}%
    \tcb@comp@h@page%
    \tcbset{height=\tcb@h@page-\kvtcb@bbtop@stand-\kvtcb@bbbottom@stand}%
  \fi%
}

\def\tcb@height@fill@unbroken@normal{\tcb@height@fill@unbroken{none}}
\def\tcb@height@fill@unbroken@compressed{\tcb@height@fill@unbroken{all}}

\def\tcb@use@after@lastbox{\bgroup\tcb@after@lastbox\egroup}

\def\tcb@drawcolorbox@breakable{%
  \tcb@prepare@break@operation%
  \global\let\tcb@after@lastbox=\kvtcb@afterbox%
  \let\kvtcb@afterbox=\@empty%
  \begingroup%
    \parskip\z@%
    \parindent\z@%
    \lineskip\z@%
    \topskip\z@%
    \tcb@split@start%
  \endgroup%
  \color{.}% hack for some special cases
  \ifx\kvtcb@float\@empty%
    \aftergroup\tcb@use@after@lastbox%
  \fi%
}

\def\tcb@split@pagebreak{%
  \tcb@undo@before%
  \iftcb@multicol\columnbreak\else\pagebreak\fi%
  \tcb@nobreak@warning%
  \tcb@enlbreak@init\tcb@break@allowedfalse%
}

\def\tcb@split@start{%
  \tcb@breakat@init%
  \tcb@comp@h@page%
  % height calculation
  \tcb@comp@h@total@standalone%
  %
  \let\tcb@split@next=\relax%
  \tcb@check@for@final@box%
  \iftcb@final@box%
    \tcb@drawcolorbox@standalone%
  \else%
    \iftcb@break@allowed%
      \ifdim\dimexpr\tcb@h@page-\tcb@h@padding-\tcb@h@padtitle<\kvtcb@breakminlines\baselineskip\relax%
        \tcb@split@pagebreak%
        \tcb@comp@h@page%
        \tcb@check@for@final@box%
        \iftcb@final@box%
          \tcb@drawcolorbox@standalone%
        \else%
          \let\tcb@split@next=\tcb@split@first%
        \fi%
      \else%
        \let\tcb@split@next=\tcb@split@first%
      \fi%
    \else%
      \let\tcb@split@next=\tcb@split@first%
    \fi%
  \fi%
  \tcb@split@next%
}


\def\tcb@setbox#1#2#3{%
  \setbox#1=\vbox{\unvbox#3}%
  \ifdim\dimexpr\ht#1+\dp#1>#2\relax%
    %\tcb@warning{Splitted box part too large by \the\dimexpr\ht#1+\dp#1-#2\relax}% switched off (99% useless/annoying)
    \setbox#1=\vbox to\the\dimexpr#2-\dp#1\relax{\unvbox#1}%
  \fi%
}


\def\tcb@setbox@upper#1#2{%
  \tcb@setbox\tcb@upperbox{#1}{#2}%
  \tcbdimto\tcb@h@upper{\ht\tcb@upperbox+\dp\tcb@upperbox}%
}


\def\tcb@split@upper@box@and@assemble{%
  \vfuzz=\maxdimen\vbadness=10000\savingvdiscards=1%
  \setbox\tcb@upperbox=\vsplit\tcb@totalupperbox to\tcb@split@dim%
  \edef\tcb@upper@box@badness{\the\badness}%
  \ifnum\tcb@upper@box@badness=1000000\relax%
    \setbox\tcb@totalupperbox=\vbox{%
      \unvbox\tcb@upperbox%
      \splitdiscards%
      \unvbox\tcb@totalupperbox}%
  \else%
    \tcb@setbox@upper{\tcb@split@dim}{\tcb@upperbox}%
  \fi%
  \vbadness=\tcb@thevbadness\vfuzz=\tcb@thevfuzz\savingvdiscards=0%
}


\def\tcb@split@upper@box{%
  \vfuzz=\maxdimen\vbadness=10000%
  \setbox\tcb@upperbox=\vsplit\tcb@totalupperbox to\tcb@split@dim%
  \edef\tcb@upper@box@badness{\the\badness}%
  \ifnum\tcb@upper@box@badness=1000000\relax%
    \tcb@warning{The upper box part has become overfull}%
  \fi%
  \tcb@setbox@upper{\tcb@split@dim}{\tcb@upperbox}%
  \vbadness=\tcb@thevbadness\vfuzz=\tcb@thevfuzz%
}


\def\tcb@setbox@lower#1#2{%
  \tcb@setbox\tcb@lowerbox{#1}{#2}%
  \tcbdimto\tcb@h@lower{\ht\tcb@lowerbox+\dp\tcb@lowerbox}%
}

\def\tcb@split@lower@box@and@assemble{%
  \vfuzz=\maxdimen\vbadness=10000\savingvdiscards=1%
  \setbox\tcb@lowerbox=\vsplit\tcb@totallowerbox to\tcb@split@dim%
  \edef\tcb@lower@box@badness{\the\badness}%
  \ifnum\tcb@lower@box@badness=1000000\relax%
    \setbox\tcb@totallowerbox=\vbox{%
      \unvbox\tcb@lowerbox%
      \splitdiscards%
      \unvbox\tcb@totallowerbox}%
  \else%
    \tcb@setbox@lower{\tcb@split@dim}{\tcb@lowerbox}%
  \fi%
  \vbadness=\tcb@thevbadness\vfuzz=\tcb@thevfuzz\savingvdiscards=0%
}


\def\tcb@split@lower@box{%
  \vfuzz=\maxdimen\vbadness=10000%
  \setbox\tcb@lowerbox=\vsplit\tcb@totallowerbox to\tcb@split@dim%
  \edef\tcb@lower@box@badness{\the\badness}%
  \ifnum\tcb@lower@box@badness=1000000\relax%
    \tcb@warning{The lower box part has become overfull}%
  \fi%
  \tcb@setbox@lower{\tcb@split@dim}{\tcb@lowerbox}%
  \vbadness=\tcb@thevbadness\vfuzz=\tcb@thevfuzz%
}


\def\tcb@split@setstate@first{%
  \edef\tcb@split@state{first}%
  \let\kvtcb@top@rule=\kvtcb@top@rule@stand%
  \let\kvtcb@bottom@rule=\kvtcb@bottom@rule@break%
  \let\kvtcb@bbtop=\kvtcb@bbtop@stand%
  \let\kvtcb@bbbottom=\kvtcb@bbbottom@break%
  \let\tcb@break@topsep=\tcb@zpt%
  \let\tcb@break@bottomsep=\kvtcb@bottomsep%
}

\def\tcb@split@setstate@middle{%
  \edef\tcb@split@state{middle}%
  \let\kvtcb@top@rule=\kvtcb@top@rule@break%
  \let\kvtcb@bottom@rule=\kvtcb@bottom@rule@break%
  \let\kvtcb@bbtop=\kvtcb@bbtop@break%
  \let\kvtcb@bbbottom=\kvtcb@bbbottom@break%
  \let\tcb@break@topsep=\kvtcb@topsep%
  \let\tcb@break@bottomsep=\kvtcb@bottomsep%
}

\def\tcb@split@setstate@last{%
  \edef\tcb@split@state{last}%
  \let\kvtcb@top@rule=\kvtcb@top@rule@break%
  \let\kvtcb@bottom@rule=\kvtcb@bottom@rule@stand%
  \let\kvtcb@bbtop=\kvtcb@bbtop@break%
  \let\kvtcb@bbbottom=\kvtcb@bbbottom@stand%
  \let\tcb@break@topsep=\kvtcb@topsep%
  \let\tcb@break@bottomsep=\tcb@zpt%
}


\def\tcb@split@force@standalone{%
  \tcb@comp@h@total@standalone%
  \ifdim\tcb@h@total>\tcb@h@page\relax%
    \tcbdimto\kvtcb@bbbottom@stand{\kvtcb@bbbottom@stand+\tcb@h@page-\tcb@h@total}%
  \fi%
}


\def\tcb@split@break@to@start{%
  \tcb@swap{\tcb@totalupperbox}{\tcb@upperbox}%
  \tcb@swap{\tcb@totallowerbox}{\tcb@lowerbox}%
  \tcbdimto\tcb@h@upper{\ht\tcb@upperbox+\dp\tcb@upperbox}%
  \tcbdimto\tcb@h@lower{\ht\tcb@lowerbox+\dp\tcb@lowerbox}%
  \tcb@split@pagebreak%
  \let\tcb@split@next=\tcb@split@start%
}

\def\tcb@split@first{%
  \setcounter{tcbbreakpart}{1}%
  \ifx\kvtcb@float\@empty%
    \iftcb@vfillbeforefirst%
      \let\tcb@before@first=\vfill%
    \else%
    \let\tcb@before@first=\@empty%
    \fi%
    \let\tcb@before@middle=\@empty%
    \let\tcb@before@last=\@empty%
    \iftcb@multicol%
      \long\def\tcb@after@first{\par}% using \columnbreak here kills multicols' algortihm sometimes
      \long\def\tcb@after@middle{\par\vfill}%
    \else%
      \long\def\tcb@after@first{\par\pagebreak\tcb@enlbreak@next}%
      \long\def\tcb@after@middle{\par\vfill\eject\tcb@enlbreak@next}%
    \fi%
    \let\tcb@after@last=\par%
  \else%
    \edef\tcb@before@first{\noexpand\tcb@float@env@begin{tcbfloat}[\kvtcb@float]\noexpand\kvtcb@everyfloat}%
    \let\tcb@before@middle=\tcb@before@first%
    \let\tcb@before@last=\tcb@before@first%
    \let\tcb@after@first=\tcb@float@env@end%
    \let\tcb@after@middle=\tcb@float@env@end%
    \let\tcb@after@last=\tcb@float@env@end%
  \fi%
  %
  \edef\kvtcb@skin@@first{\kvtcb@skin@first}%
  \edef\kvtcb@skin@@middle{\kvtcb@skin@middle}%
  \edef\kvtcb@skin@@last{\kvtcb@skin@last}%
  %
  \let\tcb@h@breaksep@first=\kvtcb@bottomsep%
  \tcbdimto\tcb@h@breaksep@middle{\kvtcb@bottomsep+\kvtcb@topsep}%
  \let\tcb@h@breaksep@last=\kvtcb@topsep%
  \tcbdimto\tcb@h@padding@first{\kvtcb@bbtop@stand+\kvtcb@bbbottom@break+\kvtcb@top@rule@stand+\kvtcb@bottom@rule@break+\tcb@h@breaksep@first+\kvtcb@boxsep*2+\kvtcb@top+\kvtcb@bottom}%
  \tcbdimto\tcb@h@padding@middle{\kvtcb@bbtop@break+\kvtcb@bbbottom@break+\kvtcb@top@rule@break+\kvtcb@bottom@rule@break+\tcb@h@breaksep@middle+\kvtcb@boxsep*2+\kvtcb@top+\kvtcb@bottom}%
  \tcbdimto\tcb@h@padding@last{\kvtcb@bbtop@break+\kvtcb@bbbottom@stand+\kvtcb@top@rule@break+\kvtcb@bottom@rule@stand+\tcb@h@breaksep@last+\kvtcb@boxsep*2+\kvtcb@top+\kvtcb@bottom}%
  %
  \tcb@split@setstate@first%
  %
  \splittopskip=0pt%
  \splitmaxdepth=0pt%
  \edef\tcb@thevfuzz{\the\vfuzz}%
  \edef\tcb@thevbadness{\the\vbadness}%
  %
  \tcb@swap{\tcb@totalupperbox}{\tcb@upperbox}%
  \tcb@swap{\tcb@totallowerbox}{\tcb@lowerbox}%
  %
  \let\tcb@split@next=\relax%
  \tcbdimto\tcb@split@dim{\tcb@h@page-\tcb@h@padding@first-\tcb@h@padtitle}%
  \ifdim\tcb@split@dim<\tcb@h@upper\relax%
    %
    %
    \iftcb@break@allowed%
      \tcb@split@upper@box@and@assemble%
      \ifnum\tcb@upper@box@badness=1000000\relax%
        \tcb@split@break@to@start%
      \else%
        \ifdim\wd\tcb@totalupperbox=0pt\relax%
          \iftcb@lowerspace%
            \tcb@sdraw@U%
            \let\tcb@split@next=\tcb@split@SL%
          \else%
            \tcb@split@force@standalone%
            \tcb@drawcolorbox@standalone%
          \fi%
        \else%
          \ifdim\dimexpr\tcb@h@upper=0pt\relax%
            \tcb@split@break@to@start%
          \else%
            \tcb@sdraw@U%
            \let\tcb@split@next=\tcb@split@USL%
          \fi%
        \fi%
      \fi%
    \else%
      \tcb@split@upper@box%
      \ifdim\wd\tcb@totalupperbox=0pt\relax%
        \iftcb@lowerspace%
          \tcb@sdraw@U%
          \let\tcb@split@next=\tcb@split@SL%
        \else%
          \tcb@split@force@standalone%
          \tcb@drawcolorbox@standalone%
        \fi%
      \else%
        \tcb@sdraw@U%
        \let\tcb@split@next=\tcb@split@USL%
      \fi%
    \fi%
  \else%
    \tcb@swap{\tcb@totalupperbox}{\tcb@upperbox}%
    \iftcb@lowerspace%
      \tcbdimto\tcb@split@dim{\tcb@split@dim-\tcb@h@upper-\tcb@h@segment}%
      \ifdim\tcb@split@dim<\kvtcb@breakminlines\baselineskip\relax%
        \tcb@sdraw@U%
        \let\tcb@split@next=\tcb@split@SL%
      \else
        \tcb@split@lower@box@and@assemble%
        \ifnum\tcb@lower@box@badness=1000000\relax%
          \tcb@sdraw@U%
          \let\tcb@split@next=\tcb@split@SL%
        \else%
          \ifdim\wd\tcb@totallowerbox=0pt\relax%
            \tcb@split@force@standalone%
            \tcb@drawcolorbox@standalone%
          \else%
            \tcb@sdraw@USL%
            \let\tcb@split@next=\tcb@split@L%
          \fi%
        \fi%
      \fi%
    \else%
      \tcb@split@force@standalone%
      \tcb@drawcolorbox@standalone%
    \fi%
  \fi%
  \tcb@split@next%
}


\def\tcb@split@force@last{%
  \tcb@split@setstate@last%
  \ifdim\tcb@h@total>\tcb@h@page%
    \tcbdimto\kvtcb@bbbottom{\kvtcb@bbbottom+\tcb@h@page-\tcb@h@total}%
  \fi%
}

\def\tcb@nextbreakpart{%
  \stepcounter{tcbbreakpart}%
  \tcb@count@boxes%
  \iftcb@checkpage%
    \tcb@phantom@savepage%
    \tcb@hasPhantomtrue%
    \sbox\tcb@phantombox{\kvtcb@phantom}%
    \let\kvtcb@phantom\@empty%
  \fi%
  \tcb@following@title%
}


\def\tcb@split@USL{%
  \tcb@nextbreakpart%
  \tcb@comp@h@page%
  \tcb@defToTotalHeight\tcb@h@upper{\tcb@totalupperbox}%
  \tcbdimto\tcb@h@total{\tcb@h@padding@last+\tcb@h@padtitle+\tcb@h@upper+\tcb@h@segment+\tcb@h@lower}%
  %
  \let\tcb@split@next=\relax%
  \tcb@check@for@final@box%
  \iftcb@final@box%
    \tcb@split@setstate@last%
    \tcb@setbox@upper{\tcb@h@upper}{\tcb@totalupperbox}%
    \iftcb@lowerspace%
      \tcb@setbox@lower{\tcb@h@lower}{\tcb@totallowerbox}%
      \tcb@sdraw@USL%
    \else
      \tcb@sdraw@U%
    \fi%
  \else
    \tcb@split@setstate@middle%
    \tcbdimto\tcb@split@dim{\tcb@h@page-\tcb@h@padding@middle-\tcb@h@padtitle}%
    \ifdim\tcb@split@dim<\tcb@h@upper\relax%
      \tcb@split@upper@box%
      \ifdim\wd\tcb@totalupperbox=0pt\relax%
        \iftcb@lowerspace%
          \tcb@sdraw@U%
          \let\tcb@split@next=\tcb@split@SL%
        \else%
          \tcb@split@force@last%
          \tcb@sdraw@U%
        \fi%
      \else%
        \tcb@sdraw@U%
        \let\tcb@split@next=\tcb@split@USL%
      \fi%
    \else%
      \tcb@setbox@upper{\tcb@h@upper}{\tcb@totalupperbox}%
      \iftcb@lowerspace%
        \tcbdimto\tcb@split@dim{\tcb@split@dim-\tcb@h@upper-\tcb@h@segment}
        \ifdim\tcb@split@dim<\kvtcb@breakminlines\baselineskip\relax%
          \tcb@sdraw@U%
          \let\tcb@split@next=\tcb@split@SL%
        \else
          \tcb@split@lower@box@and@assemble%
          \ifnum\tcb@lower@box@badness=1000000\relax%
            \tcb@sdraw@U%
            \let\tcb@split@next=\tcb@split@SL%
          \else%
            \ifdim\wd\tcb@totallowerbox=0pt\relax%
              \tcb@split@force@last%
              \tcb@sdraw@USL%
            \else%
              \tcb@sdraw@USL%
              \let\tcb@split@next=\tcb@split@L%
            \fi%
          \fi%
        \fi%
      \else%
        \tcb@split@force@last%
        \tcb@sdraw@U%
      \fi%
    \fi%
  \fi%
  \tcb@split@next%
}


\def\tcb@split@SL{%
  \tcb@nextbreakpart%
  \tcb@comp@h@page%
  \let\tcb@h@upper=\tcb@zpt%
  \tcb@defToTotalHeight\tcb@h@lower{\tcb@totallowerbox}%
  \tcbdimto\tcb@h@total{\tcb@h@padding@last-\kvtcb@top-\kvtcb@boxsep+\tcb@h@padtitle+\tcb@h@segment+\tcb@h@lower}%
  %
  \let\tcb@split@next=\relax%
  \tcb@check@for@final@box%
  \iftcb@final@box%
    \tcb@split@setstate@last%
    \tcb@setbox@lower{\tcb@h@lower}{\tcb@totallowerbox}%
    \tcb@sdraw@SL%
  \else
    \tcb@split@setstate@middle%
    \tcbdimto\tcb@split@dim{\tcb@h@page-\tcb@h@padding@middle+\kvtcb@top+\kvtcb@boxsep-\tcb@h@padtitle-\tcb@h@segment}%
    \tcb@split@lower@box%
    \ifdim\wd\tcb@totallowerbox=0pt\relax%
      \tcb@split@force@last%
      \tcb@sdraw@SL%
    \else
      \tcb@sdraw@SL%
      \let\tcb@split@next=\tcb@split@L%
    \fi%
  \fi%
  \tcb@split@next%
}


\def\tcb@split@L{%
  \tcb@nextbreakpart%
  \tcb@comp@h@page%
  \let\tcb@h@upper=\tcb@zpt%
  \tcb@defToTotalHeight\tcb@h@lower{\tcb@totallowerbox}%
  \tcbdimto\tcb@h@total{\tcb@h@padding@last+\tcb@h@padtitle+\tcb@h@lower}%
  %
  \let\tcb@split@next=\relax%
  \tcb@check@for@final@box%
  \iftcb@final@box%
    \tcb@split@setstate@last%
    \tcb@setbox@lower{\tcb@h@lower}{\tcb@totallowerbox}%
    \tcb@sdraw@L%
  \else
    \tcb@split@setstate@middle%
    \tcbdimto\tcb@split@dim{\tcb@h@page-\tcb@h@padding@middle-\tcb@h@padtitle}%
    \tcb@split@lower@box%
    \ifdim\wd\tcb@totallowerbox=0pt\relax%
      \tcb@split@force@last%
      \tcb@sdraw@L%
    \else
      \tcb@sdraw@L%
      \let\tcb@split@next=\tcb@split@L%
    \fi%
  \fi%
  \tcb@split@next%
}


\def\tcb@break@ch@fixed{%
  \ifdim\tcb@natheight<\tcb@h@page\relax%
    \tcbdimto\kvtcb@height@fixed{\tcb@h@page-\kvtcb@bbtop-\kvtcb@bbbottom}%
    \tcb@ch@fixed%
  \else%
    \tcb@ch@natural%
  \fi%
}


\def\tcb@sdraw@USL{%
  \begingroup%
  \tcbset{skin=\csname kvtcb@skin@@\tcb@split@state\endcsname}%
  \csuse{tcb@extras@\tcb@split@state}%
  \tcb@afteroptions@hook%
  \def\tcb@segment@state{1}%
  \tcbdimto\tcb@natheight{\tcb@h@padtitle+\kvtcb@top@rule+\kvtcb@bottom@rule+\kvtcb@boxsep*2+\kvtcb@top+\kvtcb@bottom+\tcb@h@upper+\tcb@h@segment+\tcb@h@lower+\csname tcb@h@breaksep@\tcb@split@state\endcsname}%
  \csname tcb@break@ch@\tcb@split@state\endcsname%
  \tcbdimto\tcb@innerheight{\tcb@height-\kvtcb@top@rule-\kvtcb@bottom@rule-\tcb@h@padtitle}%
  \tcbdimto\tcbtextheight{\tcb@innerheight-\kvtcb@boxsep*2-\kvtcb@top-\kvtcb@bottom}%
  \tcb@drawing@env@begin%
    \tcb@extensions@preframe%
     % draw frame and interior
    \tcb@adraw@frame%
    \tcb@adraw@interior%
    \iftcb@lowerseparated%
      \tcb@segmentation@code%
    \fi%
    \tcb@adraw@title%
    \tcb@extensions@postframe%
    % draw text boxes
    \tcb@tdraw@title%
    \tcb@tdraw@upper%
    \tcb@tdraw@lower%
    \tcb@extensions@final%
  \tcb@drawing@env@end%
  \endgroup%
}


\def\tcb@sdraw@U{%
  \begingroup%
  \tcbset{skin=\csname kvtcb@skin@@\tcb@split@state\endcsname}%
  \csuse{tcb@extras@\tcb@split@state}%
  \tcb@afteroptions@hook%
  \def\tcb@segment@state{0}%
  \tcbdimto\tcb@natheight{\tcb@h@padtitle+\kvtcb@top@rule+\kvtcb@bottom@rule+\kvtcb@boxsep*2+\kvtcb@top+\kvtcb@bottom+\tcb@h@upper+\csname tcb@h@breaksep@\tcb@split@state\endcsname}%
  \csname tcb@break@ch@\tcb@split@state\endcsname%
  \tcbdimto\tcb@innerheight{\tcb@height-\kvtcb@top@rule-\kvtcb@bottom@rule-\tcb@h@padtitle}%
  \tcbdimto\tcbtextheight{\tcb@innerheight-\kvtcb@boxsep*2-\kvtcb@top-\kvtcb@bottom}%
  \tcb@drawing@env@begin%
    \tcb@extensions@preframe%
    % draw frame and interior
    \tcb@adraw@frame%
    \tcb@adraw@interior%
    \tcb@adraw@title%
    \tcb@extensions@postframe%
    % draw text boxes
    \tcb@tdraw@title%
    \tcb@tdraw@upper%
    \tcb@extensions@final%
  \tcb@drawing@env@end%
  \endgroup%
}


\def\tcb@sdraw@SL{%
  \begingroup%
  \tcbset{skin=\csname kvtcb@skin@@\tcb@split@state\endcsname}%
  \csuse{tcb@extras@\tcb@split@state}%
  \tcb@afteroptions@hook%
  \def\tcb@segment@state{1}%
  \tcbdimto\tcb@natheight{\tcb@h@padtitle+\kvtcb@top@rule+\kvtcb@bottom@rule+\kvtcb@bottom+\kvtcb@boxsep+\tcb@h@segment+\tcb@h@lower+\csname tcb@h@breaksep@\tcb@split@state\endcsname}%
  \csname tcb@break@ch@\tcb@split@state\endcsname%
  \tcbdimto\tcb@innerheight{\tcb@height-\kvtcb@top@rule-\kvtcb@bottom@rule-\tcb@h@padtitle}%
  \tcbdimto\tcbtextheight{\tcb@innerheight-\kvtcb@boxsep*2-\kvtcb@top-\kvtcb@bottom}%
  \tcb@drawing@env@begin%
    \tcb@extensions@preframe%
    % draw frame and interior
    \tcb@adraw@frame%
    \tcb@adraw@interior%
    \iftcb@lowerseparated%
      \tcb@segmentation@code%
    \fi%
    \tcb@adraw@title%
    \tcb@extensions@postframe%
    % draw text boxes
    \tcb@tdraw@title%
    \tcb@tdraw@lower%
    \tcb@extensions@final%
  \tcb@drawing@env@end%
  \endgroup%
}


\def\tcb@sdraw@L{%
  \begingroup%
  \tcbset{skin=\csname kvtcb@skin@@\tcb@split@state\endcsname}%
  \csuse{tcb@extras@\tcb@split@state}%
  \tcb@afteroptions@hook%
  \def\tcb@segment@state{2}%
  \tcbdimto\tcb@natheight{\tcb@h@padtitle+\kvtcb@top@rule+\kvtcb@bottom@rule+\kvtcb@boxsep*2+\kvtcb@top+\kvtcb@bottom+\ht\tcb@lowerbox+\dp\tcb@lowerbox+\csname tcb@h@breaksep@\tcb@split@state\endcsname}%
  \csname tcb@break@ch@\tcb@split@state\endcsname%
  \tcbdimto\tcb@innerheight{\tcb@height-\kvtcb@top@rule-\kvtcb@bottom@rule-\tcb@h@padtitle}%
  \tcbdimto\tcbtextheight{\tcb@innerheight-\kvtcb@boxsep*2-\kvtcb@top-\kvtcb@bottom}%
  \tcb@drawing@env@begin%
    \tcb@extensions@preframe%
    % draw frame and interior
    \tcb@adraw@frame%
    \tcb@adraw@interior%
    \tcb@adraw@title%
    \tcb@extensions@postframe%
    % draw text boxes
    \tcb@tdraw@title%
    \tcb@tdraw@lower%
    \tcb@extensions@final%
  \tcb@drawing@env@end%
  \endgroup%
}



\tcbset{%
  breakable@true/.code={%
    \let\tcb@savebox=\tcb@vbox%
    \let\endtcb@savebox=\endtcb@vbox%
    \let\tcb@defToTotalHeight=\tcb@defToTotalHeightBreakable%
    \let\tcb@drawcolorbox=\tcb@drawcolorbox@breakable},
  breakable@unlimited/.code={%
    \let\tcb@savebox=\tcb@vbox%
    \let\endtcb@savebox=\endtcb@vbox%
    \let\tcb@defToTotalHeight=\tcb@defToTotalHeightUnlimited%
    \let\tcb@drawcolorbox=\tcb@drawcolorbox@breakable},
  breakable/.style={breakable@#1},
  breakable/.default=true,%
  unbreakable/.style={breakable=false},%
  enforce breakable/.code={%
    \let\tcb@savebox=\tcb@vbox%
    \let\endtcb@savebox=\endtcb@vbox%
    \let\tcb@defToTotalHeight=\tcb@defToTotalHeightBreakable%
    \let\tcb@drawcolorbox=\tcb@drawcolorbox@breakable},
  title after break/.store in=\kvtcb@followingtitle,%
  notitle after break/.style={title after break=},%
  adjusted title after break/.style={title after break={#1\vphantom{\kvtcb@adjusttext}}},%
  lines before break/.store in=\kvtcb@breakminlines,%
  shrink break goal/.store in=\kvtcb@shrinkbreakgoal,%
  toprule at break/.store in=\kvtcb@top@rule@break,
  bottomrule at break/.store in=\kvtcb@bottom@rule@break,
  topsep at break/.store in=\kvtcb@topsep,%
  bottomsep at break/.store in=\kvtcb@bottomsep,%
  pad before break/.code={\let\kvtcb@bottom@rule@break=\tcb@zpt%
    \tcbdimto\kvtcb@bottomsep{#1-\kvtcb@bottom-\kvtcb@boxsep}},%
  pad before break*/.style={pad before break={#1},%
    code={\tcbdimto\tcb@temp{\kvtcb@bottom@rule@stand-\kvtcb@bottomsep}%
      \ifdim\tcb@temp>0pt\relax%
        \tcbdimto\kvtcb@enlargepage@flex{\kvtcb@enlargepage@flex+\tcb@temp}\fi}},%
  pad after break/.code={\let\kvtcb@top@rule@break=\tcb@zpt%
    \tcbdimto\kvtcb@topsep{#1-\kvtcb@top-\kvtcb@boxsep}},%
  pad at break/.style={pad before break={#1},pad after break={#1}},%
  pad at break*/.style={pad before break*={#1},pad after break={#1}},%
  enlargepage/.store in=\kvtcb@enlargepage,%
  enlargepage flexible/.store in=\kvtcb@enlargepage@flex,%
  break at/.store in=\kvtcb@breakatdim,%
  height fixed for/.is choice,%
  height fixed for/none/.code={%
    \let\tcb@break@ch@first=\tcb@ch@natural%
    \let\tcb@break@ch@middle=\tcb@ch@natural%
    \let\tcb@break@ch@last=\tcb@ch@natural},%
  height fixed for/first/.code={%
    \let\tcb@break@ch@first=\tcb@break@ch@fixed%
    \let\tcb@break@ch@middle=\tcb@ch@natural%
    \let\tcb@break@ch@last=\tcb@ch@natural},%
  height fixed for/middle/.code={%
    \let\tcb@break@ch@first=\tcb@ch@natural%
    \let\tcb@break@ch@middle=\tcb@break@ch@fixed%
    \let\tcb@break@ch@last=\tcb@ch@natural},%
  height fixed for/last/.code={%
    \let\tcb@break@ch@first=\tcb@ch@natural%
    \let\tcb@break@ch@middle=\tcb@ch@natural%
    \let\tcb@break@ch@last=\tcb@break@ch@fixed},%
  height fixed for/first and middle/.code={%
    \let\tcb@break@ch@first=\tcb@break@ch@fixed%
    \let\tcb@break@ch@middle=\tcb@break@ch@fixed%
    \let\tcb@break@ch@last=\tcb@ch@natural},%
  height fixed for/middle and last/.code={%
    \let\tcb@break@ch@first=\tcb@ch@natural%
    \let\tcb@break@ch@middle=\tcb@break@ch@fixed%
    \let\tcb@break@ch@last=\tcb@break@ch@fixed},%
  height fixed for/all/.code={%
    \let\tcb@break@ch@first=\tcb@break@ch@fixed%
    \let\tcb@break@ch@middle=\tcb@break@ch@fixed%
    \let\tcb@break@ch@last=\tcb@break@ch@fixed},%
  vfill before first/.is if=tcb@vfillbeforefirst,%
  height fill/true/.code={\let\tcb@height@adjust\tcb@height@fill@unbroken@normal},%
  height fill/maximum/.code={\let\tcb@height@adjust\tcb@height@fill@unbroken@compressed},%
  height fill/.default=true,%
  compress page/.is choice,%
  compress page/all/.code={\def\tcb@comp@compress{\def\tcb@compress@height{\pageshrink-1sp}}},%
  compress page/none/.code={\def\tcb@comp@compress{\let\tcb@compress@height\tcb@zpt}},%
  compress page/baselineskip/.code={\def\tcb@comp@compress{%
    \ifdim\pageshrink>\baselineskip%
      \let\tcb@compress@height\baselineskip%
    \else%
      \def\tcb@compress@height{\pageshrink-1sp}%
    \fi}},%
  compress page/.default=all,%
  compress page=baselineskip,% global setting
  extras unbroken/.code={\appto\tcb@extras@unbroken{\tcbset{#1}}},%
  extras first/.code={\appto\tcb@extras@first{\tcbset{#1}}},%
  extras middle/.code={\appto\tcb@extras@middle{\tcbset{#1}}},%
  extras last/.code={\appto\tcb@extras@last{\tcbset{#1}}},%
  extras/.style={extras unbroken={#1},extras first={#1},extras middle={#1},extras last={#1}},%
  extras broken/.style={extras first={#1},extras middle={#1},extras last={#1}},%
  extras unbroken and first/.style={extras unbroken={#1},extras first={#1}},%
  extras unbroken and last/.style={extras unbroken={#1},extras last={#1}},%
  extras middle and last/.style={extras middle={#1},extras last={#1}},%
  extras first and middle/.style={extras first={#1},extras middle={#1}},%
  no extras unbroken/.code={\let\tcb@extras@unbroken\@empty},%
  no extras first/.code={\let\tcb@extras@first\@empty},%
  no extras middle/.code={\let\tcb@extras@middle\@empty},%
  no extras last/.code={\let\tcb@extras@last\@empty},%
  no extras/.code={\let\tcb@extras@unbroken\@empty\let\tcb@extras@first\@empty\let\tcb@extras@middle\@empty\let\tcb@extras@last\@empty},%
  if odd page*/.style 2 args={check odd page,extras={if odd page={#1}{#2}}},%
}


\tcbset{%
  reset@breakable/.style={%
    unbreakable,notitle after break,
    shrink break goal=0pt,
    lines before break=2,
    topsep at break=0pt,
    bottomsep at break=0pt,
    enlargepage=0pt,enlargepage flexible=0pt,
    break at=0pt,
    height fixed for=none,
    vfill before first=false,
    no extras,
  },
  initialize@reset=reset@breakable,
}


==> tcbdocumentation.code.tex <==
%% The LaTeX package tcolorbox - version 3.90 (2016/02/29)
%% tcbdocumentation.code.tex: Code for LaTeX documentations
%%
%% -------------------------------------------------------------------------------------------
%% Copyright (c) 2006-2016 by Prof. Dr. Dr. Thomas F. Sturm <thomas dot sturm at unibw dot de>
%% -------------------------------------------------------------------------------------------
%%
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either version 1.3
%% of this license or (at your option) any later version.
%% The latest version of this license is in
%%   http://www.latex-project.org/lppl.txt
%% and version 1.3 or later is part of all distributions of LaTeX
%% version 2005/12/01 or later.
%%
%% This work has the LPPL maintenance status `author-maintained'.
%%
%% This work consists of all files listed in README
%%
\tcb@set@library@version{3.90}

\tcbuselibrary{listings,skins,xparse,external}

\RequirePackage{pifont}[2005/04/12]
\RequirePackage{marvosym}[2011/07/20]
\ifdefined\printindex\else\RequirePackage{makeidx}[2000/03/29]\fi
\RequirePackage{refcount}[2011/10/16]
\RequirePackage{hyperref}[2012/02/06]
\ifdefined\marginnote\else\RequirePackage{marginnote}[2012/03/29]\fi

\definecolor{Option}{rgb}{0.118,0.546,0.222}
\definecolor{Definition}{rgb}{0.784,0.06,0.176}
\definecolor{ExampleFrame}{rgb}{0.628,0.705,0.942}
\definecolor{ExampleBack}{rgb}{0.963,0.971,0.994}
\definecolor{Hyperlink}{rgb}{0.281,0.275,0.485}

\def\colDef#1{\textcolor{\kvtcb@col@command}{#1}}
\def\colOpt#1{\textcolor{\kvtcb@col@opt}{#1}}

\lstdefinestyle{tcbdocumentation}{language={[LaTeX]TeX},
    aboveskip={0\p@ \@plus 6\p@},
    belowskip={0\p@ \@plus 6\p@},
    columns=fullflexible,
    keepspaces=true,
    breaklines=true,
    prebreak={\Righttorque},
    postbreak={\space\Lefttorque},
    breakatwhitespace=true,
    basicstyle=\ttfamily\footnotesize,
    extendedchars=true,
    moredelim={[is][\itshape\rmfamily]{^^a7}{^^a7}},
    nolol,inputencoding=\kvtcb@listingencoding}

% The following macros are taken from ltxdoc
\DeclareRobustCommand\cs[1]{\texttt{\char`\\#1}}
\def\meta@font@select{\rmfamily\itshape}

\AtEndPreamble{%
  \@ifpackageloaded{doc}{%
  }{% code taken from doc.sty
    \ifx\l@nohyphenation\undefined
      \newlanguage\l@nohyphenation
    \fi
    \DeclareRobustCommand\meta[1]{%
         \ensuremath\langle
         \ifmmode \expandafter \nfss@text \fi
         {%
          \meta@font@select
          \edef\meta@hyphen@restore
            {\hyphenchar\the\font\the\hyphenchar\font}%
          \hyphenchar\font\m@ne
          \language\l@nohyphenation
          #1\/%
          \meta@hyphen@restore
         }\ensuremath\rangle
    }%
  }%
}%

\def\marg#1{%
  {\ttfamily\char`\{}\meta{#1}{\ttfamily\char`\}}}
\def\oarg#1{%
  \colOpt{{\ttfamily[}\meta{#1}{\ttfamily]}}}

\newrobustcmd\tcb@cs[1]{{\catcode`\_=12\relax\catcode`\@11\relax\ttfamily\char`\\\scantokens{#1}\unskip}}
\newrobustcmd\tcb@scantokens[1]{{\catcode`\_=12\relax\catcode`\@11\relax\ttfamily\scantokens{#1}\unskip}}

\newif\iftcb@doc@toindex
\newif\iftcb@doc@colorize
\newif\iftcb@doc@annotate

% language specific texts
\tcbset{
  doclang/.cd,
  color/.store in=\kvtcb@text@color,
  colors/.store in=\kvtcb@text@colors,
  counter/.store in=\kvtcb@text@counter,
  counters/.store in=\kvtcb@text@counters,
  environment content/.store in=\kvtcb@text@envcontent,
  environment/.store in=\kvtcb@text@env,
  environments/.store in=\kvtcb@text@envs,
  index/.store in=\kvtcb@text@index,
  key/.store in=\kvtcb@text@key,
  keys/.store in=\kvtcb@text@keys,
  length/.store in=\kvtcb@text@length,
  lengths/.store in=\kvtcb@text@lengths,
  new/.store in=\kvtcb@text@new,
  pageshort/.store in=\kvtcb@text@pageshort,
  updated/.store in=\kvtcb@text@updated,
  value/.store in=\kvtcb@text@value,
  values/.store in=\kvtcb@text@values,
}

% documentation options
\tcbset{
  documentation listing options/.store in=\kvtcb@doclistingoptions,%
  documentation listing style/.style={documentation listing options={style=#1}},%
  documentation minted style/.store in=\kvtcb@docmintstyle,
  documentation minted options/.store in=\kvtcb@docmintoptions,
  color command/.store in=\kvtcb@col@command,
  color environment/.store in=\kvtcb@col@environment,
  color key/.store in=\kvtcb@col@key,
  color value/.store in=\kvtcb@col@value,
  color counter/.store in=\kvtcb@col@counter,
  color length/.store in=\kvtcb@col@length,
  color color/.store in=\kvtcb@col@color,
  color definition/.style={color command={#1},color environment={#1},color key={#1},
    color value={#1},color color={#1},color counter={#1},color length={#1}},
  color option/.store in=\kvtcb@col@opt,
  color hyperlink/.store in=\kvtcb@colhyper,
  color frame/.store in=\kvtcb@colhyper,
  index actual/.store in=\idx@actual,
  index quote/.store in=\idx@quote,
  index level/.store in=\idx@level,
  index format/.store in=\idx@format,
  index colorize/.is if=tcb@doc@colorize,%
  index annotate/.is if=tcb@doc@annotate,%
  index command/.code={\def\kvtcb@index@command##1{#1{##1}}},%
  index command name/.code={\def\kvtcb@index@command##1{\index[#1]{##1}}},%
  doc left/.dimstore in=\kvtcb@doc@left,
  doc right/.dimstore in=\kvtcb@doc@right,
  doc left indent/.dimstore in=\kvtcb@doc@indentleft,
  doc right indent/.dimstore in=\kvtcb@doc@indentright,
  doc head command/.style={doc@head@command/.style={#1}},
  doc head environment/.style={doc@head@environment/.style={#1}},
  doc head key/.style={doc@head@key/.style={#1}},
  doc head/.style={doc head command={#1},doc head environment={#1},doc head key={#1}},
  before doc body command/.store in=\kvtcb@doc@body@command@before,
  after doc body command/.store in=\kvtcb@doc@body@command@after,
  before doc body environment/.store in=\kvtcb@doc@body@environment@before,
  after doc body environment/.store in=\kvtcb@doc@body@environment@after,
  before doc body key/.store in=\kvtcb@doc@body@key@before,
  after doc body key/.store in=\kvtcb@doc@body@key@after,
  before doc body/.style={before doc body command={#1},before doc body environment={#1},before doc body key={#1}},
  after doc body/.style={after doc body command={#1},after doc body environment={#1},after doc body key={#1}},
  doc description/.store in=\kvtcb@doc@description,%
  doc into index/.is if=tcb@doc@toindex,%
  doc updated/.style={before upper={\tcbdocmarginnote{\tcbdocupdated{#1}}}},
  doc new/.style={before upper={\tcbdocmarginnote{\tcbdocnew{#1}}}},
  doc new and updated/.style 2 args={before upper={\tcbdocmarginnote{\tcbdocnew{#1}\\\tcbdocupdated{#2}}}},
  doc marginnote/.style={doc@marginnote/.style={#1}},
}


% styles
\tcbset{
  docexample/.style={colframe=ExampleFrame,colback=ExampleBack,
    before skip=\medskipamount,after skip=\medskipamount,
    fontlower=\footnotesize},
  documentation minted style=,
  documentation minted options={tabsize=2,fontsize=\small},
  index default settings/.style={index actual={@},index quote={"},index level={!}},
  index german settings/.style={index actual={=},index quote={!},index level={>}},
  english language/.code={\tcbset{doclang/.cd,
    color=color,colors=Colors,
    counter=counter,counters=Counters,
    environment content=environment content,
    environment=environment,environments=Environments,
    index=Index,
    key=key,keys=Keys,
    length=length,lengths=Lengths,
    new=New,
    pageshort={P.},
    updated=Updated,
    value=value,values=Values}},
}

\AtBeginDocument{%
  \csname tcb@doc@index@\idx@format\endcsname%
  \hypersetup{
  citecolor=\kvtcb@colhyper,
  linkcolor=\kvtcb@colhyper,
  urlcolor=\kvtcb@colhyper,
  filecolor=\kvtcb@colhyper,
  menucolor=\kvtcb@colhyper
}}

\def\dispExample{\tcb@layer@pushup\tcbset{docexample}\begingroup\tcbwritetemp}

\def\enddispExample{%
  \endtcbwritetemp\endgroup%
  \begin{tcolorbox}%
  \tcb@doc@usetemplisting%
  \tcblower%
  \tcbusetemp%
  \end{tcolorbox}%
}

\newenvironment{dispExample*}[1]{%
  \tcb@layer@pushup\tcbset{docexample,#1}\begingroup\tcbwritetemp%
  }{\enddispExample}

\def\dispListing{\tcb@layer@pushup\tcbset{docexample}\begingroup\tcbwritetemp}

\def\enddispListing{%
  \endtcbwritetemp\endgroup%
  \begin{tcolorbox}%
  \tcb@doc@usetemplisting%
  \end{tcolorbox}%
}

\newenvironment{dispListing*}[1]{%
  \tcb@layer@pushup\tcbset{docexample,#1}\begingroup\tcbwritetemp%
  }{\enddispListing}

% index auxiliary macros
\def\tcb@Index@Print@CA#1#2#3{%
  \iftcb@doc@colorize\textcolor{#2}{\tcb@scantokens{#1}}\else\tcb@scantokens{#1}\fi%
  \iftcb@doc@annotate\ #3\fi%
}

\def\tcb@Index@Print@C#1#2{%
  \iftcb@doc@colorize\textcolor{#2}{\tcb@scantokens{#1}}\else\tcb@scantokens{#1}\fi%
}

\def\tcb@Index@Print@ComCA#1#2#3{%
  \iftcb@doc@colorize\textcolor{#2}{\tcb@cs{#1}}\else\tcb@cs{#1}\fi%
  \iftcb@doc@annotate\ #3\fi%
}

\def\tcb@Index@Print@ComC#1#2{%
  \iftcb@doc@colorize\textcolor{#2}{\tcb@cs{#1}}\else\tcb@cs{#1}\fi%
}

\newrobustcmd{\tcbIndexPrintComC}[1]{\tcb@Index@Print@ComC{#1}{\kvtcb@col@command}}
\def\tcb@Print@Com#1{\textcolor{\kvtcb@col@command}{\bfseries\tcb@cs{#1}}}

\newrobustcmd{\tcbIndexPrintEnvCA}[1]{\tcb@Index@Print@CA{#1}{\kvtcb@col@environment}{\kvtcb@text@env}}
\newrobustcmd{\tcbIndexPrintEnvC}[1]{\tcb@Index@Print@C{#1}{\kvtcb@col@environment}}
\def\tcb@Print@Env#1{\textcolor{\kvtcb@col@environment}{\bfseries\tcb@scantokens{#1}}}

\newrobustcmd{\tcbIndexPrintKeyCA}[1]{\tcb@Index@Print@CA{#1}{\kvtcb@col@key}{\kvtcb@text@key}}
\newrobustcmd{\tcbIndexPrintKeyC}[1]{\tcb@Index@Print@C{#1}{\kvtcb@col@key}}
\def\tcb@Print@Key#1{\textcolor{\kvtcb@col@key}{\bfseries\tcb@scantokens{#1}}}

\newrobustcmd{\tcbIndexPrintValCA}[1]{\tcb@Index@Print@CA{#1}{\kvtcb@col@value}{\kvtcb@text@value}}
\newrobustcmd{\tcbIndexPrintValC}[1]{\tcb@Index@Print@C{#1}{\kvtcb@col@value}}
\def\tcb@Print@Val#1{\textcolor{\kvtcb@col@value}{\bfseries\tcb@scantokens{#1}}}

\newrobustcmd{\tcbIndexPrintColCA}[1]{\tcb@Index@Print@CA{#1}{\kvtcb@col@color}{\kvtcb@text@color}}
\newrobustcmd{\tcbIndexPrintColC}[1]{\tcb@Index@Print@C{#1}{\kvtcb@col@color}}
\def\tcb@Print@Col#1{\textcolor{\kvtcb@col@color}{\bfseries\tcb@scantokens{#1}}}

\newrobustcmd{\tcbIndexPrintCountCA}[1]{\tcb@Index@Print@CA{#1}{\kvtcb@col@counter}{\kvtcb@text@counter}}
\newrobustcmd{\tcbIndexPrintCountC}[1]{\tcb@Index@Print@C{#1}{\kvtcb@col@counter}}
\def\tcb@Print@Count#1{\textcolor{\kvtcb@col@counter}{\bfseries\tcb@scantokens{#1}}}

\newrobustcmd{\tcbIndexPrintLenCA}[1]{\tcb@Index@Print@ComCA{#1}{\kvtcb@col@length}{\kvtcb@text@length}}
\newrobustcmd{\tcbIndexPrintLenC}[1]{\tcb@Index@Print@ComC{#1}{\kvtcb@col@length}}
\def\tcb@Print@Len#1{\textcolor{\kvtcb@col@length}{\bfseries\tcb@cs{#1}}}

\def\tcb@index@Com#1{\iftcb@doc@toindex\kvtcb@index@command{#1\idx@actual\tcbIndexPrintComC{#1}}\fi}
\def\tcb@index@Env#1{\iftcb@doc@toindex\kvtcb@index@command{#1\idx@actual\tcbIndexPrintEnvCA{#1}}\kvtcb@index@command{\kvtcb@text@envs\idx@level#1\idx@actual\tcbIndexPrintEnvC{#1}}\fi}
\def\tcb@index@Key#1{\iftcb@doc@toindex\kvtcb@index@command{#1\idx@actual\tcbIndexPrintKeyCA{#1}}\kvtcb@index@command{\kvtcb@text@keys\idx@level#1\idx@actual\tcbIndexPrintKeyC{#1}}\fi}%
\def\tcb@index@KeyPath#1#2{\iftcb@doc@toindex\kvtcb@index@command{#2\idx@actual\tcbIndexPrintKeyCA{#2}}\kvtcb@index@command{\kvtcb@text@keys\idx@level#1\idx@actual\tcbIndexPrintKeyC{/#1/}\idx@level#2\idx@actual\tcbIndexPrintKeyC{#2}}\fi}%
\def\tcb@index@Val#1{\iftcb@doc@toindex\kvtcb@index@command{#1\idx@actual\tcbIndexPrintValCA{#1}}\kvtcb@index@command{\kvtcb@text@values\idx@level#1\idx@actual\tcbIndexPrintValC{#1}}\fi}
\def\tcb@index@Col#1{\iftcb@doc@toindex\kvtcb@index@command{#1\idx@actual\tcbIndexPrintColCA{#1}}\kvtcb@index@command{\kvtcb@text@colors\idx@level#1\idx@actual\tcbIndexPrintColC{#1}}\fi}
\def\tcb@index@Count#1{\iftcb@doc@toindex\kvtcb@index@command{#1\idx@actual\tcbIndexPrintCountCA{#1}}\kvtcb@index@command{\kvtcb@text@counters\idx@level#1\idx@actual\tcbIndexPrintCountC{#1}}\fi}
\def\tcb@index@Len#1{\iftcb@doc@toindex\kvtcb@index@command{#1\idx@actual\tcbIndexPrintLenCA{#1}}\kvtcb@index@command{\kvtcb@text@lengths\idx@level#1\idx@actual\tcbIndexPrintLenC{#1}}\fi}

\def\brackets#1{{\ttfamily\char`\{}#1{\ttfamily\char`\}}}

\newenvironment{tcb@manual@entry}{\begin{list}{}{%
  \setlength{\leftmargin}{\kvtcb@doc@left}%
  \setlength{\itemindent}{0pt}%
  \setlength{\itemsep}{0pt}%
  \setlength{\parsep}{0pt}%
  \setlength{\rightmargin}{\kvtcb@doc@right}%
  }\item}{\end{list}}

\def\tcb@manual@top#1{\itemsep=0pt\parskip=0pt\item\strut{#1}\par\topsep=0pt}

\def\tcb@doc@do@description{%
  \ifx\kvtcb@doc@description\@empty\else\tcblower\raggedleft(\kvtcb@doc@description)\fi%
}

\newtcolorbox{tcb@doc@head}[1]{blank,colback=white,colframe=white,
  code={\tcbdimto\tcb@temp@grow@left{-\kvtcb@doc@indentleft}%
        \tcbdimto\tcb@temp@grow@right{-\kvtcb@doc@indentright}},
  grow to left by=\tcb@temp@grow@left,%
  grow to right by=\tcb@temp@grow@right,
  sidebyside,sidebyside align=top,
  sidebyside gap=-\tcb@w@upper@real,
  phantom=\phantomsection,%
  enlarge bottom by=-0.2\baselineskip,#1}

% main documentation environments
\newenvironment{docCommand}[3][]{\tcbset{#1}%
  \begin{tcb@manual@entry}%
  \begin{tcb@doc@head}{doc@head@command}%
  \tcb@Print@Com{#2}\tcb@index@Com{#2}\protected@edef\@currentlabel{\noexpand\tcb@cs{#2}}\label{com:#2}{\ttfamily #3}%
  \tcb@doc@do@description%
  \end{tcb@doc@head}\nobreak\tcbset{before upper=}\kvtcb@doc@body@command@before\ignorespaces}%
  {\ifvmode\else\unskip\fi\kvtcb@doc@body@command@after\end{tcb@manual@entry}}

\newenvironment{docCommand*}{\bgroup\tcb@doc@toindexfalse\begin{docCommand}}{\end{docCommand}\egroup}

\newenvironment{docEnvironment}[3][]{\tcbset{#1}%
  \begin{tcb@manual@entry}%
  \begin{tcb@doc@head}{doc@head@environment}%
  \strut\cs{begin}\brackets{\tcb@Print@Env{#2}}\tcb@index@Env{#2}\protected@edef\@currentlabel{#2}\label{env:#2}{\ttfamily #3}\par%
  \strut~~\meta{\kvtcb@text@envcontent}\par%
  \strut\cs{end}\brackets{\tcb@Print@Env{#2}}%
  \tcb@doc@do@description%
  \end{tcb@doc@head}\nobreak\tcbset{before upper=}\kvtcb@doc@body@environment@before\ignorespaces}%
  {\ifvmode\else\unskip\fi\kvtcb@doc@body@environment@after\end{tcb@manual@entry}}

\newenvironment{docEnvironment*}{\bgroup\tcb@doc@toindexfalse\begin{docEnvironment}}{\end{docEnvironment}\egroup}

\NewDocumentEnvironment{docKey}{ O{} +O{} m m +m }{\tcbset{#2,doc description={#5}}%
  \begin{tcb@manual@entry}%
  \begin{tcb@doc@head}{doc@head@key}%
  \ifblank{#1}{%
    \tcb@Print@Key{#3}\tcb@index@Key{#3}\protected@edef\@currentlabel{#3}\label{key:#3}{\ttfamily #4}%
  }{%
    \tcb@Print@Key{/#1/#3}%
    \tcb@index@KeyPath{#1}{#3}\protected@edef\@currentlabel{/#1/#3}\label{key:/#1/#3}{\ttfamily #4}%
  }%
  \tcb@doc@do@description%
  \end{tcb@doc@head}\nobreak\tcbset{before upper=}\kvtcb@doc@body@key@before\ignorespaces}%
  {\ifvmode\else\unskip\fi\kvtcb@doc@body@key@after\end{tcb@manual@entry}}

\newenvironment{docKey*}{\bgroup\tcb@doc@toindexfalse\begin{docKey}}{\end{docKey}\egroup}

\def\tcbmakedocSubKey#1#2{%
  \NewDocumentEnvironment{#1}{ O{} +O{} m m +m }{%
    \ifblank{##1}{\def\tcb@key@path{#2}}{\def\tcb@key@path{#2/##1}}%
    \begin{docKey}[\tcb@key@path][##2]{##3}{##4}{##5}}%
      {\end{docKey}}%
  \newenvironment{#1*}{\bgroup\tcb@doc@toindexfalse\begin{#1}}{\end{#1}\egroup}%
}

\DeclareDocumentCommand\docAuxCommand{sm}{%
  \tcb@Print@Com{#2}%
  \IfBooleanTF{#1}{}{\tcb@index@Com{#2}}%
}

\DeclareDocumentCommand\docAuxEnvironment{sm}{%
  \tcb@Print@Env{#2}%
  \IfBooleanTF{#1}{}{\tcb@index@Env{#2}}%
}

\DeclareDocumentCommand\docAuxKey{sO{}m}{%
  \ifblank{#2}{%
    \tcb@Print@Key{#3}%
    \IfBooleanTF{#1}{}{\tcb@index@Key{#3}}%
  }{%
    \tcb@Print@Key{/#2/#3}%
    \IfBooleanTF{#1}{}{\tcb@index@KeyPath{#2}{#3}}%
}}

\DeclareDocumentCommand\docColor{sm}{%
  \tcb@Print@Col{#2}%
  \IfBooleanTF{#1}{}{\tcb@index@Col{#2}}%
}

\DeclareDocumentCommand\docCounter{sm}{%
  \tcb@Print@Count{#2}%
  \IfBooleanTF{#1}{}{\tcb@index@Count{#2}}%
}

\DeclareDocumentCommand\docLength{sm}{%
  \tcb@Print@Len{#2}%
  \IfBooleanTF{#1}{}{\tcb@index@Len{#2}}%
}

\DeclareDocumentCommand\docValue{sm}{%
  \tcb@Print@Val{#2}%
  \IfBooleanTF{#1}{}{\tcb@index@Val{#2}}%
}

\setrefcountdefault{-1}
\DeclareDocumentCommand\tcb@ref@doc{msm}{%
  \hyperref[#1:#3]{\texttt{\ref*{#1:#3}}%
  \IfBooleanTF{#2}{}{%
    \ifnum\getpagerefnumber{#1:#3}=\thepage%
    \else%
      \textsuperscript{\ding{213}\,\kvtcb@text@pageshort\,\pageref*{#1:#3}}%
    \fi}}%
}

\def\refCom{\tcb@ref@doc{com}}
\def\refEnv{\tcb@ref@doc{env}}
\def\refKey{\tcb@ref@doc{key}}

\def\refAux#1{\textcolor{\kvtcb@colhyper}{\tcb@scantokens{#1}}}
\def\refAuxcs#1{\textcolor{\kvtcb@colhyper}{\tcb@cs{#1}}}

\newenvironment{absquote}
               {\list{}{\leftmargin2cm\rightmargin\leftmargin}%
                \item\relax\footnotesize}
               {\endlist}

\newcommand{\tcbdocmarginnote}[2][]{%
  \marginnote{%
  \begin{tcolorbox}[enhanced jigsaw,size=fbox,boxrule=1pt,leftrule=0pt,rightrule=0pt,
    arc=0pt,outer arc=1pt,boxsep=1pt,top=1pt,bottom=1pt,
    nobeforeafter,width=\marginparwidth,
    colframe=red!50!white,colback=red!25!yellow!5!white,fontupper=\scriptsize,before upper=\flushright,
    doc@marginnote,#1]#2\end{tcolorbox}}}

\newcommand*{\tcbdocnew}[1]{\kvtcb@text@new: #1}
\newcommand*{\tcbdocupdated}[1]{\kvtcb@text@updated: #1}

%--- index macros taken from pgfmanual-en-macros
\def\tcb@doc@index@pgf@{%
  \ifdefined\c@IndexColumns%
    \c@IndexColumns=2%
  \fi%
  \def\theindex{\@restonecoltrue
    \columnseprule \z@  \columnsep 29\p@
    \twocolumn[\index@prologue]%
    \parindent -30pt%
    \columnsep 15pt%
    \parskip 0pt plus 1pt%
    \leftskip 30pt%
    \rightskip 0pt plus 2cm%
    \small%
    \def\@idxitem{\par}%
    \let\item\@idxitem\ignorespaces}
  \def\endtheindex{\onecolumn}%
  \def\noindexing{\let\index=\@gobble}%
}

\def\tcb@doc@index@pgfsection{%
  \def\index@prologue{\section*{\kvtcb@text@index}\addcontentsline{toc}{section}{\kvtcb@text@index}%
    \par\noindent%
  }%
  \tcb@doc@index@pgf@%
}

\def\tcb@doc@index@pgfchapter{%
  \def\index@prologue{\ifdefined\phantomsection\phantomsection\fi\@makeschapterhead{\kvtcb@text@index}\addcontentsline{toc}{chapter}{\kvtcb@text@index}}%
  \tcb@doc@index@pgf@%
}

\let\tcb@doc@index@pgf=\tcb@doc@index@pgfsection%

\def\tcb@doc@index@doc{%
  \let\tcb@index@Com=\SpecialMainIndex%%
  \let\tcb@index@Env=\SpecialMainEnvIndex%
  \tcbset{index german settings}%
  \EnableCrossrefs%
  \PageIndex%
}

\def\tcb@doc@index@off{}%

\tcbset{%
  reset@documentation/.style={%
    index command=\index,%
    index format=pgf,
    english language,
    documentation listing style=tcbdocumentation,
    index default settings,
    color option=Option,
    color definition=Definition,
    color hyperlink=Hyperlink,
    doc left=2em,
    doc right=0pt,
    doc left indent=-2em,
    doc right indent=0pt,
    doc head=,
    before doc body=,
    after doc body=,
    doc description=,
    doc into index=true,
    index colorize=false,
    index annotate=true,
    doc marginnote=,
    },
  initialize@reset=reset@documentation,
}

% deprecated
\tcbset{
  before example/.store in=\kvtcb@beforeexample,
  after example/.store in=\kvtcb@afterexample,
    before example=\par\smallskip,
    after example=,
}


==> tcbexternal.code.tex <==
%% The LaTeX package tcolorbox - version 3.90 (2016/02/29)
%% tcbexternal.code.tex: Code for externalization
%%
%% -------------------------------------------------------------------------------------------
%% Copyright (c) 2006-2016 by Prof. Dr. Dr. Thomas F. Sturm <thomas dot sturm at unibw dot de>
%% -------------------------------------------------------------------------------------------
%%
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either version 1.3
%% of this license or (at your option) any later version.
%% The latest version of this license is in
%%   http://www.latex-project.org/lppl.txt
%% and version 1.3 or later is part of all distributions of LaTeX
%% version 2005/12/01 or later.
%%
%% This work has the LPPL maintenance status `author-maintained'.
%%
%% This work consists of all files listed in README
%%
\tcb@set@library@version{3.90}

{
\catcode`\"=12
\xdef\tcbexternal@normal@dq{"}
\catcode`\"=13
\gdef\tcbexternal@activate@normal@dq{\let"=\tcbexternal@normal@dq}
}

\long\def\tcbifexternal#1#2{%
  \ifdefined\TCBEXTERNALINPUT%
    #1%
  \else%
    #2%
  \fi%
}

\tcbifexternal{%
  \def\tcbEXTERNALIZE{%
    \RequirePackage{incgraph}%
    \TCBEXTERNALPREAMBLE%
    \begin{document}%
    \begin{inctext}[border=\TCBEXTERNALSAFETY]%
    \input{\TCBEXTERNALINPUT}%
    \end{inctext}%
    \end{document}%
  }%
}{%
  \def\tcbEXTERNALIZE{%
    \tcbset{
      external/.cd,
      externalize/.is if=tcb@externalize,
      externalize=true,
    }%
  }%
}

\@onlypreamble\tcbEXTERNALIZE

\def\tcbexternal@setbasename#1{%
  \edef\tcbexternal@job@name{\expandonce{\tcbexternal@prefix}\expandonce{#1}}%
  \edef\tcbexternal@job@mdfive{\expandonce{\tcbexternal@job@name.md5}}%
  \edef\tcbexternal@job@source{\expandonce{\tcbexternal@job@name.tex}}%
  \edef\tcbexternal@job@pdf{\expandonce{\tcbexternal@job@name.pdf}}%
}

\def\tcbexternal@corecompile{%
  \begingroup%
  \ifnum\the\catcode`\"=13 \tcbexternal@activate@normal@dq\fi%
  \message{=== Compile external '\tcbexternal@job@name': }%
  \immediate\openout\tcb@out="\tcbexternal@run@tex"
  \immediate\write\tcb@out{\string\gdef\string\TCBEXTERNALINPUT{"\tcbexternal@job@source"}}%
  \immediate\write\tcb@out{\string\gdef\string\TCBEXTERNALSAFETY{\tcbexternal@safety}}%
  \immediate\write\tcb@out{\string\gdef\string\TCBEXTERNALPREAMBLE{\expandonce{\tcbexternal@preamble}}}%
  \ifdefempty{\tcbexternal@preclass}{}{\immediate\write\tcb@out{\expandonce{\tcbexternal@preclass}}}%
  \immediate\write\tcb@out{\string\input{"\jobname.tex"}}%
  \immediate\closeout\tcb@out%
  \foreach \n in {1,...,\tcbexternal@runs}
  {%
    \immediate\write18{%
      \tcbexternal@compiler\space
      -shell-escape
      -halt-on-error
      -interaction=batchmode
      -jobname="\tcbexternal@job@name"
      "\tcbexternal@run@tex"
    }%
  }%
  \endgroup%
}

\def\tcbexternal@inputsource{%
  \IfFileExists{\tcbexternal@job@source}%
    {\input{\tcbexternal@job@source}}%
    {\tcb@error{File '\tcbexternal@job@source' missing.}{}}%
}

\def\tcbexternal@pdfmissing@warning{%
  \tcb@warning{File '\tcbexternal@job@pdf' missing.
    Compilation error or shell-escape wasn't enabled or a subdirectory could'nt be generated}%
  \message{Load '\tcbexternal@job@source' instead}%
  \tcbexternal@inputsource%
}

\def\tcbexternal@pdfmissing@error{%
  \tcb@error{File '\tcbexternal@job@pdf' missing.
    Compilation error or shell-escape wasn't enabled or a subdirectory could'nt be generated}{}%
}

\def\tcbexternal@inputpdf{%
  \IfFileExists{\tcbexternal@job@pdf}%
    {%
      \begingroup\edef\x{\endgroup%
        \noexpand\includegraphics[trim=\tcbexternal@safety\space\tcbexternal@safety%
        \space\tcbexternal@safety\space\tcbexternal@safety]{\expandonce{\tcbexternal@job@pdf}}}%
      \x%
    }%
    {\tcbexternal@pdfmissing}%
}

\newif\iftcb@externalize
\tcb@externalizefalse

\def\tcbexternal@generatemdivesum{%
  \iftcb@externalize%
    \def\tcbexternallastmdfivesum{}%
    \IfFileExists{\tcbexternal@job@mdfive}{\input{\tcbexternal@job@mdfive}}{}%
    \edef\tcbexternalmdfivesum{\pdfmdfivesum file {\tcbexternal@job@source}}%
  \else%
    \def\tcbexternallastmdfivesum{x}%
    \edef\tcbexternalmdfivesum{}%
  \fi%
  \immediate\openout\tcb@out=\tcbexternal@job@mdfive%
  \immediate\write\tcb@out{\string\def\string\tcbexternallastmdfivesum{\tcbexternalmdfivesum}\@percentchar}%
  \immediate\closeout\tcb@out%
}

\def\tcbexternal@conditionalcompile{%
  \IfFileExists{\tcbexternal@job@pdf}{%
    \ifdefstrequal{\tcbexternallastmdfivesum}{\tcbexternalmdfivesum}{%
    }{%
      \tcbexternal@corecompile%
    }%
  }{%
    \tcbexternal@corecompile%
  }%
}

\def\tcb@useexternal{%
  \tcbexternal@generatemdivesum%
  \iftcb@externalize%
    \tcbexternal@compile%
    \tcbexternal@inputpdf%
  \else%
    \tcbexternal@inputsource%
  \fi%
}

\newenvironment{tcbexternal}[2][]{%
  \tcbset{external/.cd,#1,name=#2}%
  \@ifundefined{@tcbexternal@JN@\tcbexternal@job@name}{%
      \global\@namedef{@tcbexternal@JN@\tcbexternal@job@name}{}%
    }{%
      \tcb@error{External job name '\tcbexternal@job@name' already used}%
        {Give a new unique name to the current external job.}%
    }%
  \begingroup%
  \let\tcb@verbatim@begin@hook=\tcbexternal@out@begin%
  \let\tcb@verbatim@end@hook=\tcbexternal@out@end%
  \tcbverbatimwrite{\tcbexternal@job@source}}%
{%
  \endtcbverbatimwrite\endgroup%
  \tcb@useexternal%
}

\long\def\new@tcb@externalizeenvironment#1#2#3#4#5{%
  \tcb@newenvironment{#1}[2][]{%
    #4%
    \begingroup%
    \tcbexternal[#3,##1,environment=#2]{##2}%
  }{%
    \endtcbexternal%
    \endgroup%
    #5%
  }%
}

\def\newtcbexternalizeenvironment{%
  \let\tcb@newenvironment\newenvironment%
  \new@tcb@externalizeenvironment%
}

\def\renewtcbexternalizeenvironment{%
  \let\tcb@newenvironment\renewenvironment%
  \new@tcb@externalizeenvironment%
}

\long\def\new@tcb@externalizetcolorbox#1#2#3#4{%
  \new@tcb@externalizeenvironment{#1}{#2}%
    {preamble tcbset={force nobeforeafter},#3}%
    {\tcb@layer@pushup\tcb@apply@box@options{#4}\tcb@set@normal@unbroken@beforeafter\tcb@before@unbroken}%
    {\tcb@after@unbroken}%
}

\def\newtcbexternalizetcolorbox{%
  \let\tcb@newenvironment\newenvironment%
  \new@tcb@externalizetcolorbox%
}

\def\renewtcbexternalizetcolorbox{%
  \let\tcb@newenvironment\renewenvironment%
  \new@tcb@externalizetcolorbox%
}


\newtcbexternalizeenvironment{extikzpicture}{tikzpicture}{}{}{}

\newtcbexternalizetcolorbox{extcolorbox}{tcolorbox}{}{}


\tcbset{
  external/.cd,
  %
  runner/.code={%
    \edef\tcbexternal@run@tex{\expandonce{#1}}%
  },
  %
  prefix/.store in=\tcbexternal@prefix,
  compiler/.store in=\tcbexternal@compiler,
  runs/.code={\numdef\tcbexternal@runs{#1}},
  name/.code={\tcbexternal@setbasename{#1}},
  safety/.store in=\tcbexternal@safety,
  preamble/.code={\appto\tcbexternal@preamble{#1}},
  preamble tcbset/.code={\appto\tcbexternal@preamble{\tcbset{#1}}},
  clear preamble/.code={\def\tcbexternal@preamble{}},
  preclass/.code={\appto\tcbexternal@preclass{#1}},
  clear preclass/.code={\def\tcbexternal@preclass{}},
  PassOptionsToPackage/.code 2 args={\appto\tcbexternal@preclass{\PassOptionsToPackage{#1}{#2}}},
  PassOptionsToClass/.code 2 args={\appto\tcbexternal@preclass{\PassOptionsToClass{#1}{#2}}},
  externalize/.code={},
  -/.style={externalize=false},
  %
  force remake/.is choice,
  force remake/true/.code={\let\tcbexternal@compile=\tcbexternal@corecompile},
  force remake/false/.code={\let\tcbexternal@compile=\tcbexternal@conditionalcompile},
  force remake/.default=true,
  !/.style=force remake,
  %
  input source on error/.is choice,
  input source on error/true/.code={\let\tcbexternal@pdfmissing=\tcbexternal@pdfmissing@warning},
  input source on error/false/.code={\let\tcbexternal@pdfmissing=\tcbexternal@pdfmissing@error},
  input source on error/.default=true,
  %
  plain/.code={%
    \let\tcbexternal@out@begin=\@empty%
    \let\tcbexternal@out@end=\@empty%
  },
  minipage/.code={%
    \appto\tcbexternal@out@begin{\immediate\write\tcb@out{\string\begin{minipage}{\the\dimexpr#1\relax}\string\ignorespaces\@percentchar}}%
    \preto\tcbexternal@out@end{\immediate\write\tcb@out{\string\end{minipage}\@percentchar}}%
  },
  minipage/.default=\linewidth,
  %
  environment with percent/.is choice,
  environment with percent/true/.style={%
    /tcb/external/environment/.code={%
      \appto\tcbexternal@out@begin{\immediate\write\tcb@out{\string\begin{##1}\@percentchar}}%
      \preto\tcbexternal@out@end{\immediate\write\tcb@out{\string\end{##1}\@percentchar}}%
    }
  },
  environment with percent/false/.style={%
    /tcb/external/environment/.code={%
      \appto\tcbexternal@out@begin{\immediate\write\tcb@out{\string\begin{##1}}}%
      \preto\tcbexternal@out@end{\immediate\write\tcb@out{\string\end{##1}}}%
    }
  },
  environment with percent/.default=true,
  %
  runner=\jobname_run.tex,
  prefix={external/},
  compiler=pdflatex,
  runs=1,
  name=unnamed,
  safety=2mm,
  clear preamble,
  clear preclass,
  force remake=false,
  input source on error,
  environment with percent,
  plain
}

\tcbset{%
  externalize example/.style={%
    external/name=#1,tempfile=\tcbexternal@job@source,
    code={\let\tcbusetemp=\tcb@useexternal}%
  },
  externalize example!/.style={externalize example=#1,external/force remake},
  externalize listing/.style={%
    external/name=#1,listing file=\tcbexternal@job@source,
    code={\let\tcbuselistingtext@input=\tcb@useexternal}%
  },
  externalize listing!/.style={externalize listing=#1,external/force remake},
}


==> tcbfitting.code.tex <==
%% The LaTeX package tcolorbox - version 3.90 (2016/02/29)
%% tcbfitting.code.tex: Code for fit boxes
%%
%% -------------------------------------------------------------------------------------------
%% Copyright (c) 2006-2016 by Prof. Dr. Dr. Thomas F. Sturm <thomas dot sturm at unibw dot de>
%% -------------------------------------------------------------------------------------------
%%
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either version 1.3
%% of this license or (at your option) any later version.
%% The latest version of this license is in
%%   http://www.latex-project.org/lppl.txt
%% and version 1.3 or later is part of all distributions of LaTeX
%% version 2005/12/01 or later.
%%
%% This work has the LPPL maintenance status `author-maintained'.
%%
%% This work consists of all files listed in README
%%
%\makeatletter
\tcb@set@library@version{3.90}

\newdimen\tcbfitdim
\newdimen\tcb@lowerfitdim
\newdimen\tcb@upperfitdim
\newif\iftcb@continue

\tcbset{%
  fit/.style={capture=fitbox},%
  fit to/.style args={#1 and #2}{capture=fitbox,width=#1,height=#2},%
  fit to height/.style={capture=fitbox,height=#1},%
  fit basedim/.code={\def\kvtcb@fit@basedim{#1}\tcbfitdim\kvtcb@fit@basedim},%
  fit skip/.store in=\kvtcb@fit@skip,%
  fit fontsize macros/.code={%
    \renewcommand\tiny{\tcb@setfontsize\tiny{0.5}}%
    \renewcommand\scriptsize{\tcb@setfontsize\scriptsize{0.7}}%
    \renewcommand\footnotesize{\tcb@setfontsize\footnotesize{0.8}}%
    \renewcommand\small{\tcb@setfontsize\small{0.9}}%
    \renewcommand\normalsize{\tcb@setfontsize\normalsize{1}}%
    \renewcommand\large{\tcb@setfontsize\large{1.2}}%
    \renewcommand\Large{\tcb@setfontsize\Large{1.44}}%
    \renewcommand\LARGE{\tcb@setfontsize\LARGE{1.728}}%
    \renewcommand\huge{\tcb@setfontsize\huge{2.0736}}%
    \renewcommand\Huge{\tcb@setfontsize\Huge{2.48832}}},%
  fit height plus/.style={fit,height plus=#1},%
  fit width plus/.dimstore in=\kvtcb@fit@plus@width,%
  fit height from/.style args={#1 to #2}{fit,height from={#1} to {#2}},
  fit width from/.style args={#1 to #2}{fit,width={#1},fit width plus={#2-#1}},
  fit maxstep/.store in=\kvtcb@fit@maxstep,%
  fit maxfontdiff/.store in=\kvtcb@fit@maxfontdiff,%
  fit maxfontdiffgap/.store in=\kvtcb@fit@maxfontdiffgap,%
  fit maxwidthdiff/.store in=\kvtcb@fit@maxwidthdiff,%
  fit maxwidthdiffgap/.store in=\kvtcb@fit@maxwidthdiffgap,%
  fit warning/.is choice,
  fit warning/on/.code={\let\tcb@fit@warn@begin=\@empty%
    \let\tcb@fit@warn@end=\@empty},
  fit warning/off/.code={\def\tcb@fit@warn@begin{\hbadness=10000\relax}%
    \let\tcb@fit@warn@end=\@empty},
  fit warning/final/.code={\tcb@cur@hbadness=\hbadness\def\tcb@fit@warn@begin{\hbadness=10000\relax}%
    \def\tcb@fit@warn@end{\hbadness=\tcb@cur@hbadness\relax\tcb@fit@@box}},
  fit algorithm/.is choice,
  fit algorithm/fontsize/.code={\let\tcbox@fitalgorithm=\tcbox@fitalgorithm@fontsize},
  fit algorithm/fontsize*/.code={\let\tcbox@fitalgorithm=\tcbox@fitalgorithm@fontsize@star},
  fit algorithm/areasize/.code={\let\tcbox@fitalgorithm=\tcbox@fitalgorithm@areasize},
  fit algorithm/areasize*/.code={\let\tcbox@fitalgorithm=\tcbox@fitalgorithm@areasize@star},
  fit algorithm/hybrid/.code={\let\tcbox@fitalgorithm=\tcbox@fitalgorithm@hybrid},
  fit algorithm/hybrid*/.code={\let\tcbox@fitalgorithm=\tcbox@fitalgorithm@hybrid@star},
  fit algorithm/squeeze/.code={\let\tcbox@fitalgorithm=\tcbox@fitalgorithm@squeeze},
  spartan@fit/.style={fit algorithm=squeeze},
}

\def\tcb@@capture@fitbox{%
  \let\endtcolorbox=\relax%
  \Collect@Body\tcbox@inner@fitbox@collected%
}

\def\tcbfontsize#1{\fontsize{#1\tcbfitdim}{#1\dimexpr\kvtcb@fit@skip\tcbfitdim}\selectfont}

\def\tcb@setfontsize#1#2{\@setfontsize#1{#2\tcbfitdim}{#2\dimexpr\kvtcb@fit@skip\tcbfitdim}}

\long\def\tcbox@inner@fitbox@collected#1{%
  \tcbox@inner@fitbox{#1}%
  \tcb@finalize@environment%
}

\newcount\tcb@cur@hbadness

\def\tcbox@fitalgorithm@fontsize{%
  \tcb@continuetrue%
  \loop%
    \tcbfitdim.5\tcbfitdim%
    \tcb@fit@@box%
    \ifnum\count@=\kvtcb@fit@maxstep\relax%
      \tcb@continuefalse%
    \else%
      \ifdim\dimexpr\tcb@fit@@h>\tcb@fit@@target\relax%
        \ifdim\tcbfitdim<18000sp\relax%
          \count@\kvtcb@fit@maxstep\relax%
          \tcb@continuefalse%
        \fi%
      \else%
        \tcb@continuefalse%
      \fi%
    \fi%
  \iftcb@continue \repeat%
  \ifnum\count@<\kvtcb@fit@maxstep\relax%
    \tcbdimto\tcb@fit@@gap{\tcb@fit@@target-\tcb@fit@@h}%
    \tcb@lowerfitdim\tcbfitdim%
    \tcb@upperfitdim2\tcbfitdim%
    \tcbfitdim1.5\tcbfitdim%
    \loop%
      \tcb@fit@@box%
      \tcb@continuetrue%
      \ifnum\count@<\kvtcb@fit@maxstep\relax%
        \ifdim\dimexpr\tcb@upperfitdim-\tcb@lowerfitdim<\kvtcb@fit@maxfontdiff\relax%
          \tcb@continuefalse%
        \else%
          \ifdim\dimexpr\tcb@upperfitdim-\tcb@lowerfitdim<\kvtcb@fit@maxfontdiffgap\relax%
            \ifdim\dimexpr\tcb@fit@@gap<\tcb@fit@@line\relax%
              \tcb@continuefalse%
            \fi%
          \fi%
        \fi%
      \else%
        \tcb@continuefalse%
      \fi%
      \iftcb@continue%
        \ifdim\dimexpr\tcb@fit@@h>\tcb@fit@@target\relax%
          \tcb@upperfitdim\tcbfitdim%
          \advance\tcbfitdim\tcb@lowerfitdim%
          \tcbfitdim0.5\tcbfitdim%
        \else%
          \tcbdimto\tcb@fit@@gap{\tcb@fit@@target-\tcb@fit@@h}%
          \tcb@lowerfitdim\tcbfitdim%
          \advance\tcbfitdim\tcb@upperfitdim%
          \tcbfitdim0.5\tcbfitdim%
        \fi%
      \else%
        \ifdim\dimexpr\tcb@fit@@h>\tcb@fit@@target\relax%
          \tcbfitdim\tcb@lowerfitdim%
          \tcb@fit@@box%
        \fi%
      \fi%
    \iftcb@continue \repeat%
  \fi%
}

\def\tcbox@fitalgorithm@fontsize@star{%
  \tcbox@fitalgorithm@fontsize%
  \tcb@resize@box{\tcb@upperbox}{\tcb@w@upper}{\tcb@fit@@target}%
  \tcbdimto\tcb@fit@@h{\ht\tcb@upperbox+\dp\tcb@upperbox}%
}

\def\tcbox@fitalgorithm@areasize@core{%
  \pgfmathdivide{\tcb@fit@@h}{\tcb@fit@@target}%
  \pgfmathsqrt{\pgfmathresult}%
  \let\tcb@temp=\pgfmathresult%
  \tcbdimto\tcb@w@upper@temp{\pgfmathresult\dimexpr\tcb@w@upper}%
  \tcb@fit@@boxsave{\tcb@w@upper@temp}%
  %
  \tcbdimto\tcb@fit@@h{\ht\tcb@upperbox+\dp\tcb@upperbox}%
  \pgfmathdivide{\tcb@fit@@h}{\tcb@fit@@target}%
  \pgfmathdivide{\pgfmathresult}{\tcb@temp}%
  \pgfmathsqrt{\pgfmathresult}%
  \ifdim\dimexpr\pgfmathresult pt<0.98pt\relax
    \tcbdimto\tcb@w@upper@temp{\pgfmathresult\dimexpr\tcb@w@upper@temp}%
    \tcb@fit@@boxsave{\tcb@w@upper@temp}%
  \else\ifdim\dimexpr\pgfmathresult pt>1.02pt\relax
    \tcbdimto\tcb@w@upper@temp{\pgfmathresult\dimexpr\tcb@w@upper@temp}%
    \tcb@fit@@boxsave{\tcb@w@upper@temp}%
  \fi\fi%
  %
  \tcbdimto\tcb@fit@@h{\ht\tcb@upperbox+\dp\tcb@upperbox}%
}

\def\tcbox@fitalgorithm@areasize{%
  \tcbox@fitalgorithm@areasize@core%
  \pgfmathdivide{\tcb@w@upper}{\tcb@w@upper@temp}%
  \tcbdimto\tcb@fit@@h{\pgfmathresult\dimexpr\tcb@fit@@h}%
  \ifdim\dimexpr\tcb@fit@@h>\tcb@fit@@target\relax%
    \let\tcb@fit@@h=\tcb@fit@@target%
  \fi
  \tcb@resize@box{\tcb@upperbox}{\tcb@w@upper}{\tcb@fit@@h}%
  %
  \tcbdimto\tcb@fit@@h{\ht\tcb@upperbox+\dp\tcb@upperbox}%
}

\def\tcbox@fitalgorithm@areasize@star{%
  \tcbox@fitalgorithm@areasize@core%
  \tcb@resize@box{\tcb@upperbox}{\tcb@w@upper}{\tcb@fit@@target}%
  \tcbdimto\tcb@fit@@h{\ht\tcb@upperbox+\dp\tcb@upperbox}%
}

\def\tcbox@fitalgorithm@squeeze{%
  \tcb@resize@box{\tcb@upperbox}{\tcb@w@upper}{\tcb@fit@@target}%
  \tcbdimto\tcb@fit@@h{\ht\tcb@upperbox+\dp\tcb@upperbox}%
}

\def\tcbox@fitalgorithm@hybrid@core{%
  \pgfmathdivide{\tcb@fit@@target}{\tcb@fit@@h}%
  \pgfmathsqrt{\pgfmathresult}%
  \tcbfitdim=\pgfmathresult\tcbfitdim%
  \tcb@fit@@box%
  %
  \pgfmathdivide{\tcb@fit@@target}{\tcb@fit@@h}%
  \pgfmathsqrt{\pgfmathresult}%
  \ifdim\dimexpr\pgfmathresult pt<0.85pt\relax
    \tcbfitdim=\pgfmathresult\tcbfitdim%
    \tcb@fit@@box%
  \else\ifdim\dimexpr\pgfmathresult pt>1.15pt\relax
    \tcbfitdim=\pgfmathresult\tcbfitdim%
    \tcb@fit@@box%
  \fi\fi%
}

\def\tcbox@fitalgorithm@hybrid{%
  \tcbox@fitalgorithm@hybrid@core%
  \tcbox@fitalgorithm@areasize%
}

\def\tcbox@fitalgorithm@hybrid@star{%
  \tcbox@fitalgorithm@hybrid@core%
  \tcbox@fitalgorithm@areasize@star%
}

\def\tcb@fit@@box{%
  \iftcb@hasTitle%
    \tcbdimto\tcb@w@title{\kvtcb@width-(\kvtcb@left@rule)-(\kvtcb@right@rule)-(\kvtcb@boxsep)*2-(\kvtcb@lefttitle)-(\kvtcb@righttitle)}%
    \begin{tcb@savebox}{\tcb@titlebox}{\tcb@w@title}\color{tcbcol@title}\kvtcb@fonttitle\kvtcb@haligntitle\kvtcb@before@title\kvtcb@title\kvtcb@after@title\end{tcb@savebox}%
    \tcbdimto\tcb@h@titletotal{\ht\tcb@titlebox+\dp\tcb@titlebox+\kvtcb@title@rule+(\kvtcb@boxsep)*2+\kvtcb@toptitle+\kvtcb@bottomtitle}%
  \else%
    \let\tcb@h@titletotal=\tcb@zpt%
  \fi%
  \tcbdimto\tcb@fit@@line{\kvtcb@fit@skip\tcbfitdim}%
  \tcbdimto\tcb@w@upper{\kvtcb@width-(\kvtcb@left@rule)-(\kvtcb@right@rule)-(\kvtcb@boxsep)*2-(\kvtcb@leftupper)-(\kvtcb@rightupper)}%
  \tcb@fit@@boxsave{\tcb@w@upper}%
  \tcbdimto\tcb@fit@@h{\ht\tcb@upperbox+\dp\tcb@upperbox}%
  \tcbdimto\tcb@fit@@target{\kvtcb@height@fixed-(\kvtcb@top@rule@stand)-(\kvtcb@bottom@rule@stand)-(\kvtcb@top)-(\kvtcb@bottom)-(\kvtcb@boxsep)*2-\tcb@h@titletotal}%
}%

\long\def\tcbox@inner@fitbox#1{%
  \tcbset{breakable@false,sidebyside=false}%
  \let\tcb@space\tcb@zpt%
  \let\tcb@val@raisebase=\tcb@zpt%
  \unless\ifdefined\kvtcb@height@fixed%
    \tcbset{height=\kvtcb@width}%
  \fi%
  \tcb@hasLowerfalse%
  %
  \count@\z@%
  \tcbfitdim\kvtcb@fit@basedim%
  \tcb@fit@warn@begin%
  %
  \def\tcb@fit@@boxsave##1{%
    \tcbdimto\tcb@innerwidth{\kvtcb@width-\kvtcb@left@rule-\kvtcb@right@rule}%
    \colorlet{tcbcol@origin}{.}%
    \tcb@set@color{tcbcol@upper}%
    \begin{tcb@savebox}{\tcb@upperbox}{##1}%
      \kvtcb@fontupper\fontsize{\tcbfitdim}{\tcb@fit@@line}\selectfont%
%      \kvtcb@halignupper\kvtcb@before@upper\ignorespaces#1\unskip\kvtcb@after@upper%
      \kvtcb@halignupper\kvtcb@before@upper\ignorespaces#1\kvtcb@after@upper%
    \end{tcb@savebox}%
    \tcb@reset@color%
    \advance\count@ 1\relax%
  }%
  %
  \tcb@set@@phantom%
  \tcb@set@@title%
  \tcb@fit@@box%
  %
  % height fit
  \ifdim\kvtcb@height@fixed@plus>0pt\relax%
    \let\tcb@fit@@minheight=\kvtcb@height@fixed%
    \ifdim\dimexpr\tcb@fit@@h>\tcb@fit@@target\relax%
      \ifdim\dimexpr\tcb@fit@@h>\dimexpr\tcb@fit@@target+\kvtcb@height@fixed@plus\relax%
        \tcbdimto\kvtcb@height@fixed{\kvtcb@height@fixed+\kvtcb@height@fixed@plus}%
        \tcbdimto\tcb@fit@@target{\tcb@fit@@target+\kvtcb@height@fixed@plus}%
      \else%
        \tcbdimto\kvtcb@height@fixed{\kvtcb@height@fixed+\tcb@fit@@h-\tcb@fit@@target}%
        \let\tcb@fit@@target=\tcb@fit@@h%
      \fi%
    \fi%
  \fi%
  %
  % width fit
  \ifdim\kvtcb@fit@plus@width>0pt\relax%
    \ifnum\count@<\kvtcb@fit@maxstep\relax%
      \ifdim\dimexpr\tcb@fit@@h>\tcb@fit@@target\relax%
        \tcb@lowerfitdim\dimexpr\kvtcb@width\relax%
        \tcb@upperfitdim\dimexpr\kvtcb@width+\kvtcb@fit@plus@width\relax%
        \tcbdimto\kvtcb@width{\tcb@upperfitdim}%
        \tcb@fit@@box%
        \ifdim\dimexpr\tcb@fit@@h>\tcb@fit@@target\relax%
        \else%
          \ifnum\count@<\kvtcb@fit@maxstep\relax%
            \tcbdimto\tcb@fit@@gap{\tcb@fit@@target-\tcb@fit@@h}%
            \tcbdimto\kvtcb@width{(\tcb@lowerfitdim+\tcb@upperfitdim)/2}%
            \loop%
              \tcb@fit@@box%
              \tcb@continuetrue%
              \ifnum\count@<\kvtcb@fit@maxstep\relax%
                \ifdim\dimexpr\tcb@upperfitdim-\tcb@lowerfitdim<\kvtcb@fit@maxwidthdiff\relax%
                  \tcb@continuefalse%
                \else%
                  \ifdim\dimexpr\tcb@upperfitdim-\tcb@lowerfitdim<\kvtcb@fit@maxwidthdiffgap\relax%
                    \ifdim\dimexpr\tcb@fit@@gap<\tcb@fit@@line\relax%
                      \tcb@continuefalse%
                    \fi%
                  \fi%
                \fi%
              \else%
                \tcb@continuefalse%
              \fi%
              \iftcb@continue%
                \ifdim\dimexpr\tcb@fit@@h>\tcb@fit@@target\relax%
                  \tcb@lowerfitdim\dimexpr\kvtcb@width\relax%
                  \tcbdimto\kvtcb@width{(\tcb@lowerfitdim+\tcb@upperfitdim)/2}%
                \else%
                  \tcb@upperfitdim\dimexpr\kvtcb@width\relax%
                  \tcbdimto\tcb@fit@@gap{\tcb@fit@@target-\tcb@fit@@h}%
                  \tcbdimto\kvtcb@width{(\tcb@lowerfitdim+\tcb@upperfitdim)/2}%
                \fi%
              \else%
                \ifdim\dimexpr\tcb@fit@@h>\tcb@fit@@target\relax%
                  \tcbdimto\kvtcb@width{\tcb@upperfitdim}%
                  \tcb@fit@@box%
                \fi%
              \fi%
            \iftcb@continue \repeat%
          \fi%
        \fi%
      \fi%
    \fi%
  \fi%
  %
  % (font) fit
  \ifnum\count@<\kvtcb@fit@maxstep\relax%
    \ifdim\dimexpr\tcb@fit@@h>\tcb@fit@@target\relax%
    \tcbox@fitalgorithm%
    \fi%
  \fi%
  %
  \tcb@fit@warn@end%
  %
  % last height fit
  \ifdim\kvtcb@height@fixed@plus>0pt\relax%
    \ifdim\dimexpr\tcb@fit@@h<\tcb@fit@@target\relax%
      \tcbdimto\tcb@temp{\kvtcb@height@fixed+\tcb@fit@@h-\tcb@fit@@target}%
      \ifdim\dimexpr\tcb@temp<\tcb@fit@@minheight\relax%
      \else%
        \let\kvtcb@height@fixed=\tcb@temp%
      \fi%
    \fi%
  \fi%
  %
  \edef\tcbfitsteps{\the\count@}%
  \tcb@set@@dimensions%
  \tcb@draw@color@box%
}

\newcommand{\tcboxfit}[2][]{%
  \tcb@ox{capture=fitbox,#1}{#2}%
}

\long\def\tcb@newtcboxfit#1#2{\expandafter\tcb@newcommand\csname#1\endcsname{\tcboxfit[#2,options@for=#1]}}

\long\def\tcb@newtcboxfit@#1[#2]#3{\expandafter\tcb@newcommand\csname#1\endcsname[#2]{\tcboxfit[#3,options@for=#1]}}

\long\def\tcb@newtcboxfit@@#1[#2][#3]#4{\expandafter\tcb@newcommand\csname#1\endcsname[#2][#3]{\tcboxfit[#4,options@for=#1]}}

\long\def\tcb@new@tcboxfit@#1[#2]{%
  \@ifnextchar[{\tcb@newtcboxfit@@{#1}[#2]}{\tcb@newtcboxfit@{#1}[#2]}}

\long\def\tcb@new@tcboxfit#1{%
  \@ifnextchar[{\tcb@new@tcboxfit@{#1}}{\tcb@newtcboxfit{#1}}}

\def\newtcboxfit{%
  \let\tcb@newcommand\newcommand%
  \let\tcb@process@newtcolorbox@continue\tcb@new@tcboxfit%
  \tcb@process@newcommand}

\def\renewtcboxfit{%
  \let\tcb@newcommand\renewcommand%
  \let\tcb@process@newtcolorbox@continue\tcb@new@tcboxfit%
  \tcb@process@newcommand}

\tcbset{%
  reset@fitting/.style={%
    fit algorithm=fontsize,%
    fit basedim=10pt,fit skip=1.2,
    height plus=0pt,fit width plus=0pt,
    fit maxstep=20,fit maxfontdiff=0.1pt,fit maxfontdiffgap=1pt,
    fit maxwidthdiff=1pt,fit maxwidthdiffgap=10pt,
    fit warning=off
  },
  initialize@reset=reset@fitting,
}



==> tcbhooks.code.tex <==
%% The LaTeX package tcolorbox - version 3.90 (2016/02/29)
%% tcbhooks.code.tex: Code for adding hooks
%%
%% -------------------------------------------------------------------------------------------
%% Copyright (c) 2006-2016 by Prof. Dr. Dr. Thomas F. Sturm <thomas dot sturm at unibw dot de>
%% -------------------------------------------------------------------------------------------
%%
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either version 1.3
%% of this license or (at your option) any later version.
%% The latest version of this license is in
%%   http://www.latex-project.org/lppl.txt
%% and version 1.3 or later is part of all distributions of LaTeX
%% version 2005/12/01 or later.
%%
%% This work has the LPPL maintenance status `author-maintained'.
%%
%% This work consists of all files listed in README
%%
%\makeatletter
\tcb@set@library@version{3.90}

\tcbset{%
  before upper app/.code={\appto\kvtcb@before@upper{#1}},%
  before upper pre/.code={\preto\kvtcb@before@upper{#1}},%
  after upper app/.code={\appto\kvtcb@after@upper{#1}},%
  after upper pre/.code={\preto\kvtcb@after@upper{#1}},%
  before lower app/.code={\appto\kvtcb@before@lower{#1}},%
  before lower pre/.code={\preto\kvtcb@before@lower{#1}},%
  after lower app/.code={\appto\kvtcb@after@lower{#1}},%
  after lower pre/.code={\preto\kvtcb@after@lower{#1}},%
  before title app/.code={\appto\kvtcb@before@title{#1}},%
  before title pre/.code={\preto\kvtcb@before@title{#1}},%
  after title app/.code={\appto\kvtcb@after@title{#1}},%
  after title pre/.code={\preto\kvtcb@after@title{#1}},%
  %
  % usable inside the document or in the preamble after setting before / after
  before app/.code={\appto\kvtcb@beforebox{#1}},%
  before pre/.code={\preto\kvtcb@beforebox{#1}},%
  after app/.code={\appto\kvtcb@afterbox{#1}},%
  after pre/.code={\preto\kvtcb@afterbox{#1}},%
  %
  overlay unbroken app/.code={\appto\tcb@overlay@unbroken{#1}},%
  overlay unbroken pre/.code={\preto\tcb@overlay@unbroken{#1}},%
  overlay first app/.code={\appto\tcb@overlay@first{#1}},%
  overlay first pre/.code={\preto\tcb@overlay@first{#1}},%
  overlay middle app/.code={\appto\tcb@overlay@middle{#1}},%
  overlay middle pre/.code={\preto\tcb@overlay@middle{#1}},%
  overlay last app/.code={\appto\tcb@overlay@last{#1}},%
  overlay last pre/.code={\preto\tcb@overlay@last{#1}},%
  %
  overlay app/.style={overlay unbroken app={#1},overlay first app={#1},overlay middle app={#1},overlay last app={#1}},%
  overlay pre/.style={overlay unbroken pre={#1},overlay first pre={#1},overlay middle pre={#1},overlay last pre={#1}},%
  overlay broken app/.style={overlay first app={#1},overlay middle app={#1},overlay last app={#1}},%
  overlay broken pre/.style={overlay first pre={#1},overlay middle pre={#1},overlay last pre={#1}},%
  overlay unbroken and first app/.style={overlay unbroken app={#1},overlay first app={#1}},%
  overlay unbroken and first pre/.style={overlay unbroken pre={#1},overlay first pre={#1}},%
  overlay unbroken and last app/.style={overlay unbroken app={#1},overlay last app={#1}},%
  overlay unbroken and last pre/.style={overlay unbroken pre={#1},overlay last pre={#1}},%
  overlay middle and last app/.style={overlay middle app={#1},overlay last app={#1}},%
  overlay middle and last pre/.style={overlay middle pre={#1},overlay last pre={#1}},%
  overlay first and middle app/.style={overlay first app={#1},overlay middle app={#1}},%
  overlay first and middle pre/.style={overlay first pre={#1},overlay middle pre={#1}},%
  %
  % skins:
  frame code app/.code={\appto\tcb@frame@code{#1}},%
  frame code pre/.code={\preto\tcb@frame@code{#1}},%
  interior titled code app/.code={\appto\tcb@interiortitled@code{#1}},%
  interior titled code pre/.code={\preto\tcb@interiortitled@code{#1}},%
  interior code app/.code={\appto\tcb@interior@code{#1}},%
  interior code pre/.code={\preto\tcb@interior@code{#1}},%
  segmentation code app/.code={\appto\tcb@segmentation@code{#1}},%
  segmentation code pre/.code={\preto\tcb@segmentation@code{#1}},%
  title code app/.code={\appto\tcb@title@code{#1}},%
  title code pre/.code={\preto\tcb@title@code{#1}},%
  %
  extras unbroken pre/.code={\preto\tcb@extras@unbroken{#1}},%
  extras first pre/.code={\preto\tcb@extras@first{#1}},%
  extras middle pre/.code={\preto\tcb@extras@middle{#1}},%
  extras last pre/.code={\preto\tcb@extras@last{#1}},%
  extras pre/.style={extras unbroken pre={#1},extras first pre={#1},extras middle pre={#1},extras last pre={#1}},%
  extras broken pre/.style={extras first pre={#1},extras middle pre={#1},extras last pre={#1}},%
  extras unbroken and first pre/.style={extras unbroken pre={#1},extras first pre={#1}},%
  extras unbroken and last pre/.style={extras unbroken pre={#1},extras last pre={#1}},%
  extras middle and last pre/.style={extras middle pre={#1},extras last pre={#1}},%
  extras first and middle pre/.style={extras first pre={#1},extras middle pre={#1}},%
  %
  underlay unbroken pre/.code={\preto\tcb@underlay@unbroken{#1}},%
  underlay first pre/.code={\preto\tcb@underlay@first{#1}},%
  underlay middle pre/.code={\preto\tcb@underlay@middle{#1}},%
  underlay last pre/.code={\preto\tcb@underlay@last{#1}},%
  underlay boxed title pre/.code={\preto\tcb@underlay@boxedtitle{#1}},%
  underlay pre/.style={underlay unbroken pre={#1},underlay first pre={#1},underlay middle pre={#1},underlay last pre={#1}},%
  underlay broken pre/.style={underlay first pre={#1},underlay middle pre={#1},underlay last pre={#1}},%
  underlay unbroken and first pre/.style={underlay unbroken pre={#1},underlay first pre={#1}},%
  underlay unbroken and last pre/.style={underlay unbroken pre={#1},underlay last pre={#1}},%
  underlay middle and last pre/.style={underlay middle pre={#1},underlay last pre={#1}},%
  underlay first and middle pre/.style={underlay first pre={#1},underlay middle pre={#1}},%
  finish unbroken pre/.code={\preto\tcb@finish@unbroken{#1}},%
  finish first pre/.code={\preto\tcb@finish@first{#1}},%
  finish middle pre/.code={\preto\tcb@finish@middle{#1}},%
  finish last pre/.code={\preto\tcb@finish@last{#1}},%
  finish pre/.style={finish unbroken pre={#1},finish first pre={#1},finish middle pre={#1},finish last pre={#1}},%
  finish broken pre/.style={finish first pre={#1},finish middle pre={#1},finish last pre={#1}},%
  finish unbroken and first pre/.style={finish unbroken pre={#1},finish first pre={#1}},%
  finish unbroken and last pre/.style={finish unbroken pre={#1},finish last pre={#1}},%
  finish middle and last pre/.style={finish middle pre={#1},finish last pre={#1}},%
  finish first and middle pre/.style={finish first pre={#1},finish middle pre={#1}},%
  %
  watermark tikz app/.style={overlay app={\tcb@drawspec@watermark@tikz{#1}}},
  watermark tikz pre/.style={overlay pre={\tcb@drawspec@watermark@tikz{#1}}},
  watermark tikz app on/.style args={#1 is #2}{overlay #1 app={\tcb@drawspec@watermark@tikz{#2}}},%
  watermark tikz pre on/.style args={#1 is #2}{overlay #1 pre={\tcb@drawspec@watermark@tikz{#2}}},%
  watermark graphics app/.style={overlay app={\tcb@drawspec@watermark@graphics{#1}}},
  watermark graphics pre/.style={overlay pre={\tcb@drawspec@watermark@graphics{#1}}},
  watermark graphics app on/.style args={#1 is #2}{overlay #1 app={\tcb@drawspec@watermark@graphics{#2}}},
  watermark graphics pre on/.style args={#1 is #2}{overlay #1 pre={\tcb@drawspec@watermark@graphics{#2}}},
  watermark text app/.style={overlay app={\tcb@drawspec@watermark@text{#1}}},
  watermark text pre/.style={overlay pre={\tcb@drawspec@watermark@text{#1}}},
  watermark text app on/.style args={#1 is #2}{overlay #1 app={\tcb@drawspec@watermark@text{#2}}},
  watermark text pre on/.style args={#1 is #2}{overlay #1 pre={\tcb@drawspec@watermark@text{#2}}},
}



==> tcblistings.code.tex <==
%% The LaTeX package tcolorbox - version 3.90 (2016/02/29)
%% tcblistings.code.tex: Code for colorboxes with listings
%%
%% -------------------------------------------------------------------------------------------
%% Copyright (c) 2006-2016 by Prof. Dr. Dr. Thomas F. Sturm <thomas dot sturm at unibw dot de>
%% -------------------------------------------------------------------------------------------
%%
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either version 1.3
%% of this license or (at your option) any later version.
%% The latest version of this license is in
%%   http://www.latex-project.org/lppl.txt
%% and version 1.3 or later is part of all distributions of LaTeX
%% version 2005/12/01 or later.
%%
%% This work has the LPPL maintenance status `author-maintained'.
%%
%% This work consists of all files listed in README
%%
%\makeatletter
\tcb@set@library@version{3.90}

\RequirePackage{listings}[2007/02/22]

\tcbuselibrary{listings@core}

\let\tcb@listing@MakeCaption@org=\lst@MakeCaption

\def\tcb@listing@set@MakeCaption@org{%
  \let\lst@MakeCaption\tcb@listing@MakeCaption@org}
\def\tcb@listing@set@MakeCaption@empty{%
  \lst@HRefStepCounter{lstlisting}%
  \let\lst@MakeCaption\@gobble}

\lstdefinestyle{tcblatex}{language={[LaTeX]TeX},
     aboveskip={0\p@ \@plus 6\p@}, belowskip={0\p@ \@plus 6\p@},
     columns=fullflexible, keepspaces=true,
     breaklines=true, breakatwhitespace=true,
     basicstyle=\ttfamily\small, extendedchars=true, nolol,
     inputencoding=\kvtcb@listingencoding}

\def\tcb@listing@input@listing#1#2{%
  \begingroup%
  \toks@=\expandafter{#1}%
  \edef\tcb@temp{\noexpand\lstinputlisting[nolol,\the\toks@]}%
  \tcb@listing@set@MakeCaption%
  \tcb@temp{#2}%
  \endgroup%
}%


\def\tcb@listing@uselistinglisting{%
  \tcb@listing@input@listing{\kvtcb@listingoptions}{\kvtcb@listingfile}%
}%

\def\tcb@listing@usetemplisting{%
  \tcb@listing@input@listing{\kvtcb@listingoptions}{\kvtcb@tempfile}%
}%

\def\tcb@listing@doc@usetemplisting{%
  \tcb@listing@input@listing{\kvtcb@doclistingoptions}{\kvtcb@tempfile}%
}

\tcbset{%
  listing options/.store in=\kvtcb@listingoptions,%
  listing style/.style={listing options={style=#1}},%
  no listing options/.style={listing options=},%
  listing inputencoding/.store in=\kvtcb@listingencoding,%
  listing remove caption/.is choice,
  listing remove caption/true/.code={\let\tcb@listing@set@MakeCaption\tcb@listing@set@MakeCaption@empty},
  listing remove caption/false/.code={\let\tcb@listing@set@MakeCaption\tcb@listing@set@MakeCaption@org},
  listing remove caption/.default=true,
  listing engine/listings/.code={\let\tcbuselistinglisting\tcb@listing@uselistinglisting%
    \let\tcbusetemplisting\tcb@listing@usetemplisting%
    \let\tcb@doc@usetemplisting\tcb@listing@doc@usetemplisting},
  every listing line/.code={%
    \def\lst@NewLine{%
      \ifx\lst@OutputBox\@gobble\else
          \par\noindent \hbox{}#1%
      \fi
      \global\advance\lst@newlines\m@ne
      \lst@newlinetrue}},%
  every listing line*/.style={every listing line={#1},%
    code={\setbox\z@=\hbox{#1}\tcbdimto\kvtcb@rightupper{\kvtcb@rightupper+\wd\z@}}},%
}


\tcbset{%
  reset@listings/.style={%
    listing style=tcblatex,
    listing inputencoding=\inputencodingname,
    listing remove caption,
    listing engine=listings,
  },
  initialize@reset=reset@listings,
}



==> tcblistingscore.code.tex <==
%% The LaTeX package tcolorbox - version 3.90 (2016/02/29)
%% tcblistingscode.code.tex: Auxiliary code for colorboxes with listings
%%
%% -------------------------------------------------------------------------------------------
%% Copyright (c) 2006-2016 by Prof. Dr. Dr. Thomas F. Sturm <thomas dot sturm at unibw dot de>
%% -------------------------------------------------------------------------------------------
%%
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either version 1.3
%% of this license or (at your option) any later version.
%% The latest version of this license is in
%%   http://www.latex-project.org/lppl.txt
%% and version 1.3 or later is part of all distributions of LaTeX
%% version 2005/12/01 or later.
%%
%% This work has the LPPL maintenance status `author-maintained'.
%%
%% This work consists of all files listed in README
%%
%\makeatletter
\tcb@set@library@version{3.90}

\RequirePackage{pdftexcmds}

\def\tcbuselistingtext@input{\input{\kvtcb@listingfile}}%
\def\tcbuselistingtext{\tcbuselistingtext@input}%
\def\tcbuselistingcomment{\kvtcb@listingcomment}%
\def\tcb@listing@listing{\tcbuselistinglisting}

\def\tcb@listing@listingAndOther{%
   \tcbuselistinglisting%
   \tcblower%
   \tcb@use@listing@other%
}

\def\tcb@listing@otherAndListing{%
   \tcb@use@listing@other%
   \tcblower%
   \tcbuselistinglisting%
}

\newenvironment{tcb@lower@outside}[1]{%
  \tcbset{savedelimiter=tcb@lower@outside}\tcb@minipage{#1}%
  \color{tcbcol@lower}\kvtcb@fontlower\kvtcb@halignlower\kvtcb@before@lower\ignorespaces}%
%  {\unskip\kvtcb@after@lower\endminipage}
  {\kvtcb@after@lower\endminipage}

\def\tcb@use@listing@other@reset{%
  \tcbset{every box on layer 1/.style={reset,every box}}%
  \tcb@use@listing@other}

\def\tcb@use@lower@outside#1{%
  \setbox\z@=\hbox{\begin{tcb@lower@outside}{#1}%
    \tcb@use@listing@other@reset%
  \end{tcb@lower@outside}}%
  \tcbdimto{\tcb@temp@wd}{\wd\z@}%
  \unhbox\z@%
}

\def\tcb@inputlisting@out@otherAboveListing{%
  {\kvtcb@beforebox}\noindent%
  \iftcb@lowervisible%
    \tcb@use@lower@outside{\kvtcb@width}%
    \par\vskip-\parskip\vspace*{\kvtcb@middle}\noindent%
  \fi%
  \begin{tcolorbox}[before=,savedelimiter=tcolorbox]\tcbuselistinglisting\end{tcolorbox}%
}

\def\tcb@inputlisting@out@otherAboveListing@Decoupled{%
  \iftcb@lowervisible%
    {\par\tcb@use@listing@other@reset\par}%
  \fi%
  \begin{tcolorbox}[savedelimiter=tcolorbox]\tcbuselistinglisting\end{tcolorbox}%
}

\def\tcb@inputlisting@out@listingAboveOther{%
  \begin{tcolorbox}[after=,savedelimiter=tcolorbox]\tcbuselistinglisting\end{tcolorbox}%
  \iftcb@lowervisible\par\vskip-\parskip\vspace*{\kvtcb@middle}\noindent%
    \tcb@use@lower@outside{\kvtcb@width}%
  \fi%
  {\kvtcb@afterbox}%
}

\def\tcb@inputlisting@out@listingAboveOther@Decoupled{%
  \begin{tcolorbox}[savedelimiter=tcolorbox]\tcbuselistinglisting\end{tcolorbox}%
  \iftcb@lowervisible%
    {\par\tcb@use@listing@other@reset\par}%
  \fi%
}


\newenvironment{tcb@outside@environment}{%
  \tcb@before@unbroken%
  \begin{minipage}{\tcb@width}}%
{%
  \end{minipage}%
  \tcb@after@unbroken}

\def\tcb@inputlisting@out@prepare{%
  \tcbdimto\tcb@width{\kvtcb@width}%
  \tcbdimto\tcb@innerwidth{\tcb@width-\kvtcb@left@rule-\kvtcb@right@rule}%
  \tcbdimto\tcb@temp{\tcb@innerwidth-\kvtcb@boxsep*2}%
  \tcbdimto\tcb@w@upper{\tcb@temp-\kvtcb@leftupper-\kvtcb@rightupper}%
  \tcbset{breakable@false}%
  \def\tcb@minipage{\csname tcb@minipage@\kvtcb@sbs@align\endcsname}%
  \tcbdimto\tcb@w@upper@real{\tcb@w@upper}%
  \tcbdimto\tcb@w@sbs{\tcb@w@upper@real-\kvtcb@sbs@gap}%
  \tcb@sbs@quota%
  \ifx\kvtcb@float\@empty%
    \let\tcb@before@unbroken=\kvtcb@beforebox%
    \let\tcb@after@unbroken=\kvtcb@afterbox%
  \else%
    \edef\tcb@before@unbroken{\noexpand\tcb@float@env@begin{tcbfloat}[\kvtcb@float]}%
    \let\tcb@after@unbroken=\tcb@float@env@end%
  \fi%
}

\def\tcb@use@lower@outside@side#1{%
  \setbox\z@=\hbox{\begin{tcb@lower@outside}{#1}%
    \tcb@use@listing@other@reset%
  \end{tcb@lower@outside}}%
  \tcb@box@align\z@%
  \tcbdimto{\tcb@temp@wd}{\wd\z@}%
  \unhbox\z@%
}

\def\tcb@inputlisting@out@listingAndOther{%
  \tcb@inputlisting@out@prepare%
  \tcbdimto\tcb@w@outside{\tcb@w@lower}%
  \tcbdimto\tcb@w@inside{\tcb@width-\tcb@w@lower-\kvtcb@sbs@gap}%
  \begin{tcb@outside@environment}%
  \setbox\z@=\hbox{\tcb@minipage{\tcb@w@inside}%
  \begin{tcolorbox}[width=\tcb@w@inside,nobeforeafter,nofloat,sidebyside=false,savedelimiter=tcolorbox]\tcbuselistinglisting\end{tcolorbox}%
  \endminipage}%
  \tcb@box@align\z@%
  \unhbox\z@%
  \kern\kvtcb@sbs@gap%
  \iftcb@lowervisible%
    \tcb@use@lower@outside@side{\tcb@w@outside}%
  \fi%
  \end{tcb@outside@environment}%
}

\def\tcb@inputlisting@out@otherAndListing{%
  \tcb@inputlisting@out@prepare%
  \tcbdimto\tcb@w@outside{\tcb@w@upper}%
  \tcbdimto\tcb@w@inside{\tcb@width-\tcb@w@upper-\kvtcb@sbs@gap}%
  \begin{tcb@outside@environment}%
  \iftcb@lowervisible%
    \tcb@use@lower@outside@side{\tcb@w@outside}%
    \tcbdimto{\tcb@temp@wd}{\tcb@w@outside-\tcb@temp@wd+\kvtcb@sbs@gap}%
  \else%
    \tcbdimto{\tcb@temp@wd}{\tcb@w@outside+\kvtcb@sbs@gap}%
  \fi%
  \kern\tcb@temp@wd%
  \setbox\z@=\hbox{\tcb@minipage{\tcb@w@inside}%
  \begin{tcolorbox}[width=\tcb@w@inside,nobeforeafter,nofloat,sidebyside=false,savedelimiter=tcolorbox]\tcbuselistinglisting\end{tcolorbox}%
  \endminipage}%
  \tcb@box@align\z@%
  \unhbox\z@%
  \end{tcb@outside@environment}%
}

\def\tcb@inputlisting@inside{%
  \begin{tcolorbox}[capture=\tcb@listing@capture,savedelimiter=tcolorbox]\tcb@listing@process\end{tcolorbox}%
}

\long\def\tcb@run@system@command#1{%
  \ifcase\pdf@shellescape\relax
    \tcb@error{You must invoke LaTeX with the -shell-escape flag}{Pass the -shell-escape flag to LaTeX.}%
  \or\or
    \tcb@warning{System call with restricted shell escape may fail}%
  \fi%
  \filename@parse{\kvtcb@listingfile}\immediate\write18{#1}%
  \relax%
}


\tcbset{%
  listing file/.store in=\kvtcb@listingfile,%
  comment/.store in=\kvtcb@listingcomment,%
  listing@process@inside/.code 2 args={%
    \let\tcb@inputlisting\tcb@inputlisting@inside%
    \let\tcb@listing@process=#1%
    \let\tcb@use@listing@other=#2},%
  listing@process@outside/.code 2 args={%
    \let\tcb@inputlisting=#1%
    \let\tcb@use@listing@other=#2},%
  listing only/.style={listing@process@inside={\tcb@listing@listing}{\tcbuselistingtext}},%
  text only/.style={listing@process@inside={\tcbuselistingtext}{\tcbuselistingtext}},%
  comment only/.style={listing@process@inside={\tcbuselistingcomment}{\tcbuselistingcomment}},%
  listing and text/.style={listing@process@inside={\tcb@listing@listingAndOther}{\tcbuselistingtext}},%
  text and listing/.style={listing@process@inside={\tcb@listing@otherAndListing}{\tcbuselistingtext}},%
  text above listing/.style={listing@process@outside={\tcb@inputlisting@out@otherAboveListing}{\tcbuselistingtext}},%
  text above* listing/.style={listing@process@outside={\tcb@inputlisting@out@otherAboveListing@Decoupled}{\tcbuselistingtext}},%
  listing above text/.style={listing@process@outside={\tcb@inputlisting@out@listingAboveOther}{\tcbuselistingtext}},%
  listing above* text/.style={listing@process@outside={\tcb@inputlisting@out@listingAboveOther@Decoupled}{\tcbuselistingtext}},%
  text outside listing/.style={listing@process@outside={\tcb@inputlisting@out@otherAndListing}{\tcbuselistingtext}},%
  listing outside text/.style={listing@process@outside={\tcb@inputlisting@out@listingAndOther}{\tcbuselistingtext}},%
  text side listing/.style={sidebyside,text and listing},%
  listing side text/.style={sidebyside,listing and text},%
  listing and comment/.style={listing@process@inside={\tcb@listing@listingAndOther}{\tcbuselistingcomment}},%
  comment and listing/.style={listing@process@inside={\tcb@listing@otherAndListing}{\tcbuselistingcomment}},%
  comment above listing/.style={listing@process@outside={\tcb@inputlisting@out@otherAboveListing}{\tcbuselistingcomment}},%
  comment above* listing/.style={listing@process@outside={\tcb@inputlisting@out@otherAboveListing@Decoupled}{\tcbuselistingcomment}},%
  listing above comment/.style={listing@process@outside={\tcb@inputlisting@out@listingAboveOther}{\tcbuselistingcomment}},%
  listing above* comment/.style={listing@process@outside={\tcb@inputlisting@out@listingAboveOther@Decoupled}{\tcbuselistingcomment}},%
  comment outside listing/.style={listing@process@outside={\tcb@inputlisting@out@otherAndListing}{\tcbuselistingcomment}},%
  listing outside comment/.style={listing@process@outside={\tcb@inputlisting@out@listingAndOther}{\tcbuselistingcomment}},%
  comment side listing/.style={sidebyside,comment and listing},%
  listing side comment/.style={sidebyside,listing and comment},%
  listing engine/.is choice,%
  image comment/.style 2 args={comment={\includegraphics[#1]{#2}}},%
  comment style/.store in=\kvtcb@commentstyle,%
  tcbimage comment/.style={comment={\let\tcb@trans@commentstyle\kvtcb@commentstyle\tcbincludegraphics[code={\pgfkeysalsofrom\tcb@trans@commentstyle}]{#1}}},
  pdf extension/.store in=\kvtcb@pdf@extension,%
  pdf comment/.style={comment={\let\tcb@trans@commentstyle\kvtcb@commentstyle\filename@parse{#1}\edef\tcb@trans@commentfile{\filename@area\filename@base.\kvtcb@pdf@extension}%
    \begin{tcbraster}[raster halign=center,sharp corners,size=tight,colback=white,code={\pgfkeysalsofrom\tcb@trans@commentstyle}]\tcbincludepdf{\tcb@trans@commentfile}\end{tcbraster}}},
  pdf comment/.default={\kvtcb@listingfile},
  process code/.code={\appto\tcb@listing@process@hook{#1}},%
  no process/.code={\def\tcb@listing@process@hook{}},%
  compilable listing/.style={listing file={\jobname-listing-\thetcblistingcount}},
  run system command/.style={process code={\tcb@run@system@command{#1}}},%
  run@system@command/.style 2 args={run system command={#1\space#2\space\filename@area\filename@base}},%
  run pdflatex/.style={run@system@command={pdflatex}{#1}},%
  run xelatex/.style={run@system@command={xelatex}{#1}},%
  run lualatex/.style={run@system@command={lualatex}{#1}},%
  run makeindex/.style={run@system@command={makeindex}{#1}},%
  run bibtex/.style={run@system@command={bibtex}{#1}},%
  run biber/.style={run@system@command={biber}{#1}},%
  run arara/.style={run@system@command={arara}{#1}},%
  run latex/.style={run@system@command={latex}{#1}},%
  run dvips/.style={run@system@command={dvips}{#1}},%
  run ps2pdf/.style={run system command={ps2pdf\space#1\space\filename@area\filename@base.ps}},%
}

\def\tcbinputlisting@core{%
  \tcb@listing@process@hook%
  \let\tcb@listing@capture=\kvtcb@capture%
  \tcb@inputlisting%
}

\newcounter{tcblisting}

\newenvironment{tcblisting}[1]{%
  \stepcounter{tcblisting}\edef\thetcblistingcount{\thetcblisting}%
  \tcb@layer@pushup%
  \tcb@apply@box@options{capture=minipage,#1}%
  \begingroup\tcbverbatimwrite{\kvtcb@listingfile}%
}{\endtcbverbatimwrite\endgroup%
  \tcbinputlisting@core%
}

\long\def\tcbinputlisting#1{%
  \begingroup%
  \stepcounter{tcblisting}\edef\thetcblistingcount{\thetcblisting}%
  \tcb@layer@pushup%
  \tcb@apply@box@options{capture=minipage,#1}%
  \tcbinputlisting@core%
  \endgroup%
}

\newenvironment{tcboutputlisting}{%
  \begingroup\tcbverbatimwrite{\kvtcb@listingfile}%
}{\endtcbverbatimwrite\endgroup}

\long\def\tcb@newtcblisting#1#2{\tcb@newenvironment{#1}{\tcblisting{#2,options@for=#1}}{\endtcblisting}}

\long\def\tcb@newtcblisting@#1[#2]#3{\tcb@newenvironment{#1}[#2]{\tcblisting{#3,options@for=#1}}{\endtcblisting}}

\long\def\tcb@newtcblisting@@#1[#2][#3]#4{\tcb@newenvironment{#1}[#2][#3]{\tcblisting{#4,options@for=#1}}{\endtcblisting}}

\long\def\tcb@new@tcblisting@#1[#2]{%
  \@ifnextchar[{\tcb@newtcblisting@@{#1}[#2]}{\tcb@newtcblisting@{#1}[#2]}}

\def\tcb@new@tcblisting#1{%
  \@ifnextchar[{\tcb@new@tcblisting@{#1}}{\tcb@newtcblisting{#1}}}

\def\newtcblisting{%
  \let\tcb@newenvironment\newenvironment%
  \let\tcb@process@newtcolorbox@continue\tcb@new@tcblisting%
  \tcb@process@newenvironment}

\def\renewtcblisting{%
  \let\tcb@newenvironment\renewenvironment%
  \let\tcb@process@newtcolorbox@continue\tcb@new@tcblisting%
  \tcb@process@newenvironment}

\long\def\tcb@newtcbinputlisting#1#2{\expandafter\tcb@newcommand\csname#1\endcsname{\tcbinputlisting{#2,options@for=#1}}}

\long\def\tcb@newtcbinputlisting@#1[#2]#3{\expandafter\tcb@newcommand\csname#1\endcsname[#2]{\tcbinputlisting{#3,options@for=#1}}}

\long\def\tcb@newtcbinputlisting@@#1[#2][#3]#4{\expandafter\tcb@newcommand\csname#1\endcsname[#2][#3]{\tcbinputlisting{#4,options@for=#1}}}

\long\def\tcb@new@tcbinputlisting@#1[#2]{%
  \@ifnextchar[{\tcb@newtcbinputlisting@@{#1}[#2]}{\tcb@newtcbinputlisting@{#1}[#2]}}

\def\tcb@new@tcbinputlisting#1{%
  \@ifnextchar[{\tcb@new@tcbinputlisting@{#1}}{\tcb@newtcbinputlisting{#1}}}

\def\newtcbinputlisting{%
  \let\tcb@newcommand\newcommand%
  \let\tcb@process@newtcolorbox@continue\tcb@new@tcbinputlisting%
  \tcb@process@newcommand}

\def\renewtcbinputlisting{%
  \let\tcb@newcommand\renewcommand%
  \let\tcb@process@newtcolorbox@continue\tcb@new@tcbinputlisting%
  \tcb@process@newcommand}

\tcbset{%
  reset@listingscore/.style={%
    listing file=\jobname.listing,
    comment=, listing and text,
    no process,comment style=,pdf extension=pdf,
  },
  initialize@reset=reset@listingscore,
}



==> tcblistingsutf8.code.tex <==
%% The LaTeX package tcolorbox - version 3.90 (2016/02/29)
%% tcblistingsutf8.code.tex: Code for colorboxes with listings in UTF-8
%%
%% -------------------------------------------------------------------------------------------
%% Copyright (c) 2006-2016 by Prof. Dr. Dr. Thomas F. Sturm <thomas dot sturm at unibw dot de>
%% -------------------------------------------------------------------------------------------
%%
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either version 1.3
%% of this license or (at your option) any later version.
%% The latest version of this license is in
%%   http://www.latex-project.org/lppl.txt
%% and version 1.3 or later is part of all distributions of LaTeX
%% version 2005/12/01 or later.
%%
%% This work has the LPPL maintenance status `author-maintained'.
%%
%% This work consists of all files listed in README
%%
\tcb@set@library@version{3.90}

\RequirePackage{listingsutf8}[2011/11/10]
\tcbuselibrary{listings}

\tcbset{
  listing utf8/.style={listing inputencoding=utf8/#1},
}

\tcbset{%
  reset@listingsutf8/.style={listing utf8=latin1},
  initialize@reset=reset@listingsutf8,
}



==> tcbmagazine.code.tex <==
%% The LaTeX package tcolorbox - version 3.90 (2016/02/29)
%% tcbmagazine.code.tex: Code for box sets and magazine styles
%%
%% -------------------------------------------------------------------------------------------
%% Copyright (c) 2006-2016 by Prof. Dr. Dr. Thomas F. Sturm <thomas dot sturm at unibw dot de>
%% -------------------------------------------------------------------------------------------
%%
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either version 1.3
%% of this license or (at your option) any later version.
%% The latest version of this license is in
%%   http://www.latex-project.org/lppl.txt
%% and version 1.3 or later is part of all distributions of LaTeX
%% version 2005/12/01 or later.
%%
%% This work has the LPPL maintenance status `author-maintained'.
%%
%% This work consists of all files listed in README
%%
\tcb@set@library@version{3.90}

\tcbuselibrary{breakable}

\def\newboxarray#1{%
  \ifcsdef{tcb@boxarray@#1@allocated}{%
    \tcb@warning{box array '#1' is allocated again by \string\newboxarray. Memory and registers are wasted}%
  }{}%
  \global\csdef{tcb@boxarray@#1@size}{0}%
  \global\csdef{tcb@boxarray@#1@allocated}{0}%
}

\newboxarray{default}

\newrobustcmd*{\boxarraygetsize}[2][default]{%
  \letcs#2{tcb@boxarray@#1@size}%
  \ifdef{#2}{}{%
    \tcb@error{undefined box array '#1'}%
    {You have to say \string\newboxarray{#1}, before '#1' can be used as box array.}%
  }%
}

\newrobustcmd*{\boxarrayreset}[1][default]{%
  \boxarraygetsize[#1]\tcb@box@array@size%
  \global\csdef{tcb@boxarray@#1@size}{0}%
}

\newrobustcmd*{\boxarrayclear}[1][default]{%
  \boxarraygetsize[#1]\tcb@box@array@size%
  \global\csdef{tcb@boxarray@#1@size}{0}%
  \letcs\tcb@box@array@allocated{tcb@boxarray@#1@allocated}%
  \begingroup%
    \count@=0%
    \loop%
    \ifnum\count@<\tcb@box@array@allocated\relax%
      \advance\count@ 1\relax%
      \letcs\tcb@box@array@box{tcb@boxarray@#1@\number\count@ @box}%
      \setbox0=\box\tcb@box@array@box%
    \repeat%
  \endgroup%
}

\newrobustcmd*{\boxarraygetbox}[3][default]{%
  \boxarraygetsize[#1]\tcb@box@array@size%
  \let#2\@undefined%
  \ifnum\numexpr#3>0\relax%
    \ifnum\numexpr#3>\tcb@box@array@size\relax%
    \else%
      \letcs#2{tcb@boxarray@#1@#3@box}%
    \fi%
  \fi%
}

\newrobustcmd*{\boxarraygetwidth}[3][default]{%
  \boxarraygetbox[#1]{\tcb@box@array@box}{#3}%
  \ifdefined\tcb@box@array@box%
    \tcbdimto#2{\wd\tcb@box@array@box}%
  \else%
    \let#2\tcb@zpt%
  \fi%
}

\newrobustcmd*{\boxarraygetheight}[3][default]{%
  \boxarraygetbox[#1]{\tcb@box@array@box}{#3}%
  \ifdefined\tcb@box@array@box%
    \tcbdimto#2{\ht\tcb@box@array@box}%
  \else%
    \let#2\tcb@zpt%
  \fi%
}

\newrobustcmd*{\boxarraygetdepth}[3][default]{%
  \boxarraygetbox[#1]{\tcb@box@array@box}{#3}%
  \ifdefined\tcb@box@array@box%
    \tcbdimto#2{\dp\tcb@box@array@box}%
  \else%
    \let#2\tcb@zpt%
  \fi%
}

\newrobustcmd*{\boxarraygettotalheight}[3][default]{%
  \boxarraygetbox[#1]{\tcb@box@array@box}{#3}%
  \ifdefined\tcb@box@array@box%
    \tcbdimto#2{\ht\tcb@box@array@box+\dp\tcb@box@array@box}%
  \else%
    \let#2\tcb@zpt%
  \fi%
}

\newrobustcmd*{\useboxarray}[2][default]{%
  \boxarraygetbox[#1]{\tcb@box@array@box}{#2}%
  \ifdefined\tcb@box@array@box%
    \usebox{\tcb@box@array@box}%
  \fi%
}

\newrobustcmd{\usetcboxarray}[3][default]{%
  \boxarraygetbox[#1]{\tcb@box@array@box}{#2}%
  \ifdefined\tcb@box@array@box%
    \tcbox[#3]{\usebox{\tcb@box@array@box}}%
  \fi%
}

\newrobustcmd*{\consumeboxarray}[2][default]{%
  \boxarraygetbox[#1]{\tcb@box@array@box}{#2}%
  \ifdefined\tcb@box@array@box%
    \leavevmode\box\tcb@box@array@box\relax%
  \fi%
}

\newrobustcmd{\consumetcboxarray}[3][default]{%
  \boxarraygetbox[#1]{\tcb@box@array@box}{#2}%
  \ifdefined\tcb@box@array@box%
    \tcbox[#3]{\leavevmode\box\tcb@box@array@box\relax}%
  \fi%
}

\def\boxarraystore#1{%
  \boxarraygetsize[#1]\tcb@box@array@size%
  \numdef\tcb@box@array@size{\tcb@box@array@size+1}%
  \global\cslet{tcb@boxarray@#1@size}{\tcb@box@array@size}%
  \letcs\tcb@box@array@allocated{tcb@boxarray@#1@allocated}%
  \ifnum\tcb@box@array@allocated<\tcb@box@array@size\relax%
    \newbox\tcb@box@array@box\csxdef{tcb@boxarray@#1@\tcb@box@array@size @box}{\the\tcb@box@array@box}%
    \global\cslet{tcb@boxarray@#1@allocated}{\tcb@box@array@size}%
  \else%
    \letcs\tcb@box@array@box{tcb@boxarray@#1@\tcb@box@array@size @box}%
  \fi%
  \edef\reserved@a{%
    \endgroup
    \global\setbox\tcb@box@array@box\hbox{%
      \begingroup\aftergroup}%
        \def\noexpand\@currenvir{\@currenvir}%
        \def\noexpand\@currenvline{\on@line}}%
  \reserved@a
    \@endpefalse
    \color@setgroup
      \ignorespaces}

\def\endboxarraystore{\unskip\color@endgroup}

\def\tcb@storetoboxarray@begin#1#2[#3]{\begin{boxarraystore}{#1}}
\def\tcb@storetoboxarray@end{\end{boxarraystore}}

\tcbset{
  store to box array/.code={%
    \def\kvtcb@float{S}\def\tcb@float@env@begin{\tcb@storetoboxarray@begin{#1}}\def\tcb@float@env@end{\tcb@storetoboxarray@end}},
  store to box array/.default=default,
  reset box array/.code={\boxarrayreset[#1]},
  reset box array/.default=default,
  reset and store to box array/.style={reset box array={#1},store to box array={#1}},%
  reset and store to box array/.default=default,
  do not store to box array/.style={nofloat},
}



==> tcbminted.code.tex <==
%% The LaTeX package tcolorbox - version 3.90 (2016/02/29)
%% tcbminted.code.tex: Code for colorboxes with listings
%%
%% -------------------------------------------------------------------------------------------
%% Copyright (c) 2006-2016 by Prof. Dr. Dr. Thomas F. Sturm <thomas dot sturm at unibw dot de>
%% -------------------------------------------------------------------------------------------
%%
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either version 1.3
%% of this license or (at your option) any later version.
%% The latest version of this license is in
%%   http://www.latex-project.org/lppl.txt
%% and version 1.3 or later is part of all distributions of LaTeX
%% version 2005/12/01 or later.
%%
%% This work has the LPPL maintenance status `author-maintained'.
%%
%% This work consists of all files listed in README
%%
%\makeatletter
\tcb@set@library@version{3.90}

\RequirePackage{minted}[2011/09/17]

\tcbuselibrary{listings@core}

\def\tcb@minted@input@listing#1#2#3#4{%
  \edef\temp@a{#4}%
  \ifx\temp@a\@empty%
  \else
    %\usemintedstyle{\temp@a}%
    \toks@=\expandafter{#4}%
    \edef\tcb@temp{\noexpand\usemintedstyle{\the\toks@}}%
    \tcb@temp%
  \fi%
  \toks@=\expandafter{#1}%
  \edef\tcb@temp{\noexpand\inputminted[\the\toks@]}%
  \tcb@temp{#2}{#3}%
}

\def\tcb@minted@uselistinglisting{%
  \tcb@minted@input@listing{\kvtcb@minted@options}{\kvtcb@minted@language}{\kvtcb@listingfile}{\kvtcb@minted@style}%
}%

\def\tcb@minted@usetemplisting{%
  \tcb@minted@input@listing{\kvtcb@minted@options}{\kvtcb@minted@language}{\kvtcb@tempfile}{\kvtcb@minted@style}%
}%

\def\tcb@minted@doc@usetemplisting{%
  \tcb@minted@input@listing{\kvtcb@docmintoptions}{latex}{\kvtcb@tempfile}{\kvtcb@docmintstyle}%
}

\tcbset{%
  minted language/.store in=\kvtcb@minted@language,
  minted options/.store in=\kvtcb@minted@options,
  minted style/.store in=\kvtcb@minted@style,
  listing engine/minted/.code={\let\tcbuselistinglisting\tcb@minted@uselistinglisting%
    \let\tcbusetemplisting\tcb@minted@usetemplisting%
    \let\tcb@doc@usetemplisting\tcb@minted@doc@usetemplisting},
}


\tcbset{%
  reset@minted/.style={%
    minted language=latex,
    minted options={tabsize=2,fontsize=\small},
    minted style=,
    listing engine=minted,
  },
  initialize@reset=reset@minted,
}



==> tcbraster.code.tex <==
%% The LaTeX package tcolorbox - version 3.90 (2016/02/29)
%% tcbskinsjigsaw.code.tex: Code for colorboxes with different skins
%%
%% -------------------------------------------------------------------------------------------
%% Copyright (c) 2006-2016 by Prof. Dr. Dr. Thomas F. Sturm <thomas dot sturm at unibw dot de>
%% -------------------------------------------------------------------------------------------
%%
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either version 1.3
%% of this license or (at your option) any later version.
%% The latest version of this license is in
%%   http://www.latex-project.org/lppl.txt
%% and version 1.3 or later is part of all distributions of LaTeX
%% version 2005/12/01 or later.
%%
%% This work has the LPPL maintenance status `author-maintained'.
%%
%% This work consists of all files listed in README
%%
\tcb@set@library@version{3.90}

\newcounter{tcbrastercolumn}
\newcounter{tcbrasterrow}
\newcounter{tcbraster}

\newrobustcmd{\thetcbrasternum}{\the\numexpr(\c@tcbrasterrow-1)*\kvtcb@raster@columns+\c@tcbrastercolumn\relax}

\def\tcb@raster@ehg@all{%
  \tcbset{equal height group={\kvtcb@raster@ehgid}}%
}

\def\tcb@raster@ehg@row{%
  \tcbset{equal height group={\kvtcb@raster@ehgid @\number\c@tcbrasterrow}}%
}


\tcbset{%
  raster columns/.store in=\kvtcb@raster@columns,
  raster rows/.store in=\kvtcb@raster@rows,
  raster width/.store in=\kvtcb@raster@width,
  raster height/.store in=\kvtcb@raster@height,
  %
  raster before skip/.store in=\kvtcb@raster@skip@before,
  raster after skip/.store in=\kvtcb@raster@skip@after,
  raster left skip/.store in=\kvtcb@raster@skip@left,
  raster right skip/.store in=\kvtcb@raster@skip@right,
  %
  raster column skip/.store in=\kvtcb@raster@xskip,
  raster row skip/.store in=\kvtcb@raster@yskip,
  %
  raster equal skip/.style={raster before skip=#1,raster after skip=#1,
    raster column skip=#1,raster row skip=#1},
  %
  raster@halign/.store in=\kvtcb@raster@halign,
  raster halign/.is choice,
  raster halign/center/.style={raster@halign=\centering},
  raster halign/left/.style={raster@halign=\raggedright},
  raster halign/right/.style={raster@halign=\raggedleft},
  %
  raster valign/.store in=\kvtcb@raster@valign,
  %
  raster equal height group/.store in=\kvtcb@raster@ehgid,%
  raster equal height/.is choice,
  raster equal height/.default=all,
  raster equal height/none/.code={\let\tcb@raster@ehg@start\@empty%
    \let\tcb@raster@ehg@continue\@empty},%
  raster equal height/rows/.code={\let\tcb@raster@ehg@start\tcb@raster@ehg@row%
    \let\tcb@raster@ehg@continue\tcb@raster@ehg@row},%
  raster equal height/all/.code={\let\tcb@raster@ehg@start\tcb@raster@ehg@all%
    \let\tcb@raster@ehg@continue\@empty},%
  %
  raster force size/.is choice,%
  raster force size/.default=true,%
  raster force size/true/.code={\let\tcb@raster@set@size\tcbset@late@options},%
  raster force size/false/.code={\let\tcb@raster@set@size\tcbset},%
  raster multicolumn/.code={%
    \ifnum\numexpr\c@tcbrastercolumn+#1>\numexpr\kvtcb@raster@columns+1\relax
      \tcb@warning{'raster multicolumn' combined too much columns}%
    \else%
      \tcbset@late@options{%
        code={\preto\kvtcb@afterbox{\addtocounter{tcbrastercolumn}{\numexpr#1-1}}},
        width=(\tcb@raster@box@width+\kvtcb@raster@xskip)*#1-\kvtcb@raster@xskip}%
    \fi%
  },
  raster multirow/.code={%
    \ifdefined\tcb@raster@box@height%
      \tcbset@late@options{%
        height=(\tcb@raster@box@height+\kvtcb@raster@yskip)*#1-\kvtcb@raster@yskip}%
    \else%
      \tcb@warning{'raster multirow' needs a fixed 'raster height'}%
    \fi%
  },
}

\tcbset{
  raster reset/.style={
    raster width=\linewidth,raster height=0pt,
    raster equal skip=2mm,
    raster columns=2,raster rows=2,
    raster left skip=0pt,raster right skip=0pt,
    raster halign=left,raster valign=center,
    raster equal height=none,
    raster equal height group={REG@\tcb@raster@number},
    raster force size,},
  raster reset
}

\setcounter{tcbraster}{0}

\let\tcb@raster@change@minipage\@empty
\let\tcb@raster@change@fitbox\@empty
\def\tcb@raster@change@hbox{\tcbset{capture=minipage}}

\def\tcb@height@fill@unbroken@raster#1{%
  \ifnum\c@tcblayer<2\relax%
    \kvtcb@beforebox%
    \def\kvtcb@beforebox{}%
    \tcb@breakat@init%
    \tcbset{compress page=#1}%
    \tcb@comp@h@page%
    \ifdim\tcb@h@page<0pt\relax\unkern\pagebreak\tcb@comp@h@page\kern\kvtcb@raster@skip@left\fi%
    \tcbset{height=\tcb@h@page-\kvtcb@bbtop@stand-\kvtcb@bbbottom@stand}%
  \fi%
}

\newenvironment{tcbraster}[1][]{%
  \tcb@layer@pushup%
  \stepcounter{tcbraster}%
  \edef\tcb@raster@number{\number\c@tcbraster}%
  \edef\tcb@raster@save@column{\number\c@tcbrastercolumn}%
  \edef\tcb@raster@save@row{\number\c@tcbrasterrow}%
  \let\tcb@raster@change@fitbox\@empty%
  \setcounter{tcbrastercolumn}{1}%
  \setcounter{tcbrasterrow}{1}%
  \let\tcb@height@fill@unbroken\tcb@height@fill@unbroken@raster%
  \tcbset{every box on layer \the\numexpr\number\c@tcblayer+1\relax/.code={%
    \tcbset{raster every box/.try}%
    \ifodd\c@tcbrastercolumn\relax%
      \tcbset{raster odd column/.try}%
    \else%
      \tcbset{raster even column/.try}%
    \fi%
    \tcbset{raster column \number\c@tcbrastercolumn/.try}%
    \ifodd\c@tcbrasterrow\relax%
      \tcbset{raster odd row/.try}%
    \else%
      \tcbset{raster even row/.try}%
    \fi%
    \tcbset{raster row \number\c@tcbrasterrow/.try}%
    \ifodd\thetcbrasternum\relax%
      \tcbset{raster odd number/.try}%
    \else%
      \tcbset{raster even number/.try}%
    \fi%
    \tcbset{raster row \number\c@tcbrasterrow\space column \number\c@tcbrastercolumn/.try}%
    \tcbset{raster number \thetcbrasternum/.try}%
  }}%
  \tcbset{#1}%
  \tcbset@late@options{%
    before={\ifhmode\unskip\fi\ifnum\c@tcbrastercolumn>1 \kern\kvtcb@raster@xskip\else%
      \ifnum\c@tcbrasterrow>1 \parindent\z@\parskip\z@\par\nointerlineskip\addvspace{\the\dimexpr\kvtcb@raster@yskip\relax}\noindent\fi%
      \kern\kvtcb@raster@skip@left\fi},
    after={%
      \ifnum\c@tcbrastercolumn=\kvtcb@raster@columns\relax%
        \kern\kvtcb@raster@skip@right%
        \setcounter{tcbrastercolumn}{1}\addtocounter{tcbrasterrow}{1}%
        \aftergroup\tcb@raster@ehg@continue%
      \else%
        \stepcounter{tcbrastercolumn}%
      \fi},%
    box align=\kvtcb@raster@valign,%
  }%
  \tcbdimto\tcb@raster@box@width{(\kvtcb@raster@width+\kvtcb@raster@xskip-\kvtcb@raster@skip@left-\kvtcb@raster@skip@right)/\kvtcb@raster@columns-\kvtcb@raster@xskip}%
  \tcb@raster@set@size{%
    code={\csuse{tcb@raster@change@\kvtcb@capture}},
    width=\tcb@raster@box@width,
  }%
  \ifdim\dimexpr\kvtcb@raster@height>0pt\relax%
    \tcbdimto\tcb@raster@box@height{(\kvtcb@raster@height+\kvtcb@raster@yskip-0.001pt)/\kvtcb@raster@rows-\kvtcb@raster@yskip}%
    \tcb@raster@set@size{height=\tcb@raster@box@height}%
  \fi%
  \tcb@raster@ehg@start%
  \let\tcb@end@raster\@empty%
  \ifinner\ifhmode%
    \color@vbox%
    \hsize=\kvtcb@raster@width%
    \let\tcb@end@raster\color@endbox%
  \fi\fi%&
  \if@nobreak%
    \iftcb@ignorenobreak%
      {\par\nointerlineskip%
      \addvspace{\glueexpr\kvtcb@raster@skip@before-\parskip}}%
    \fi%
  \else%
    {\par\nointerlineskip%
    \addvspace{\glueexpr\kvtcb@raster@skip@before-\parskip}}%
  \fi%
  \kvtcb@raster@halign\noindent%
}{%
  \ifhmode\unskip\fi%
  \ifnum\c@tcbrastercolumn>1 %
    \kern\kvtcb@raster@skip@right%
  \fi%
  \begingroup%
  \par\nointerlineskip%
  \addvspace{\glueexpr\kvtcb@raster@skip@after-\parskip}%
  \endgroup%
  \tcb@end@raster%
  \setcounter{tcbrastercolumn}{\tcb@raster@save@column}%
  \setcounter{tcbrasterrow}{\tcb@raster@save@row}%
}

\newcommand{\tcbitem@following}[1][]{%
  \end{tcolorbox}\begin{tcolorbox}[#1]%
}

\newcommand{\tcbitem@first}[1][]{%
  \let\tcbitem=\tcbitem@following%
  \begin{tcolorbox}[#1]%
}

\newenvironment{tcbitemize}[1][]{%
  \begin{tcbraster}[#1]%
  \let\tcb@raster@change@fitbox=\tcb@raster@change@hbox%
  \let\tcbitem=\tcbitem@first%
}{\end{tcolorbox}\end{tcbraster}}

\newenvironment{tcboxedraster}[2][]{%
  \tcolorbox[#2]\tcbraster[#1]}%
  {\endtcbraster\endtcolorbox}


==> tcbskins.code.tex <==
%% The LaTeX package tcolorbox - version 3.90 (2016/02/29)
%% tcbskins.code.tex: Code for colorboxes with different skins
%%
%% -------------------------------------------------------------------------------------------
%% Copyright (c) 2006-2016 by Prof. Dr. Dr. Thomas F. Sturm <thomas dot sturm at unibw dot de>
%% -------------------------------------------------------------------------------------------
%%
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either version 1.3
%% of this license or (at your option) any later version.
%% The latest version of this license is in
%%   http://www.latex-project.org/lppl.txt
%% and version 1.3 or later is part of all distributions of LaTeX
%% version 2005/12/01 or later.
%%
%% This work has the LPPL maintenance status `author-maintained'.
%%
%% This work consists of all files listed in README
%%
\tcb@set@library@version{3.90}

\RequirePackage{tikz}[2010/10/13]

\newenvironment{tikzpicture@tcb@hooked}{%
  \edef\tcb@tikzpicture@begin{\noexpand\tikzpicture[\expandonce\tcb@tikz@option@hook]}%
  \tcb@tikzpicture@begin\tcb@tikz@begin@hook}{\tcb@tikz@end@hook\endtikzpicture}

\def\tcb@creategeonodes@true{%
  \begin{scope}[every node/.style={line width=0mm,inner sep=0mm,outer sep=0mm,draw=none,fill=none,rectangle}]
    \node[name=frame,at={(0,0)},above right,minimum width=\tcb@width,minimum height=\tcb@height]{};
    \node[name=interior,at={({\kvtcb@left@rule},{\kvtcb@bottom@rule})},above right,minimum width=\tcb@innerwidth,minimum height=\tcb@innerheight]{};
    \ifnum\tcb@segment@state=1%
    \node[name=segmentation,at={({\kvtcb@left@rule},{\the\dimexpr\kvtcb@bottom@rule+\kvtcb@boxsep*2+\tcb@break@bottomsep+\kvtcb@bottom+\tcb@height@lower\relax})},above right,
       minimum width=\tcb@innerwidth,minimum height=\the\dimexpr\kvtcb@middle*2\relax]{};
    \else\iftcb@sidebyside%
    \node[name=segmentation,at={({\the\dimexpr\kvtcb@left@rule+\kvtcb@boxsep+\kvtcb@leftupper+\tcb@w@upper\relax},{\the\dimexpr\kvtcb@bottom@rule\relax})},above right,
       minimum width=\the\dimexpr\kvtcb@sbs@gap\relax,minimum height=\tcb@innerheight]{};
    \fi\fi%
    \iftcb@hasTitle%
    \node[name=title,at={({\kvtcb@left@rule},{\the\dimexpr\kvtcb@bottom@rule+\tcb@innerheight+\kvtcb@title@rule\relax})},above right,
       minimum width=\tcb@innerwidth,minimum height=\the\dimexpr\tcb@h@title+\kvtcb@toptitle+\kvtcb@bottomtitle+\kvtcb@boxsep*2\relax]{};
    \fi%
    \tcb@specialgeonodes@hook%
  \end{scope}%
}

\def\tcbsettowidthofnode#1#2{%
  \pgfpointanchor{#2}{east}\unskip%
  #1\pgf@x%
  \pgfpointanchor{#2}{west}\unskip%
  \advance #1 by -\pgf@x\relax%
}

\def\tcbsetmacrotowidthofnode#1#2{%
  \tcbsettowidthofnode\pgf@xa{#2}%
  \edef#1{\the\pgf@xa}%
}

\def\tcbsettoheightofnode#1#2{%
  \pgfpointanchor{#2}{north}\unskip%
  #1\pgf@y%
  \pgfpointanchor{#2}{south}\unskip%
  \advance #1 by -\pgf@y\relax%
}

\def\tcbsetmacrotoheightofnode#1#2{%
  \tcbsettoheightofnode\pgf@ya{#2}%
  \edef#1{\the\pgf@ya}%
}

\def\tcb@spec#1{\tikzset{tcb@spec/.style={#1}}}

\def\tcb@gettikzxy#1#2#3{%
  \tikz@scan@one@point\pgfutil@firstofone#1\relax%
  \edef#2{\the\pgf@x}%
  \edef#3{\the\pgf@y}%
}

\def\tcb@boundary@tikzbase#1#2#3#4#5#6{%
  \tcb@gettikzxy{(#1)}{\tcb@xa}{\tcb@ya}%
  \tcb@gettikzxy{(#2)}{\tcb@xb}{\tcb@yb}%
  \pgfpathmoveto{\pgfqpoint{\tcb@xa}{\tcb@ya}}%
  #4\pgfpathlineto{\pgfqpoint{\tcb@xa}{\tcb@yb}}%
  #5\pgfpathlineto{\pgfqpoint{\tcb@xb}{\tcb@yb}}%
  #6\pgfpathlineto{\pgfqpoint{\tcb@xb}{\tcb@ya}}%
  #3\pgfpathclose%
}

\def\tcb@pathboundary#1#2{\path[#1]\pgfextra{#2};}

\def\tcb@pathbase#1#2#3#4#5#6#7{\tcb@pathboundary{#1}{\tcb@boundary@tikzbase{#2}{#3}{#4}{#5}{#6}{#7}}}

\def\tcb@boundaryframe@pathfirst{%
  \tcb@boundary@base{0pt}{0pt}%
    {\tcb@width}{\tcb@height}%
    {\tcb@arc@zpt}{\tcb@arc@out@NW}{\tcb@arc@out@NE}{\tcb@arc@zpt}%
}

\def\tcb@boundaryframe@pathmiddle{%
  \tcb@boundary@base{0pt}{0pt}%
    {\tcb@width}{\tcb@height}%
    {\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}%
}

\def\tcb@boundaryframe@pathlast{%
  \tcb@boundary@base{0pt}{0pt}%
    {\tcb@width}{\tcb@height}%
    {\tcb@arc@out@SW}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@out@SE}%
}

\tikzset{%
  tcb fill frame/.style={fill=tcbcol@frame,fill opacity=\kvtcb@opacityframe,tcb@spec,frame@style},%
  tcb fill interior/.style={fill=tcbcol@back,fill opacity=\kvtcb@opacityback,tcb@spec,interior@style},%
  tcb fill title/.style={fill=tcbcol@backtitle,fill opacity=\kvtcb@opacitybacktitle,tcb@spec,title@style},%
}

% fill frame
\def\tcb@drawframe@path{\tcb@pathboundary{tcb fill frame}{\tcb@outerboundary}}
\let\tcb@drawframe@pathfirst=\tcb@drawframe@path
\let\tcb@drawframe@pathmiddle=\tcb@drawframe@path
\let\tcb@drawframe@pathlast=\tcb@drawframe@path


% fill inner box with title
\def\tcb@drawwithtitle@path{\tcb@pathboundary{tcb fill interior}{\tcb@boundaryinterior@title@standard}}

\def\tcb@drawwithtitle@pathfirst{%
  \tcb@pathbase{tcb fill interior}{interior.west|-frame.south}{interior.north east}%
    {\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}%
}

\let\tcb@drawwithtitle@pathmiddle=\tcb@drawwithtitle@pathfirst

\let\tcb@drawwithtitle@pathlast=\tcb@drawwithtitle@path

% fill inner box without title
\def\tcb@drawwithouttitle@path{\tcb@pathboundary{tcb fill interior}{\tcb@boundaryinterior@notitle@standard}}

\def\tcb@drawwithouttitle@pathfirst{%
  \tcb@pathbase{tcb fill interior}{interior.west|-frame.south}{interior.north east}%
    {\tcb@arc@zpt}{\tcb@arc@ins@NW}{\tcb@arc@ins@NE}{\tcb@arc@zpt}%
}

\def\tcb@drawwithouttitle@pathmiddle{%
  \tcb@pathbase{tcb fill interior}{interior.west|-frame.south}{interior.east|-frame.north}%
    {\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}%
}

\def\tcb@drawwithouttitle@pathlast{%
  \tcb@pathbase{tcb fill interior}{interior.south west}{interior.east|-frame.north}%
    {\tcb@arc@ins@SW}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@ins@SE}%
}

% draw title box
\def\tcb@drawtitle@path{\tcb@pathboundary{tcb fill title}{\tcb@boundarytitle@standard}}

\let\tcb@drawtitle@pathfirst=\tcb@drawtitle@path

\def\tcb@drawtitle@pathmiddle{%
  \tcb@pathbase{tcb fill title}{title.south west}{title.north east}%
    {\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}%
}

\let\tcb@drawtitle@pathlast=\tcb@drawtitle@pathmiddle

% draw segmentation line
\def\tcb@drawlower@path{%
  \iftcb@sidebyside%
    \path[draw=tcbcol@frame,fill opacity=\kvtcb@opacityframe,dash pattern=on 1mm off 1mm,dash phase=0.5mm,tcb@spec,segmentation@style]
    (segmentation.north)--(segmentation.south);%
  \else%
    \path[draw=tcbcol@frame,fill opacity=\kvtcb@opacityframe,dash pattern=on 1mm off 1mm,dash phase=0.5mm,tcb@spec,segmentation@style]
    (segmentation.west)--(segmentation.east);%
  \fi%
}

\def\tcb@draw@pseudo@segmentation#1{%
\begingroup\tcb@shield@externalize\begin{tikzpicture}%
  \path[use as bounding box] (0,{\the\dimexpr-\kvtcb@middle-\kvtcb@boxsep\relax})
     rectangle (\linewidth,{\the\dimexpr\kvtcb@middle+\kvtcb@boxsep\relax});
  \node[line width=0mm,inner sep=0mm,draw=none,fill=none,rectangle,
        name=segmentation,at={({\the\dimexpr-\kvtcb@boxsep-(#1)\relax},0)},right,%
        minimum width=\tcb@innerwidth,minimum height=\the\dimexpr\kvtcb@middle*2\relax]{};
  \tcb@drawlower@path%
\end{tikzpicture}\endgroup}

\def\tcbline@star#1{%
{\parskip\z@\par\nointerlineskip}%
\xleaders\vbox{\tcb@draw@pseudo@segmentation{#1}}\vskip\dimexpr(\kvtcb@middle+\kvtcb@boxsep)*2\relax%
{\parskip\z@\par\nointerlineskip}}

\def\tcbline@#1{%
{\parskip\z@\par\nointerlineskip}%
\tcb@draw@pseudo@segmentation{#1}%
{\parskip\z@\par\nointerlineskip}}

\def\tcbline{%
  \@ifstar{\iftcb@hasLower\tcbline@star{\kvtcb@leftlower}\else\tcbline@star{\kvtcb@leftupper}\fi}%
  {\iftcb@hasLower\tcbline@{\kvtcb@leftlower+\@totalleftmargin}\else\tcbline@{\kvtcb@leftupper+\@totalleftmargin}\fi}}


% draw special versions
\def\tcb@drawspec@UT{%
  \tcb@pathbase{tcb fill interior}{segmentation.west}{interior.north east}%
    {\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}%
}

\def\tcb@drawspec@UR{%
  \tcb@pathbase{tcb fill interior}{segmentation.west}{interior.north east}%
    {\tcb@arc@zpt}{\tcb@arc@ins@NW}{\tcb@arc@ins@NE}{\tcb@arc@zpt}%
}

\def\tcb@drawspec@US{%
  \tcb@pathbase{tcb fill interior}{segmentation.west}{interior.east|-frame.north}%
    {\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}%
}

\def\tcb@drawspec@LR#1{%
  \tcb@pathbase{#1,segmentation@style}{interior.south west}{[yshift=0.1mm]segmentation.east}%
    {\tcb@arc@ins@SW}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@ins@SE}%
}

\def\tcb@drawspec@LS#1{%
  \tcb@pathbase{#1,segmentation@style}{interior.west|-frame.south}{[yshift=0.1mm]segmentation.east}%
    {\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}%
}

\def\tcb@drawspec@sbs@A#1{%
  \tcb@pathbase{#1,segmentation@style}{segmentation.south}{interior.north east}%
    {\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@ins@NE}{\tcb@arc@ins@SE}%
}

\def\tcb@drawspec@sbs@B#1{%
  \tcb@pathbase{#1,segmentation@style}{segmentation.south}{interior.north east}%
    {\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@ins@SE}%
}

\def\tcb@drawspec@sbs@C#1{%
  \tcb@pathbase{#1,segmentation@style}{segmentation.south|-frame.south}{interior.north east}%
    {\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@ins@NE}{\tcb@arc@zpt}%
}

\def\tcb@drawspec@sbs@D#1{%
  \tcb@pathbase{#1,segmentation@style}{segmentation.south|-frame.south}{interior.north east}%
    {\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}%
}

\def\tcb@drawspec@sbs@E#1{%
  \tcb@pathbase{#1,segmentation@style}{segmentation.south|-frame.south}{interior.east|-frame.north}%
  {\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}%
}

\def\tcb@drawspec@sbs@F#1{%
  \tcb@pathbase{#1,segmentation@style}{segmentation.south}{interior.east|-frame.north}%
  {\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@ins@SE}%
}

\def\tcb@drawspec@T{%
  \tcb@pathbase{top color=tcbcol@frame,bottom color=tcbcol@back,fill opacity=\kvtcb@opacitybacktitle}{[yshift=-0.01pt]interior.north west}{[yshift=0.01pt]title.south east}%
  {\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}%
}

\def\tcb@drawframe@freelance{\tcb@frame@code}
\def\tcb@drawwithtitle@freelance{\tcb@interiortitled@code}
\def\tcb@drawwithouttitle@freelance{\tcb@interior@code}
\def\tcb@drawlower@freelance{\tcb@segmentation@code}
\def\tcb@drawtitle@freelance{\tcb@title@code}


\def\tcb@drawframe@spartan{%
  \begin{pgfscope}%
  \pgfpathrectangle{\pgfpointorigin}{\pgfqpoint{\tcb@width}{\tcb@height}}%
  \pgfsetfillcolor{tcbcol@frame}%
  \pgfsetfillopacity{\kvtcb@opacityframe}%
  \pgfusepath{fill}%
  \end{pgfscope}%
}

\def\tcb@drawwithtitle@spartan{%
  \begin{pgfscope}%
  \pgfpathrectanglecorners{\pgfqpoint{\kvtcb@left@rule}{\kvtcb@bottom@rule}}%
   {\pgfqpoint{\the\dimexpr\tcb@width-\kvtcb@right@rule\relax}{\the\dimexpr\kvtcb@bottom@rule+\tcb@innerheight\relax}}%
  \pgfsetfillcolor{tcbcol@back}%
  \pgfsetfillopacity{\kvtcb@opacityback}%
  \pgfusepath{fill}%
  \end{pgfscope}%
}

\def\tcb@drawwithouttitle@spartan{%
  \begin{pgfscope}%
  \pgfpathrectanglecorners{\pgfqpoint{\kvtcb@left@rule}{\kvtcb@bottom@rule}}%
   {\pgfqpoint{\the\dimexpr\tcb@width-\kvtcb@right@rule\relax}{\the\dimexpr\tcb@height-\kvtcb@top@rule\relax}}%
  \pgfsetfillcolor{tcbcol@back}%
  \pgfsetfillopacity{\kvtcb@opacityback}%
  \pgfusepath{fill}%
  \end{pgfscope}%
}

\def\tcb@drawtitle@spartan{%
  \begin{pgfscope}%
  \pgfpathrectanglecorners{\pgfqpoint{\kvtcb@left@rule}{\the\dimexpr\kvtcb@bottom@rule+\tcb@innerheight+\kvtcb@title@rule\relax}}%
   {\pgfqpoint{\the\dimexpr\tcb@width-\kvtcb@right@rule\relax}{\the\dimexpr\tcb@height-\kvtcb@top@rule\relax}}%
  \pgfsetfillcolor{tcbcol@backtitle}%
  \pgfsetfillopacity{\kvtcb@opacitybacktitle}%
  \pgfusepath{fill}%
  \end{pgfscope}%
}

\def\tcb@drawlower@spartan{%
  \begin{pgfscope}%
  \iftcb@sidebyside%
  \tcbdimto\tcb@seg@pos{\kvtcb@left@rule+\kvtcb@boxsep+\kvtcb@leftupper+\tcb@w@upper+\kvtcb@sbs@gap/2}%
  \pgfpathmoveto{\pgfqpoint{\tcb@seg@pos}{\the\dimexpr\kvtcb@bottom@rule+\tcb@innerheight\relax}}%
  \pgfpathlineto{\pgfqpoint{\tcb@seg@pos}{\kvtcb@bottom@rule}}%
  \else%
  \tcbdimto\tcb@seg@pos{\kvtcb@bottom@rule+\kvtcb@boxsep*2+\tcb@break@bottomsep+\kvtcb@middle+\kvtcb@bottom+\tcb@height@lower}%
  \pgfpathmoveto{\pgfqpoint{\kvtcb@left@rule}{\tcb@seg@pos}}%
  \pgfpathlineto{\pgfqpoint{\the\dimexpr\tcb@width-\kvtcb@right@rule\relax}{\tcb@seg@pos}}%
  \fi%
  \pgfsetcolor{tcbcol@frame}%
  \pgfsetstrokeopacity{\kvtcb@opacityframe}%
  \pgfusepath{stroke}%
  \end{pgfscope}%
}


\tcbset{%
  frame style/.code={\tikzset{frame@style/.style={#1}}},%
  frame hidden/.style={frame style={draw=none,fill=none}},
  frame engine/path/.style={frame code=\tcb@drawframe@path},
  frame engine/pathfirst/.style={frame code=\tcb@drawframe@pathfirst},
  frame engine/pathmiddle/.style={frame code=\tcb@drawframe@pathmiddle},
  frame engine/pathlast/.style={frame code=\tcb@drawframe@pathlast},
  frame engine/freelance/.style={frame code=\tcb@drawframe@standard},
  frame engine/spartan/.style={frame code=\tcb@drawframe@spartan},
  frame engine/empty/.style={frame code=},
  %
  interior titled engine/path/.style={interior titled code=\tcb@drawwithtitle@path},
  interior titled engine/pathfirst/.style={interior titled code=\tcb@drawwithtitle@pathfirst},
  interior titled engine/pathmiddle/.style={interior titled code=\tcb@drawwithtitle@pathmiddle},
  interior titled engine/pathlast/.style={interior titled code=\tcb@drawwithtitle@pathlast},
  interior titled engine/freelance/.style={interior titled code=\tcb@drawwithtitle@standard},
  interior titled engine/spartan/.style={interior titled code=\tcb@drawwithtitle@spartan},
  interior titled engine/empty/.style={interior titled code=},
  %
  interior engine/path/.style={interior code=\tcb@drawwithouttitle@path},
  interior engine/pathfirst/.style={interior code=\tcb@drawwithouttitle@pathfirst},
  interior engine/pathmiddle/.style={interior code=\tcb@drawwithouttitle@pathmiddle},
  interior engine/pathlast/.style={interior code=\tcb@drawwithouttitle@pathlast},
  interior engine/freelance/.style={interior code=\tcb@drawwithouttitle@standard},
  interior engine/spartan/.style={interior code=\tcb@drawwithouttitle@spartan},
  interior engine/empty/.style={interior code=},
  %
  segmentation engine/path/.style={segmentation code=\tcb@drawlower@path},
  segmentation engine/freelance/.style={segmentation code=\tcb@drawlower@standard},
  segmentation engine/spartan/.style={segmentation code=\tcb@drawlower@spartan},
  segmentation engine/empty/.style={segmentation code=},
  %
  title engine/path/.style={@title code=\tcb@drawtitle@path},
  title engine/pathfirst/.style={@title code=\tcb@drawtitle@pathfirst},
  title engine/pathmiddle/.style={@title code=\tcb@drawtitle@pathmiddle},
  title engine/pathlast/.style={@title code=\tcb@drawtitle@pathlast},
  title engine/freelance/.style={@title code=\tcb@drawtitle@standard},
  title engine/spartan/.style={@title code=\tcb@drawtitle@spartan},
  title engine/empty/.style={@title code=},
  %
  interior style/.code={\tikzset{interior@style/.style={#1}}},%
  interior hidden/.style={interior style={draw=none,fill=none}},
  segmentation style/.code={\tikzset{segmentation@style/.style={#1}}},%
  segmentation hidden/.style={segmentation style={draw=none,fill=none}},
  @title style/.code={\tikzset{title@style/.style={#1}}},%
  title style/.style={title filled,@title style={#1}},
  title hidden/.style={title style={draw=none,fill=none}},
  titlerule style/.style={%
    underlay={\iftcb@hasTitle%
      \path[draw,line width=\kvtcb@title@rule+1000sp,#1]
        ([yshift=-\kvtcb@title@rule/2]title.south west)--([yshift=-\kvtcb@title@rule/2]title.south east);
    \fi}},%
  colbacklower/.colorlet=tcbcol@backlower,%
  clear@spec/.code={\tcb@spec{}},%
  tikz/.code={\appto\tcb@tikz@option@hook{,#1}},%
  tikz reset/.code={\let\tcb@tikz@option@hook\@empty},%
  at begin tikz/.code={\appto\tcb@tikz@begin@hook{#1}},%
  at begin tikz reset/.code={\let\tcb@tikz@begin@hook\@empty},%
  at end tikz/.code={\appto\tcb@tikz@end@hook{#1}},%
  at end tikz reset/.code={\let\tcb@tikz@end@hook\@empty},%
  rotate/.style={tikz={rotate=#1,transform shape}},%
  scale/.style={tikz={scale=#1,transform shape},%
    at begin tikz={%
    \tcbdimto\kvtcb@arc{#1\dimexpr\kvtcb@arc}%
    \tcbdimto\tcb@outer@arc{#1\dimexpr\tcb@outer@arc}%
    \def\tcb@shadow@comp@arc{%
      \tcbdimto\tcb@shadow@ts{#1\dimexpr\tcb@shadow@ts}%
      \ifdim\dimexpr\tcb@outer@arc>\tcb@arc@scale\dimexpr\tcb@shadow@ts\relax%
        \tcbdimto\tcb@shadow@arc{\tcb@outer@arc-\tcb@arc@scale\dimexpr\tcb@shadow@ts\relax}%
      \else%
        \let\tcb@shadow@arc=\tcb@zpt%
      \fi%
    }%
    }},%
  remember/.style={tikz={remember picture}},%
  remember as/.style={tikz={remember picture},at end tikz={\pgfnodealias{#1}{frame}}},%
}

\tcbset{%
  base@unbroken/.style={%
    clear@spec,graphical environment=tikzpicture@tcb@hooked,geometry nodes,%
    set@outerboundary=\tcb@boundaryframe@standard,%
    shape@of@skin=unbroken,%
    set@extensions@preframe={\kvtcb@shadow},%
    set@extensions@postframe={\tcb@draw@border@unbroken\tcb@apply@underlay\tcb@apply@overlay},%
    set@extensions@final={\tcb@apply@finish}%
  },%
  base@first/.style={%
    clear@spec,graphical environment=tikzpicture@tcb@hooked,geometry nodes,%
    set@outerboundary=\tcb@boundaryframe@pathfirst,%
    shape@of@skin=first,%
    set@extensions@preframe={\kvtcb@shadow},%
    set@extensions@postframe={\tcb@draw@border@first\tcb@apply@underlay\tcb@apply@overlay},%
    set@extensions@final={\tcb@apply@finish}%
  },%
  base@middle/.style={%
    clear@spec,graphical environment=tikzpicture@tcb@hooked,geometry nodes,%
    set@outerboundary=\tcb@boundaryframe@pathmiddle,%
    shape@of@skin=middle,%
    set@extensions@preframe={\kvtcb@shadow},%
    set@extensions@postframe={\tcb@draw@border@middle\tcb@apply@underlay\tcb@apply@overlay},%
    set@extensions@final={\tcb@apply@finish}%
  },%
  base@last/.style={%
    clear@spec,graphical environment=tikzpicture@tcb@hooked,geometry nodes,%
    set@outerboundary=\tcb@boundaryframe@pathlast,%
    shape@of@skin=last,%
    set@extensions@preframe={\kvtcb@shadow},%
    set@extensions@postframe={\tcb@draw@border@last\tcb@apply@underlay\tcb@apply@overlay},%
    set@extensions@final={\tcb@apply@finish}%
  },%
}

\tcb@new@skin{enhanced}{base@unbroken,%
  frame engine=path,interior titled engine=path,interior engine=path,segmentation engine=path,title engine=path,%
  skin first=enhancedfirst,skin middle=enhancedmiddle,skin last=enhancedlast}

\tcb@new@skin{enhancedfirst}{base@first,%
  frame engine=pathfirst,interior titled engine=pathfirst,interior engine=pathfirst,segmentation engine=path,title engine=pathfirst,%
  skin first=enhancedfirst,skin middle=enhancedmiddle,skin last=enhancedmiddle}

\tcb@new@skin{enhancedmiddle}{base@middle,%
  frame engine=pathmiddle,interior titled engine=pathmiddle,interior engine=pathmiddle,segmentation engine=path,title engine=pathmiddle,%
  skin first=enhancedmiddle,skin middle=enhancedmiddle,skin last=enhancedmiddle}

\tcb@new@skin{enhancedlast}{base@last,%
  frame engine=pathlast,interior titled engine=pathlast,interior engine=pathlast,segmentation engine=path,title engine=pathlast,%
  skin first=enhancedmiddle,skin middle=enhancedmiddle,skin last=enhancedlast}

\tcbset{enhanced/.style={skin=enhanced},%
  enhanced standard/.style={skin=enhanced,
    skin first=enhanced,skin middle=enhanced,skin last=enhanced},%
  blank/.style={enhanced,frame hidden,interior hidden,segmentation hidden,%
    arc=0pt,outer arc=0pt,boxsep=0pt,top=0pt,bottom=0pt,left=0pt,right=0pt,boxrule=0pt,%
    bottomtitle=6pt,middle=3pt}}

\tcb@new@skin{empty}{base@unbroken,%
  frame engine=empty,interior titled engine=empty,interior engine=empty,segmentation engine=empty,title engine=empty,%
  skin first=emptyfirst,skin middle=emptymiddle,skin last=emptylast}

\tcb@new@skin{emptyfirst}{base@first,%
  frame engine=empty,interior titled engine=empty,interior engine=empty,segmentation engine=empty,title engine=empty,%
  skin first=emptyfirst,skin middle=emptymiddle,skin last=emptymiddle}

\tcb@new@skin{emptymiddle}{base@middle,%
  frame engine=empty,interior titled engine=empty,interior engine=empty,segmentation engine=empty,title engine=empty,%
  skin first=emptymiddle,skin middle=emptymiddle,skin last=emptymiddle}

\tcb@new@skin{emptylast}{base@last,%
  frame engine=empty,interior titled engine=empty,interior engine=empty,segmentation engine=empty,title engine=empty,%
  skin first=emptymiddle,skin middle=emptymiddle,skin last=emptylast}

\tcbset{empty/.style={skin=empty},%
  blanker/.style={empty,arc=0pt,outer arc=0pt,boxsep=0pt,top=0pt,bottom=0pt,left=0pt,right=0pt,boxrule=0pt,%
    bottomtitle=6pt,middle=3pt},
  blankest/.style={blanker,notitle,
    no shadow,no underlay,no overlay,no finish,no borderline},
  }

\tcb@new@skin{freelance}{base@unbroken,%
  frame engine=freelance,interior titled engine=freelance,interior engine=freelance,segmentation engine=freelance,title engine=freelance,%
  skin first=freelancefirst,skin middle=freelancemiddle,skin last=freelancelast}%

\tcb@new@skin{freelancefirst}{base@first,%
  frame engine=freelance,interior titled engine=freelance,interior engine=freelance,segmentation engine=freelance,title engine=freelance,%
  skin first=freelancefirst,skin middle=freelancemiddle,skin last=freelancemiddle}%

\tcb@new@skin{freelancemiddle}{base@middle,%
  frame engine=freelance,interior titled engine=freelance,interior engine=freelance,segmentation engine=freelance,title engine=freelance,%
  skin first=freelancemiddle,skin middle=freelancemiddle,skin last=freelancemiddle}%

\tcb@new@skin{freelancelast}{base@last,%
  frame engine=freelance,interior titled engine=freelance,interior engine=freelance,segmentation engine=freelance,title engine=freelance,%
  skin first=freelancemiddle,skin middle=freelancemiddle,skin last=freelancelast}%

\tcbset{freelance/.style={skin=freelance},
  % for backward compatibility:
  extend freelance/.style={#1},%
  extend freelancefirst/.style={skin first is subskin of={freelancefirst}{#1}},%
  extend freelancemiddle/.style={skin middle is subskin of={freelancemiddle}{#1}},%
  extend freelancelast/.style={skin last is subskin of={freelancelast}{#1}}}

\tcb@new@skin{bicolor}{base@unbroken,%
  frame engine=path,interior titled engine=empty,interior engine=empty,segmentation engine=empty,title engine=path,%
  interior titled code={%
    \iftcb@lowerseparated%
      \ifcase\tcb@segment@state%
      {\tcb@spec{fill=tcbcol@back}\tcb@drawwithtitle@path}%
      \or%
      \tcb@spec{fill=tcbcol@back}\tcb@drawspec@UT%
      \else%
      {\tcb@spec{fill=tcbcol@backlower}\tcb@drawwithtitle@path}%
      \fi%
    \else%
      {\tcb@spec{fill=tcbcol@back}\tcb@drawwithtitle@path}%
    \fi\tcb@spec{}},
  interior code={%
    \iftcb@lowerseparated%
      \ifcase\tcb@segment@state%
      {\tcb@spec{fill=tcbcol@back}\tcb@drawwithouttitle@path}%
      \or%
      \tcb@spec{fill=tcbcol@back}\tcb@drawspec@UR%
      \else%
      {\tcb@spec{fill=tcbcol@backlower}\tcb@drawwithouttitle@path}%
      \fi%
    \else%
      {\tcb@spec{fill=tcbcol@back}\tcb@drawwithouttitle@path}%
    \fi\tcb@spec{}},
  segmentation code={\iftcb@sidebyside%
    \iftcb@hasTitle\tcb@drawspec@sbs@B{fill=tcbcol@backlower}\else%
    \tcb@drawspec@sbs@A{fill=tcbcol@backlower}\fi\else\tcb@drawspec@LR{fill=tcbcol@backlower}\fi\tcb@spec{}},%
  skin first=bicolorfirst,skin middle=bicolormiddle,skin last=bicolorlast}

\tcbset{bicolor/.style={skin=bicolor}}

\tcb@new@skin{bicolorfirst}{base@first,%
  frame engine=pathfirst,interior titled engine=empty,interior engine=empty,segmentation engine=empty,title engine=pathfirst,%
  interior titled code={%
    \iftcb@lowerseparated%
      \ifcase\tcb@segment@state%
      {\tcb@spec{fill=tcbcol@back}\tcb@drawwithtitle@pathfirst}%
      \or%
      \tcb@spec{fill=tcbcol@back}\tcb@drawspec@UT%
      \else%
      {\tcbset{interior style=}\tcb@spec{fill=tcbcol@backlower}\tcb@drawwithtitle@pathfirst}%
      \fi%
    \else%
      {\tcb@spec{fill=tcbcol@back}\tcb@drawwithtitle@pathfirst}%
    \fi\tcb@spec{}},
  interior code={%
    \iftcb@lowerseparated%
      \ifcase\tcb@segment@state%
      {\tcb@spec{fill=tcbcol@back}\tcb@drawwithouttitle@pathfirst}%
      \or%
      \tcb@spec{fill=tcbcol@back}\tcb@drawspec@UR%
      \else%
      {\tcbset{interior style=}\tcb@spec{fill=tcbcol@backlower}\tcb@drawwithouttitle@pathfirst}%
      \fi%
    \else%
      {\tcb@spec{fill=tcbcol@back}\tcb@drawwithouttitle@pathfirst}%
    \fi\tcb@spec{}},
  segmentation code={\iftcb@sidebyside%
    \iftcb@hasTitle\tcb@drawspec@sbs@D{fill=tcbcol@backlower}\else%
    \tcb@drawspec@sbs@C{fill=tcbcol@backlower}\fi\else\tcb@drawspec@LS{fill=tcbcol@backlower}\fi\tcb@spec{}},%
  skin first=bicolorfirst,skin middle=bicolormiddle,skin last=bicolormiddle}

\tcb@new@skin{bicolormiddle}{base@middle,%
  frame engine=pathmiddle,interior titled engine=empty,interior engine=empty,segmentation engine=empty,title engine=pathmiddle,%
  interior titled code={%
    \iftcb@lowerseparated%
      \ifcase\tcb@segment@state%
      {\tcb@spec{fill=tcbcol@back}\tcb@drawwithtitle@pathmiddle}%
      \or%
      \tcb@spec{fill=tcbcol@back}\tcb@drawspec@UT%
      \else%
      {\tcbset{interior style=}\tcb@spec{fill=tcbcol@backlower}\tcb@drawwithtitle@pathmiddle}%
      \fi%
    \else%
      {\tcb@spec{fill=tcbcol@back}\tcb@drawwithtitle@pathmiddle}%
    \fi\tcb@spec{}},%
  interior code={%
    \iftcb@lowerseparated%
      \ifcase\tcb@segment@state%
      {\tcb@spec{fill=tcbcol@back}\tcb@drawwithouttitle@pathmiddle}%
      \or%
      \tcb@spec{fill=tcbcol@back}\tcb@drawspec@US%
      \else%
      {\tcbset{interior style=}\tcb@spec{fill=tcbcol@backlower}\tcb@drawwithouttitle@pathmiddle}%
      \fi%
    \else%
      {\tcb@spec{fill=tcbcol@back}\tcb@drawwithouttitle@pathmiddle}%
    \fi\tcb@spec{}},
  segmentation code={\iftcb@sidebyside%
    \iftcb@hasTitle\tcb@drawspec@sbs@D{fill=tcbcol@backlower}\else%
    \tcb@drawspec@sbs@E{fill=tcbcol@backlower}\fi\else\tcb@drawspec@LS{fill=tcbcol@backlower}\fi\tcb@spec{}},%
  skin first=bicolormiddle,skin middle=bicolormiddle,skin last=bicolormiddle}

\tcb@new@skin{bicolorlast}{base@last,%
  frame engine=pathlast,interior titled engine=empty,interior engine=empty,segmentation engine=empty,title engine=pathlast,%
  interior titled code={%
    \iftcb@lowerseparated%
      \ifcase\tcb@segment@state
      {\tcb@spec{fill=tcbcol@back}\tcb@drawwithtitle@pathlast}%
      \or%
      \tcb@spec{fill=tcbcol@back}\tcb@drawspec@UT%
      \else%
      {\tcbset{interior style=}\tcb@spec{fill=tcbcol@backlower}\tcb@drawwithtitle@pathlast}%
      \fi%
    \else%
      {\tcb@spec{fill=tcbcol@back}\tcb@drawwithtitle@pathlast}%
    \fi\tcb@spec{}},
  interior code={%
    \iftcb@lowerseparated%
      \ifcase\tcb@segment@state%
      {\tcb@spec{fill=tcbcol@back}\tcb@drawwithouttitle@pathlast}%
      \or%
      \tcb@spec{fill=tcbcol@back}\tcb@drawspec@US%
      \else
      {\tcbset{interior style=}\tcb@spec{fill=tcbcol@backlower}\tcb@drawwithouttitle@pathlast}%
      \fi%
    \else%
      {\tcb@spec{fill=tcbcol@back}\tcb@drawwithouttitle@pathlast}%
    \fi\tcb@spec{}},%
  segmentation code={\iftcb@sidebyside%
    \iftcb@hasTitle\tcb@drawspec@sbs@B{fill=tcbcol@backlower}\else%
    \tcb@drawspec@sbs@F{fill=tcbcol@backlower}\fi\else\tcb@drawspec@LR{fill=tcbcol@backlower}\fi\tcb@spec{}},%
  skin first=bicolormiddle,skin middle=bicolormiddle,skin last=bicolorlast}

\tcb@new@skin{tile}{skin@bicolor,frame engine=empty,%
  skin first=tilefirst,skin middle=tilemiddle,skin last=tilelast}

\tcbset{tile/.style={skin=tile,boxrule=0pt,sharp corners,title filled,fonttitle=\bfseries}}

\tcb@new@skin{tilefirst}{skin@bicolorfirst,frame engine=empty,%
  skin first=tilefirst,skin middle=tilemiddle,skin last=tilemiddle}

\tcb@new@skin{tilemiddle}{skin@bicolormiddle,frame engine=empty,%
  skin first=tilemiddle,skin middle=tilemiddle,skin last=tilemiddle}

\tcb@new@skin{tilelast}{skin@bicolorlast,frame engine=empty,%
  skin first=tilemiddle,skin middle=tilemiddle,skin last=tilelast}

\tikzset{beamer@color/.style={fill=none,top color=tcbcol@back,bottom color=tcbcol@back!85!black}}

\tcb@new@skin{beamer}{base@unbroken,%
  frame engine=path,interior titled engine=empty,interior engine=empty,segmentation engine=empty,title engine=path,%
  interior titled code={%
    \iftcb@lowerseparated%
      \ifnum\tcb@segment@state=1%
      \tcb@spec{beamer@color}\tcb@drawspec@UT%
      \else%
      {\tcb@spec{beamer@color}\tcb@drawwithtitle@path}%
      \fi%
    \else%
      {\tcb@spec{beamer@color}\tcb@drawwithtitle@path}%
    \fi%
    \tcb@drawspec@T\tcb@spec{}},
  interior code={%
    \iftcb@lowerseparated%
      \ifnum\tcb@segment@state=1
      \tcb@spec{beamer@color}\tcb@drawspec@UR%
      \else%
      {\tcb@spec{beamer@color}\tcb@drawwithouttitle@path}%
      \fi%
    \else%
      {\tcb@spec{beamer@color}\tcb@drawwithouttitle@path}%
    \fi\tcb@spec{}},
  segmentation code={\iftcb@sidebyside\tcb@drawlower@path\else\tcb@drawspec@LR{beamer@color}\fi\tcb@spec{}},%
  skin first=beamerfirst,skin middle=beamermiddle,skin last=beamerlast}

\tcbset{beamer/.style={skin=beamer,boxrule=0mm,titlerule=1mm,toptitle=0.5mm,arc=2mm,fonttitle=\bfseries,drop fuzzy shadow}}

\tcb@new@skin{beamerfirst}{base@first,%
  frame engine=pathfirst,interior titled engine=empty,interior engine=empty,segmentation engine=empty,title engine=pathfirst,%
  interior titled code={%
    \iftcb@lowerseparated%
      \ifnum\tcb@segment@state=1%
      \tcb@spec{beamer@color}\tcb@drawspec@UT%
      \else%
      {\tcb@spec{beamer@color}\tcb@drawwithtitle@pathfirst}%
      \fi%
    \else%
      {\tcb@spec{beamer@color}\tcb@drawwithtitle@pathfirst}%
    \fi%
    \tcb@drawspec@T\tcb@spec{}},%
  interior code={%
    \iftcb@lowerseparated%
      \ifnum\tcb@segment@state=1
      \tcb@spec{beamer@color}\tcb@drawspec@UR%
      \else%
      {\tcb@spec{beamer@color}\tcb@drawwithouttitle@pathfirst}%
      \fi%
    \else%
      {\tcb@spec{beamer@color}\tcb@drawwithouttitle@pathfirst}%
    \fi\tcb@spec{}},
  segmentation code={\iftcb@sidebyside\tcb@drawlower@path\else\tcb@drawspec@LS{beamer@color}\fi\tcb@spec{}},%
  skin first=beamerfirst,skin middle=beamermiddle,skin last=beamermiddle}

\tcb@new@skin{beamermiddle}{base@middle,%
  frame engine=pathmiddle,interior titled engine=empty,interior engine=empty,segmentation engine=empty,title engine=pathmiddle,%
  interior titled code={%
    \iftcb@lowerseparated%
      \ifnum\tcb@segment@state=1%
      \tcb@spec{beamer@color}\tcb@drawspec@UT%
      \else%
      {\tcb@spec{beamer@color}\tcb@drawwithtitle@pathmiddle}%
      \fi%
    \else%
      {\tcb@spec{beamer@color}\tcb@drawwithtitle@pathmiddle}%
    \fi%
    \tcb@drawspec@T\tcb@spec{}},%
  interior code={%
    \iftcb@lowerseparated%
      \ifnum\tcb@segment@state=1
      \tcb@spec{beamer@color}\tcb@drawspec@US%
      \else%
      {\tcb@spec{beamer@color}\tcb@drawwithouttitle@pathmiddle}%
      \fi%
    \else%
      {\tcb@spec{beamer@color}\tcb@drawwithouttitle@pathmiddle}%
    \fi\tcb@spec{}},
  segmentation code={\iftcb@sidebyside\tcb@drawlower@path\else\tcb@drawspec@LS{beamer@color}\fi\tcb@spec{}},%
  skin first=beamermiddle,skin middle=beamermiddle,skin last=beamermiddle}

\tcb@new@skin{beamerlast}{base@last,%
  frame engine=pathlast,interior titled engine=empty,interior engine=empty,segmentation engine=empty,title engine=pathlast,%
  interior titled code={%
    \iftcb@lowerseparated%
      \ifnum\tcb@segment@state=1%
      \tcb@spec{beamer@color}\tcb@drawspec@UT%
      \else%
      {\tcb@spec{beamer@color}\tcb@drawwithtitle@pathlast}%
      \fi%
    \else%
      {\tcb@spec{beamer@color}\tcb@drawwithtitle@pathlast}%
    \fi%
    \tcb@drawspec@T\tcb@spec{}},%
  interior code={%
    \iftcb@lowerseparated%
      \ifnum\tcb@segment@state=1
      \tcb@spec{beamer@color}\tcb@drawspec@US%
      \else%
      {\tcb@spec{beamer@color}\tcb@drawwithouttitle@pathlast}%
      \fi%
    \else%
      {\tcb@spec{beamer@color}\tcb@drawwithouttitle@pathlast}%
    \fi\tcb@spec{}},
  segmentation code={\iftcb@sidebyside\tcb@drawlower@path\else\tcb@drawspec@LR{beamer@color}\fi\tcb@spec{}},%
  skin first=beamermiddle,skin middle=beamermiddle,skin last=beamerlast}

\def\tcb@drawspec@widgetsegment{%
  \iftcb@sidebyside%
  \tcb@drawlower@path%
  \else%
  \path[left color=tcbcol@frame!75!white,right color=tcbcol@frame!75!white!25!tcbcol@back,segmentation@style]
    ([yshift={-\kvtcb@middle/4}]segmentation.west) rectangle ([yshift={\kvtcb@middle/4}]segmentation.east);
  \fi%
}

\tikzset{widget@color/.style={left color=tcbcol@frame!75!white,right color=tcbcol@frame!75!white!25!tcbcol@back}}

\tcb@new@skin{widget}{base@unbroken,%
  frame engine=path,interior titled engine=path,interior engine=path,segmentation engine=empty,title engine=empty,%
  title code={{\tcb@spec{widget@color}\tcb@drawtitle@path}},
  segmentation code={\tcb@drawspec@widgetsegment},%
  skin first=widgetfirst,skin middle=widgetmiddle,skin last=widgetlast}

\tcbset{widget/.style={skin=widget,arc=0.5mm,fonttitle=\bfseries,titlerule=0mm,toprule at break=0mm}}

\tcb@new@skin{widgetfirst}{base@first,%
  frame engine=pathfirst,interior titled engine=pathfirst,interior engine=pathfirst,segmentation engine=empty,title engine=empty,%
  title code={{\tcb@spec{widget@color}\tcb@drawtitle@pathfirst}},%
  segmentation code={\tcb@drawspec@widgetsegment},%
  skin first=widgetfirst,skin middle=widgetmiddle,skin last=widgetmiddle}

\tcb@new@skin{widgetmiddle}{base@middle,%
  frame engine=pathmiddle,interior titled engine=pathmiddle,interior engine=pathmiddle,segmentation engine=empty,title engine=empty,%
  title code={{\tcb@spec{widget@color}\tcb@drawtitle@pathmiddle}},%
  segmentation code={\tcb@drawspec@widgetsegment},%
  skin first=widgetmiddle,skin middle=widgetmiddle,skin last=widgetmiddle}

\tcb@new@skin{widgetlast}{base@last,%
  frame engine=pathlast,interior titled engine=pathlast,interior engine=pathlast,segmentation engine=empty,title engine=empty,%
  title code={{\tcb@spec{widget@color}\tcb@drawtitle@pathlast}},
  segmentation code={\tcb@drawspec@widgetsegment},%
  skin first=widgetmiddle,skin middle=widgetmiddle,skin last=widgetlast}

\tcb@new@skin{spartan}{graphical environment=tikzpicture@tcb@hooked,geometry nodes=true,shape@of@skin=unbroken,%
  set@extensions@preframe=,set@extensions@postframe={\tcb@apply@underlay},set@extensions@final=,%
  frame engine=spartan,interior titled engine=spartan,interior engine=spartan,title engine=spartan,segmentation engine=spartan,%
  set@outerboundary=\tcb@boundaryframe@standard,%
  skin first=spartan,skin middle=spartan,skin last=spartan}

\tcbset{spartan/.style={skin=spartan}}

\tcb@new@skin{draft}{clear@spec,graphical environment=tikzpicture@tcb@hooked,geometry nodes,shape@of@skin=unbroken,%
  frame engine=empty,interior titled engine=empty,interior engine=empty,segmentation engine=path,title empty,%
  segmentation style={draw=black,dashed},
  set@extensions@postframe=,
  set@extensions@final={\tcb@apply@finish},no finish,%
  colupper=black!50!white,collower=black!50!white,coltitle=black!50!white,
  frame code={%
    \path[draw=blue!10!white,double,line width=1pt,dashed] (current bounding box.south west) rectangle (current bounding box.north east);
    {\tcb@spec{fill=black!15!white,draw=black}\tcb@drawframe@path}%
    \iftcb@hasTitle%
      \path[fill=red!10!white,draw,dotted,rounded corners=\kvtcb@arc]
        ([xshift={\kvtcb@left@rule},yshift={\kvtcb@bottom@rule}]frame.south west) rectangle
        (interior.north east);
      \path[fill=red!10!white,draw,dotted,rounded corners=\kvtcb@arc]
        ([yshift={\kvtcb@title@rule}]interior.north west) rectangle
        ([xshift={-\kvtcb@right@rule},yshift={-\kvtcb@top@rule}]frame.north east);
      \path[fill=white,draw,dotted]
        ([xshift={\kvtcb@boxsep},yshift={\kvtcb@boxsep}]title.south west) rectangle
        ([xshift={-\kvtcb@boxsep},yshift={-\kvtcb@boxsep}]title.north east);
      \path[fill=green!20!white,draw=green!75!black,dashed]
        ([xshift={\kvtcb@boxsep+\kvtcb@lefttitle},yshift={\kvtcb@boxsep+\kvtcb@bottomtitle}]title.south west)
         rectangle node[font=\scriptsize] {title: w=\tcb@w@title, h=\tcb@h@title}
        +(\tcb@w@title,\tcb@h@title);
      \path[draw=red,opacity=0.5] (title.south west) rectangle (title.north east);
    \else%
      \path[fill=red!10!white,draw,dotted,rounded corners=\kvtcb@arc]
        ([xshift={\kvtcb@left@rule},yshift={\kvtcb@bottom@rule}]frame.south west) rectangle
        ([xshift={-\kvtcb@right@rule},yshift={-\kvtcb@top@rule}]frame.north east);
    \fi%
    \ifcase\tcb@segment@state
      \path[fill=white,draw,dotted]
        ([xshift={\kvtcb@boxsep},yshift={\kvtcb@boxsep+\tcb@break@bottomsep}]interior.south west) rectangle
        ([xshift={-\kvtcb@boxsep},yshift={-\kvtcb@boxsep-\tcb@break@topsep}]interior.north east);
      \path[fill=green!20!white,draw=green!75!black,dashed]
        ([xshift={\kvtcb@boxsep+\kvtcb@leftupper},yshift={\kvtcb@boxsep+\kvtcb@bottom+\tcb@break@bottomsep}]interior.south west)
        rectangle node[font=\scriptsize] {upper: w=\tcb@w@upper, h=\tcb@height@upper}
        +(\tcb@w@upper,\tcb@height@upper);
      \iftcb@sidebyside%
      \path[fill=green!20!white,draw=green!75!black,dashed]
        ([yshift={\kvtcb@boxsep+\kvtcb@bottom+\tcb@break@bottomsep}]segmentation.south east)
        rectangle node[font=\scriptsize] {lower: w=\tcb@w@lower, h=\tcb@height@upper}
        +(\tcb@w@lower,\tcb@height@upper);
      \fi%
    \or%
      \ifdim\wd\tcb@upperbox=0pt\relax
        \path[fill=white,draw,dotted]
          ([xshift={\kvtcb@boxsep},yshift={\kvtcb@boxsep+\tcb@break@bottomsep}]interior.south west) rectangle
          ([xshift={-\kvtcb@boxsep},yshift={-\kvtcb@boxsep-\tcb@break@topsep}]interior.north east);
      \else
        \path[fill=white,draw,dotted]
          ([xshift={\kvtcb@boxsep},yshift={\kvtcb@boxsep+\tcb@break@bottomsep}]interior.south west) rectangle
          ([xshift={-\kvtcb@boxsep},yshift={-\kvtcb@boxsep}]segmentation.east);
        \path[fill=white,draw,dotted]
           ([xshift={\kvtcb@boxsep},yshift={\kvtcb@boxsep}]segmentation.west)
           rectangle ([xshift={-\kvtcb@boxsep},yshift={-\kvtcb@boxsep-\tcb@break@topsep}]interior.north east);
        \path[fill=green!20!white,draw=green!75!black,dashed]
          ([xshift={\kvtcb@boxsep+\kvtcb@leftupper},yshift={\kvtcb@boxsep}]segmentation.north west)
           rectangle node[font=\scriptsize] {upper: w=\tcb@w@upper, h=\tcb@height@upper}
           +(\tcb@w@upper,\tcb@height@upper);
      \fi%
      \path[fill=green!20!white,draw=green!75!black,dashed]
        ([xshift={\kvtcb@boxsep+\kvtcb@leftlower},yshift={\kvtcb@boxsep+\kvtcb@bottom+\tcb@break@bottomsep}]interior.south west)
        rectangle  node[font=\scriptsize] {lower: w=\tcb@w@lower, h=\tcb@height@lower}
        +(\tcb@w@lower,\tcb@height@lower);
      \path[draw=red,opacity=0.5] (segmentation.south west) rectangle (segmentation.north east);
    \else
      \path[fill=white,draw,dotted]
        ([xshift={\kvtcb@boxsep},yshift={\kvtcb@boxsep+\tcb@break@bottomsep}]interior.south west) rectangle
        ([xshift={-\kvtcb@boxsep},yshift={-\kvtcb@boxsep-\tcb@break@topsep}]interior.north east);
      \path[fill=green!20!white,draw=green!75!black,dashed]
        ([xshift={\kvtcb@boxsep+\kvtcb@leftlower},yshift={\kvtcb@boxsep+\kvtcb@bottom+\tcb@break@bottomsep}]interior.south west)
        rectangle  node[font=\scriptsize] {lower: w=\tcb@w@lower, h=\tcb@height@lower}
        +(\tcb@w@lower,\tcb@height@lower);
    \fi%
    \path[draw=red,opacity=0.5] (interior.south west) rectangle (interior.north east);
    \path[draw=red,opacity=0.5] (frame.south west) rectangle (frame.north east);
    \node[above,font=\scriptsize,red!50!black] at (interior.south) {interior: w=\tcb@innerwidth, h=\tcb@innerheight};
    \node[above,font=\scriptsize,red!50!black] at (frame.north) {frame: w=\the\dimexpr\tcb@width\relax, h=\tcb@height};
    \path[draw=blue!10!white,double,line width=1pt,dashed,opacity=0.3] (current bounding box.south west) rectangle (current bounding box.north east);
    \pgfsetfillopacity{0.3}
  },
  skin first=draft,skin middle=draft,skin last=draft}

\tcbset{draft/.style={skin=draft}}

\tikzset{%
  tcb@forced@clip/.code={\tikz@addmode{\tikz@mode@cliptrue}\let\tikz@options=\pgfutil@empty},%
  tcb@invclip/.style={clip,insert path={{[reset cm]\pgfextra{%
    \pgfpathmoveto{\pgfqpoint{-16383.99999pt}{-16383.99999pt}}%
    \pgfpathlineto{\pgfqpoint{16383.99999pt}{-16383.99999pt}}%
    \pgfpathlineto{\pgfqpoint{16383.99999pt}{16383.99999pt}}%
    \pgfpathlineto{\pgfqpoint{-16383.99999pt}{16383.99999pt}}%
    \pgfpathclose}}}}%
}%

\def\tcb@clip@frame{\tcb@pathboundary{clip}{\tcb@outerboundary}}

\def\tcb@invclip@frame{\tcb@pathboundary{tcb@invclip}{\tcb@outerboundary}}

\def\tcb@clip@interior{%
  \begingroup%
  \tcbset{interior hidden}%
  \tcb@spec{tcb@forced@clip}%
  \def\tcb@spec##1{}%
  \iftcb@hasTitle%
    \tcb@interiortitled@code%
  \else%
    \tcb@interior@code%
  \fi%
  \endgroup%
}

\def\tcb@clip@title{%
  \begingroup%
  \tcbset{title hidden}%
  \tcb@spec{tcb@forced@clip}%
  \def\tcb@spec##1{}%
    \iftcb@hasTitle%
      \tcb@title@code%
    \fi%
  \endgroup%
}

\newenvironment{tcbclipframe}{\begin{scope}\tcb@clip@frame}{\end{scope}}
\newenvironment{tcbinvclipframe}{\begin{scope}\tcb@invclip@frame}{\end{scope}}
\newenvironment{tcbclipinterior}{\begin{scope}\tcb@clip@interior}{\end{scope}}
\newenvironment{tcbcliptitle}{\begin{scope}\tcb@clip@title}{\end{scope}}

\def\tcb@apply@underlay{\csname tcb@underlay@\tcb@split@state\endcsname}%
\def\tcb@apply@finish{\csname tcb@finish@\tcb@split@state\endcsname}%

\tcbset{%
  underlay unbroken/.code={\appto\tcb@underlay@unbroken{#1}},%
  underlay first/.code={\appto\tcb@underlay@first{#1}},%
  underlay middle/.code={\appto\tcb@underlay@middle{#1}},%
  underlay last/.code={\appto\tcb@underlay@last{#1}},%
  underlay boxed title/.code={\appto\tcb@underlay@boxedtitle{#1}},%
  underlay/.style={underlay unbroken={#1},underlay first={#1},underlay middle={#1},underlay last={#1}},%
  underlay broken/.style={underlay first={#1},underlay middle={#1},underlay last={#1}},%
  underlay unbroken and first/.style={underlay unbroken={#1},underlay first={#1}},%
  underlay unbroken and last/.style={underlay unbroken={#1},underlay last={#1}},%
  underlay middle and last/.style={underlay middle={#1},underlay last={#1}},%
  underlay first and middle/.style={underlay first={#1},underlay middle={#1}},%
  no underlay unbroken/.code={\let\tcb@underlay@unbroken\@empty},%
  no underlay first/.code={\let\tcb@underlay@first\@empty},%
  no underlay middle/.code={\let\tcb@underlay@middle\@empty},%
  no underlay last/.code={\let\tcb@underlay@last\@empty},%
  no underlay boxed title/.code={\let\tcb@underlay@boxedtitle\@empty},%
  no underlay/.style={no underlay unbroken,no underlay first,no underlay middle,no underlay last,no underlay boxed title},%
  finish unbroken/.code={\appto\tcb@finish@unbroken{#1}},%
  finish first/.code={\appto\tcb@finish@first{#1}},%
  finish middle/.code={\appto\tcb@finish@middle{#1}},%
  finish last/.code={\appto\tcb@finish@last{#1}},%
  finish/.style={finish unbroken={#1},finish first={#1},finish middle={#1},finish last={#1}},%
  finish broken/.style={finish first={#1},finish middle={#1},finish last={#1}},%
  finish unbroken and first/.style={finish unbroken={#1},finish first={#1}},%
  finish unbroken and last/.style={finish unbroken={#1},finish last={#1}},%
  finish middle and last/.style={finish middle={#1},finish last={#1}},%
  finish first and middle/.style={finish first={#1},finish middle={#1}},%
  no finish unbroken/.code={\let\tcb@finish@unbroken\@empty},%
  no finish first/.code={\let\tcb@finish@first\@empty},%
  no finish middle/.code={\let\tcb@finish@middle\@empty},%
  no finish last/.code={\let\tcb@finish@last\@empty},%
  no finish/.style={no finish unbroken,no finish first,no finish middle,no finish last},%
}

\def\tcb@trans@set@boxedsize@copy@top{%
  \begingroup\edef\x{\endgroup\noexpand\def\noexpand\tcb@trans@boxedsize{%
    leftrule=\kvtcb@left@rule,rightrule=\kvtcb@right@rule,
    toprule=\kvtcb@top@rule@stand,bottomrule=\kvtcb@title@rule,
    boxsep=\kvtcb@boxsep,leftupper=\kvtcb@lefttitle,rightupper=\kvtcb@righttitle,
    top=\kvtcb@toptitle,bottom=\kvtcb@bottomtitle,arc=\kvtcb@arc,
    sharp corners=south,
  }}\x}%
\def\tcb@trans@set@boxedsize@copy@bottom{%
  \begingroup\edef\x{\endgroup\noexpand\def\noexpand\tcb@trans@boxedsize{%
    leftrule=\kvtcb@left@rule,rightrule=\kvtcb@right@rule,
    toprule=\kvtcb@title@rule,bottomrule=\kvtcb@bottom@rule@stand,
    boxsep=\kvtcb@boxsep,leftupper=\kvtcb@lefttitle,rightupper=\kvtcb@righttitle,
    top=\kvtcb@toptitle,bottom=\kvtcb@bottomtitle,arc=\kvtcb@arc,
    sharp corners=north,
  }}\x}%

\tcbset{%
  boxed title size/.is choice,
  boxed title size/standard/.code={\def\tcb@trans@set@boxedsize##1{\let\tcb@trans@boxedsize\@empty}},
  boxed title size/title/.code={\def\tcb@trans@set@boxedsize##1{\def\tcb@trans@boxedsize{size=title}}},
  boxed title size/copy/.code={\def\tcb@trans@set@boxedsize##1{%
    \ifstrequal{##1}{top}{\tcb@trans@set@boxedsize@copy@top}{\tcb@trans@set@boxedsize@copy@bottom}}},
  before@boxed@title/.store in=\kvtcb@before@boxedtitle,%
  after@boxed@title/.store in=\kvtcb@after@boxedtitle,%
  boxed title style/.code={\appto\kvtcb@style@boxedtitle{,#1}},%
  no boxed title style/.code={\let\kvtcb@style@boxedtitle\@empty},%
  %
  varwidth boxed title/.style={before@boxed@title={\tcbdimto\tcb@w@title{#1}\begin{varwidth}{\tcb@w@title}},after@boxed@title={\end{varwidth}}},%
  varwidth boxed title/.default={\kvtcb@width-(\kvtcb@left@rule)-(\kvtcb@right@rule)-(\kvtcb@boxsep)*2-(\kvtcb@lefttitle)-(\kvtcb@righttitle)},
  varwidth boxed title*/.style={varwidth boxed title={\kvtcb@width+#1}},
  varwidth boxed title*/.default={0pt-(\kvtcb@left@rule)-(\kvtcb@right@rule)-(\kvtcb@boxsep)*2-(\kvtcb@lefttitle)-(\kvtcb@righttitle)},
  %
  minipage boxed title/.style={before@boxed@title={\tcbdimto\tcb@w@title{#1}\begin{minipage}{\tcb@w@title}},after@boxed@title={\end{minipage}}},%
  minipage boxed title/.default={\kvtcb@width-(\kvtcb@left@rule)-(\kvtcb@right@rule)-(\kvtcb@boxsep)*2-(\kvtcb@lefttitle)-(\kvtcb@righttitle)},
  minipage boxed title*/.style={minipage boxed title={\kvtcb@width+#1}},
  minipage boxed title*/.default={0pt-(\kvtcb@left@rule)-(\kvtcb@right@rule)-(\kvtcb@boxsep)*2-(\kvtcb@lefttitle)-(\kvtcb@righttitle)},
  %
  tikznode boxed title/.style={before@boxed@title={\centering\tcb@shield@externalize\begin{tikzpicture}\node[align=center,inner sep=0pt,outer sep=0pt,#1]\bgroup},after@boxed@title={\egroup;\end{tikzpicture}}},%
  hbox boxed title/.style={before@boxed@title=,after@boxed@title=},%
  %
  boxtitle/xshift/.dimstore in=\kvtcb@xshift@boxedtitle,%
  boxtitle/yshift/.dimstore in=\kvtcb@yshift@boxedtitle,%
  boxtitle/yshifttext/.dimstore in=\kvtcb@yinnershift@boxedtitle,%
  %
  boxtitle/yshift*@top/.style={yshift*/.code={%
    \tcbdimto\kvtcb@yshift@boxedtitle{##1}%
    \tcbdimto\kvtcb@yinnershift@boxedtitle{\kvtcb@yshift@boxedtitle+\kvtcb@top@rule@stand}%
    \ifdim\dimexpr\kvtcb@yinnershift@boxedtitle>0pt\relax\let\kvtcb@yinnershift@boxedtitle\tcb@zpt\fi%
  }},
  boxtitle/yshift*@bottom/.style={yshift*/.code={%
    \tcbdimto\kvtcb@yshift@boxedtitle{##1}%
    \tcbdimto\kvtcb@yinnershift@boxedtitle{\kvtcb@yshift@boxedtitle-\kvtcb@bottom@rule@stand}%
    \ifdim\dimexpr\kvtcb@yinnershift@boxedtitle<0pt\relax\let\kvtcb@yinnershift@boxedtitle\tcb@zpt\fi%
  }},
  boxtitle/adapt@top/.code={%
    \ifdim\dimexpr\tcboxedtitleheight+\kvtcb@yshift@boxedtitle>0pt\relax
      \tcbdimto\kvtcb@bbtop@stand{\kvtcb@bbtop@stand+\tcboxedtitleheight+\kvtcb@yshift@boxedtitle}%
    \fi%
    \tcbdimto\kvtcb@top{\kvtcb@top-\kvtcb@yinnershift@boxedtitle}%
  },
  boxtitle/adapt@bottom/.code={%
    \ifdim\dimexpr\tcboxedtitleheight-\kvtcb@yshift@boxedtitle>0pt\relax
      \tcbdimto\kvtcb@bbbottom@stand{\kvtcb@bbbottom@stand+\tcboxedtitleheight-\kvtcb@yshift@boxedtitle}%
    \fi%
    \tcbdimto\kvtcb@bottom{\kvtcb@bottom+\kvtcb@yinnershift@boxedtitle}%
  },
  attach@title@boxed/.style n args={5}{%
    detach title,
    code={\def\tcb@specialtitle@hook{%
      \ifx\tcbtitletext\@empty\else%
      \tcb@trans@set@boxedsize{#2}%
      \colorlet{tcbtranscol@frame}{tcbcol@frame}%
      \colorlet{tcbtranscol@back}{tcbcol@backtitle}%
      \let\tcb@trans@skin@current\kvtcb@skin@current%
      \let\tcb@trans@boxedstyle\kvtcb@style@boxedtitle%
      \setbox\tcb@titlebox\color@hbox\bgroup\color{tcbcol@title}\kvtcb@fonttitle\kvtcb@before@boxedtitle\kvtcb@haligntitle\kvtcb@before@title\tcbtitletext\kvtcb@after@title\kvtcb@after@boxedtitle\egroup\color@endbox%
      \setbox\tcb@titlebox\color@hbox\tcbox[skin=\tcb@trans@skin@current,colframe=tcbtranscol@frame,colback=tcbtranscol@back,%
        code={\pgfkeysalsofrom\tcb@trans@boxedsize\pgfkeysalsofrom\tcb@trans@boxedstyle}]{\box\tcb@titlebox}\color@endbox%
      %
      \tcbdimto\tcboxedtitleheight{\ht\tcb@titlebox+\dp\tcb@titlebox}%
      \tcbdimto\tcboxedtitlewidth{\wd\tcb@titlebox}%
      \tcbset{boxtitle/.cd,xshift=0pt,yshift=0pt,yshifttext=0pt,yshift*@#2,#1,adapt@#2}%
      \let\tcb@specialgeonodes@first\relax%
      \let\tcb@specialgeonodes@middle\relax%
      \let\tcb@specialgeonodes@last\relax%
      \def\tcb@specialgeonodes@unbroken{%
        \node[#4,name=title,at={([xshift=\kvtcb@xshift@boxedtitle,yshift=\kvtcb@yshift@boxedtitle]frame.#5)},
                minimum width=\tcboxedtitlewidth,minimum height=\tcboxedtitleheight]{};}%
      \cslet{tcb@specialgeonodes@#3}{\tcb@specialgeonodes@unbroken}%
      \def\tcb@specialgeonodes@hook{\csname tcb@specialgeonodes@\tcb@split@state\endcsname}%
      \preto\tcb@underlay@unbroken{\tcb@underlay@boxedtitle\pgftext[at={\pgfpointanchor{title}{center}}]{\box\tcb@titlebox}}%
      \cspreto{tcb@underlay@#3}{\tcb@underlay@boxedtitle\pgftext[at={\pgfpointanchor{title}{center}}]{\box\tcb@titlebox}}%
      \fi}}%
    },
  attach@title@boxed@top/.style n args={3}{attach@title@boxed={#1}{top}{first}{#2}{#3}},%
  attach@title@boxed@bottom/.style n args={3}{attach@title@boxed={#1}{bottom}{last}{#2}{#3}},%
  %
  attach boxed title to top left/.style={attach@title@boxed@top={#1}{above right}{north west}},
  attach boxed title to top center/.style={attach@title@boxed@top={#1}{above}{north}},
  attach boxed title to top right/.style={attach@title@boxed@top={#1}{above left}{north east}},
  attach boxed title to bottom left/.style={attach@title@boxed@bottom={#1}{below right}{south west}},
  attach boxed title to bottom center/.style={attach@title@boxed@bottom={#1}{below}{south}},
  attach boxed title to bottom right/.style={attach@title@boxed@bottom={#1}{below left}{south east}},
  reduce@vertical@rules/.code={%
    \ifdim\dimexpr\kvtcb@left@rule<\dimexpr\kvtcb@right@rule\relax%
      \tcbdimto\tcb@temp{\kvtcb@left@rule/2}%
    \else%
      \tcbdimto\tcb@temp{\kvtcb@right@rule/2}%
    \fi%
    \tcbset{leftrule/.expanded=\the\dimexpr\kvtcb@left@rule-\tcb@temp\relax,
      rightrule/.expanded=\the\dimexpr\kvtcb@right@rule-\tcb@temp\relax}%
  },
  attach boxed title to bottom/.style={%
    attach boxed title to bottom center={yshift*=\tcboxedtitleheight,#1},
    minipage boxed title,boxed title size=copy,
  },
  attach boxed title to bottom*/.style={%
    attach boxed title to bottom={#1},
    boxed title style={reduce@vertical@rules},
  },
  attach boxed title to top/.style={%
    attach boxed title to top center={yshift*=-\tcboxedtitleheight,#1},
    minipage boxed title,boxed title size=copy,
  },
  attach boxed title to top*/.style={%
    attach boxed title to top={#1},
    boxed title style={reduce@vertical@rules},
  },
  flip title/.style={attach boxed title to bottom,
    boxed title style={reduce@vertical@rules,#1}},
}


\newbox\tcb@waterbox

\def\tcb@setratio#1#2#3{\edef#1{\strip@pt\dimexpr\number\numexpr\number\dimexpr#2\relax*65536/\number\dimexpr#3\relax\relax sp\relax}}

\def\tcb@setratiorobust#1#2#3{\ifdim\dimexpr#3<1pt\tcb@setratio#1{#2}{1pt}\else\tcb@setratio#1{#2}{#3}\fi}

\def\tcb@comp@waterbox@stretch#1#2#3{%
  \tcb@setratiorobust\tcb@scale@x{#1\dimexpr#2}{\wd\tcb@waterbox}%
  \tcb@setratiorobust\tcb@scale@y{#1\dimexpr#3}{\ht\tcb@waterbox+\dp\tcb@waterbox}%
}

\def\tcb@comp@waterbox@zoom#1#2#3{%
  \tcb@comp@waterbox@stretch{#1}{#2}{#3}%
  \ifdim\dimexpr\tcb@scale@x pt\relax<\dimexpr\tcb@scale@y pt\relax\let\tcb@scale@y=\tcb@scale@x\else\let\tcb@scale@x=\tcb@scale@y\fi%
}

\def\tcb@comp@waterbox@overzoom#1#2#3{%
  \tcb@comp@waterbox@stretch{#1}{#2}{#3}%
  \ifdim\dimexpr\tcb@scale@x pt\relax>\dimexpr\tcb@scale@y pt\relax\let\tcb@scale@y=\tcb@scale@x\else\let\tcb@scale@x=\tcb@scale@y\fi%
}

\def\tcb@comp@waterbox@shrink#1#2#3{%
  \tcb@comp@waterbox@zoom{#1}{#2}{#3}%
  \ifdim\dimexpr\tcb@scale@x pt\relax>1pt\relax%
    \edef\tcb@scale@x{1}\edef\tcb@scale@y{1}%
  \fi%
}

\def\tcb@box@scaled@waterbox{\scalebox{\tcb@scale@x}[\tcb@scale@y]{\box\tcb@waterbox}}

\def\tcb@drawspec@watermark@@noclip{%
  \tcb@comp@wm%
  \node[opacity=\kvtcb@watermark@opacity,anchor=center] at (interior) {\tcb@box@scaled@waterbox};%
}

\def\tcb@drawspec@watermark@@clip{%
  \begin{tcbclipinterior}%
  \tcb@drawspec@watermark@@noclip%
  \end{tcbclipinterior}%
}

\def\tcb@drawspec@watermark@tikz#1{%
  \setbox\tcb@waterbox=\color@hbox\pgfinterruptpicture{\pgfsetbaseline{0pt}\begin{tikzpicture}[color=\kvtcb@watermark@color]#1\end{tikzpicture}}\endpgfinterruptpicture\color@endbox%
  \tcb@drawspec@watermark%
}

\def\tcb@drawspec@watermark@graphics#1{%
  \setbox\tcb@waterbox=\color@hbox\pgfinterruptpicture{\includegraphics{#1}}\endpgfinterruptpicture\color@endbox%
  \tcb@drawspec@watermark%
}

\def\tcb@drawspec@watermark@text#1{%
  \tcb@drawspec@watermark@tikz{\node[inner sep=0pt,align=flush center]{#1};}%
}


\tcbset{%
  watermark opacity/.store in=\kvtcb@watermark@opacity,%
  watermark color/.store in=\kvtcb@watermark@color,%
%
  watermark stretch/.code={\def\tcb@comp@wm{\tcb@comp@waterbox@stretch{#1}{\tcb@innerwidth}{\tcb@innerheight}}},%
  watermark zoom/.code={\def\tcb@comp@wm{\tcb@comp@waterbox@zoom{#1}{\tcb@innerwidth}{\tcb@innerheight}}},%
  watermark overzoom/.code={\def\tcb@comp@wm{\tcb@comp@waterbox@overzoom{#1}{\tcb@innerwidth}{\tcb@innerheight}}},%
  watermark shrink/.code={\def\tcb@comp@wm{\tcb@comp@waterbox@shrink{#1}{\tcb@innerwidth}{\tcb@innerheight}}},%
%
  watermark tikz/.style={overlay={\tcb@drawspec@watermark@tikz{#1}}},
  watermark tikz on/.style args={#1 is #2}{overlay #1={\tcb@drawspec@watermark@tikz{#2}}},%
  watermark graphics/.style={overlay={\tcb@drawspec@watermark@graphics{#1}}},
  watermark graphics on/.style args={#1 is #2}{overlay #1={\tcb@drawspec@watermark@graphics{#2}}},
  watermark text/.style={overlay={\tcb@drawspec@watermark@text{#1}}},
  watermark text on/.style args={#1 is #2}{overlay #1={\tcb@drawspec@watermark@text{#2}}},
  no watermark/.style={no overlay},
  clip watermark/.is choice,
  clip watermark/true/.code={\let\tcb@drawspec@watermark=\tcb@drawspec@watermark@@clip},
  clip watermark/false/.code={\let\tcb@drawspec@watermark=\tcb@drawspec@watermark@@noclip},
  clip watermark/.default=true,
  show bounding box/.style={border@line app={%
    \path[preaction={draw,line width=0.1pt,#1},draw,double=white,line width=1pt,dashed,opacity=0.5,#1]
    (current bounding box.south west) rectangle (current bounding box.north east);}},%
  show bounding box/.default={red},%
}

\def\tcb@tdraw@title@clip{%
  \begin{tcbcliptitle}%
  \tcb@tdraw@title@core%
  \end{tcbcliptitle}%
}

\def\tcb@tdraw@upper@clip{%
  \begin{tcbclipinterior}%
  \tcb@tdraw@upper@core%
  \end{tcbclipinterior}%
}

\def\tcb@tdraw@lower@clip{%
  \begin{tcbclipinterior}%
  \tcb@tdraw@lower@core%
  \end{tcbclipinterior}%
}


\def\tcb@process@ppbb{%
  \pgf@process{\pgfpointanchor{path picture bounding box}{south west}}%
  \pgf@xa\pgf@x\pgf@ya\pgf@y%
  \pgf@process{\pgfpointanchor{path picture bounding box}{north east}}%
  \pgf@xb\pgf@x\pgf@yb\pgf@y%
  \pgfsetfillopacity{\tcb@tikz@fill@graphics@opacity}%
  \pgfsetstrokeopacity{\tcb@tikz@fill@graphics@opacity}%
}

\def\tcb@process@ppbb@wh{%
  \tcb@process@ppbb%
  \tcbdimto\tcb@ppbb@width{\pgf@xb-\pgf@xa}%
  \tcbdimto\tcb@ppbb@height{\pgf@yb-\pgf@ya}%
}

\def\tcb@set@waterbox@to@graphics#1{%
  \setbox\tcb@waterbox=\color@hbox\pgfinterruptpicture{\expandafter\includegraphics\expandafter[\tcb@tikz@fill@graphics@options]{#1}}\endpgfinterruptpicture\color@endbox%
}

\def\tcb@set@waterbox@to@picture#1{%
  \setbox\tcb@waterbox=\color@hbox\pgfinterruptpicture{\pgfsetbaseline{0pt}\begin{tikzpicture}#1\end{tikzpicture}}\endpgfinterruptpicture\color@endbox%
}

\tikzset{%
  fill image opacity/.store in=\tcb@tikz@fill@graphics@opacity,%
  fill image opacity=1,%
  fill image scale/.store in=\tcb@tikz@fill@graphics@scale,%
  fill image scale=1,%
  fill image options/.store in=\tcb@tikz@fill@graphics@options,%
  fill image options=,%
  fill plain image/.style={path picture={%
    \node at (path picture bounding box.center) {\expandafter\includegraphics\expandafter[\tcb@tikz@fill@graphics@options]{#1}};
  }},
  fill plain picture/.style={path picture={%
    \tcb@set@waterbox@to@picture{#1}%
    \node at (path picture bounding box.center) {\box\tcb@waterbox};
  }},
  fill stretch image/.style={path picture={%
    \tcb@process@ppbb@wh%
    \node at (path picture bounding box.center) {\expandafter\includegraphics\expandafter[\tcb@tikz@fill@graphics@options,%
      width=\the\dimexpr\tcb@tikz@fill@graphics@scale\dimexpr\tcb@ppbb@width\relax,%
      height=\the\dimexpr\tcb@tikz@fill@graphics@scale\dimexpr\tcb@ppbb@height\relax]{#1}};
  }},
  fill stretch picture/.style={path picture={%
    \tcb@process@ppbb@wh%
    \tcb@set@waterbox@to@picture{#1}%
    \tcb@comp@waterbox@stretch{\tcb@tikz@fill@graphics@scale}{\tcb@ppbb@width}{\tcb@ppbb@height}%
    \node at (path picture bounding box.center) {\tcb@box@scaled@waterbox};%
  }},
  fill@overzoom/.style={path picture={%
    \tcb@process@ppbb@wh%
    #1%
    \tcb@comp@waterbox@overzoom{\tcb@tikz@fill@graphics@scale}{\tcb@ppbb@width}{\tcb@ppbb@height}%
    \node at (path picture bounding box.center) {\tcb@box@scaled@waterbox};%
  }},
  fill overzoom image/.style={fill@overzoom={\tcb@set@waterbox@to@graphics{#1}}},%
  fill overzoom picture/.style={fill@overzoom={\tcb@set@waterbox@to@picture{#1}}},%
  fill@zoom/.style={path picture={%
    \tcb@process@ppbb@wh%
    #1%
    \tcb@comp@waterbox@zoom{\tcb@tikz@fill@graphics@scale}{\tcb@ppbb@width}{\tcb@ppbb@height}%
    \node at (path picture bounding box.center) {\tcb@box@scaled@waterbox};%
  }},
  fill zoom image/.style={fill@zoom={\tcb@set@waterbox@to@graphics{#1}}},%
  fill zoom picture/.style={fill@zoom={\tcb@set@waterbox@to@picture{#1}}},%
  fill@shrink/.style={path picture={%
    \tcb@process@ppbb@wh%
    #1%
    \tcb@comp@waterbox@shrink{\tcb@tikz@fill@graphics@scale}{\tcb@ppbb@width}{\tcb@ppbb@height}%
    \node at (path picture bounding box.center) {\tcb@box@scaled@waterbox};%
  }},
  fill shrink image/.style={fill@shrink={\tcb@set@waterbox@to@graphics{#1}}},%
  fill shrink picture/.style={fill@shrink={\tcb@set@waterbox@to@picture{#1}}},%
  fill@tile/.style={path picture={%
    \tcb@process@ppbb%
    #1%
    \tcbdimto\tcb@ppbb@tilew{\wd\tcb@waterbox}%
    \tcbdimto\tcb@ppbb@tileh{\ht\tcb@waterbox+\dp\tcb@waterbox}%
    \pgf@xc\pgf@xa\pgf@yc\pgf@yb%
    \pgfutil@loop%
      \pgfutil@loop%
        \pgftext[x=\pgf@xc,y=\pgf@yc,left,top]{\copy\tcb@waterbox}%
        \ifdim\pgf@xc<\pgf@xb%
        \advance\pgf@xc\tcb@ppbb@tilew%
      \pgfutil@repeat%
      \ifdim\pgf@yc>\pgf@ya%
      \advance\pgf@yc-\tcb@ppbb@tileh%
      \pgf@xc\pgf@xa%
    \pgfutil@repeat%
  }},%
  fill tile image/.style={fill@tile={\tcb@set@waterbox@to@graphics{#1}}},%
  fill tile picture/.style={fill@tile={\tcb@set@waterbox@to@picture{#1}}},%
  fill tile picture*/.style 2 args={fill@tile={\tcb@set@waterbox@to@picture{#2}%
    \setbox\tcb@waterbox=\color@hbox\scalebox{#1}{\box\tcb@waterbox}\color@endbox}},%
  %
  fill plain image*/.style 2 args={fill image options={#1},fill plain image={#2}},%
  fill stretch image*/.style 2 args={fill image options={#1},fill stretch image={#2}},%
  fill overzoom image*/.style 2 args={fill image options={#1},fill overzoom image={#2}},%
  fill zoom image*/.style 2 args={fill image options={#1},fill zoom image={#2}},%
  fill shrink image*/.style 2 args={fill image options={#1},fill shrink image={#2}},%
  fill tile image*/.style 2 args={fill image options={#1},fill tile image={#2}},%
}

\tcbset{%
  frame style image/.style={frame style={fill=none,fill stretch image={#1}}},
  frame style tile/.style 2 args={frame style={fill=none,fill tile image*={#1}{#2}}},
  interior style image/.style={interior style={fill=none,fill stretch image={#1}}},
  interior style tile/.style 2 args={interior style={fill=none,fill tile image*={#1}{#2}}},
  title style image/.style={title style={fill=none,fill stretch image={#1}}},
  title style tile/.style 2 args={title style={fill=none,fill tile image*={#1}{#2}}},
}

\tcbset{%
  clip title/.is choice,
  clip title/true/.code={\let\tcb@tdraw@title=\tcb@tdraw@title@clip},
  clip title/false/.code={\let\tcb@tdraw@title=\tcb@tdraw@title@core},
  clip title/.default=true,
  clip upper/.is choice,
  clip upper/true/.code={\let\tcb@tdraw@upper=\tcb@tdraw@upper@clip},
  clip upper/false/.code={\let\tcb@tdraw@upper=\tcb@tdraw@upper@core},
  clip upper/.default=true,
  clip lower/.is choice,
  clip lower/true/.code={\let\tcb@tdraw@lower=\tcb@tdraw@lower@clip},
  clip lower/false/.code={\let\tcb@tdraw@lower=\tcb@tdraw@lower@core},
  clip lower/.default=true,
}


\tcbset{marker/.style={%
  skin=enhancedmiddle jigsaw,
  breakable,parbox=false,
  boxrule=0mm,leftrule=5mm,rightrule=5mm,boxsep=0mm,
  left=3mm,right=3mm,top=1mm,bottom=1mm,
  toptitle=1mm,bottomtitle=1mm,fonttitle=\bfseries,
  arc=0mm,outer arc=0mm,
  colback=yellow!10!white,colframe=red,
  watermark color=yellow!75!red!25!white,
  enlarge left by=-8mm,
  enlarge right by=-8mm,
  enlarge top by=0mm,
  enlarge bottom by=0mm,
  width=\the\dimexpr\linewidth+1.6cm\relax,
  frame style={top color=tcbcol@frame,bottom color=tcbcol@frame,middle color=yellow!75!tcbcol@frame},
  title style={left color=tcbcol@frame,right color=tcbcol@frame,middle color=yellow!75!tcbcol@frame},
  watermark tikz={\draw[line width=2mm] circle (1cm) node{\fontfamily{ptm}\fontseries{b}\fontsize{20mm}{20mm}\selectfont!};},
  watermark zoom=0.75,
}}


\def\tcb@arc@bor{\pgfsetcornersarced{\pgfqpoint{\tcb@border@arc}{\tcb@border@arc}}}%

\def\tcb@arc@bor@NW{\csname tcb@arc@bor@NW@\tcb@corner@mode@NW\endcsname}
\def\tcb@arc@bor@NE{\csname tcb@arc@bor@NE@\tcb@corner@mode@NE\endcsname}
\def\tcb@arc@bor@SW{\csname tcb@arc@bor@SW@\tcb@corner@mode@SW\endcsname}
\def\tcb@arc@bor@SE{\csname tcb@arc@bor@SE@\tcb@corner@mode@SE\endcsname}

\let\tcb@arc@bor@NW@sharp\tcb@arc@zpt
\let\tcb@arc@bor@NE@sharp\tcb@arc@zpt
\let\tcb@arc@bor@SW@sharp\tcb@arc@zpt
\let\tcb@arc@bor@SE@sharp\tcb@arc@zpt

\let\tcb@arc@bor@NW@rounded\tcb@arc@bor
\let\tcb@arc@bor@NE@rounded\tcb@arc@bor
\let\tcb@arc@bor@SW@rounded\tcb@arc@bor
\let\tcb@arc@bor@SE@rounded\tcb@arc@bor

\def\tcb@border@prepare#1#2{%
  \tcbdimto\tcb@border@ts{#2+(#1)/2}%
  \ifdim\dimexpr\tcb@outer@arc>\tcb@arc@scale\dimexpr\tcb@border@ts\relax%
    \tcbdimto\tcb@border@arc{\tcb@outer@arc-\tcb@arc@scale\dimexpr\tcb@border@ts\relax}%
  \else%
    \let\tcb@border@arc=\tcb@zpt%
  \fi%
}

\def\tcb@border@unbroken#1#2#3{%
  \tcb@border@prepare{#1}{#2}%
  \tcb@pathbase{draw,line width=#1,#3}{[xshift=\tcb@border@ts,yshift=\tcb@border@ts]frame.south west}%
    {[xshift=-\tcb@border@ts,yshift=-\tcb@border@ts]frame.north east}%
    {\tcb@arc@bor@SW}{\tcb@arc@bor@NW}{\tcb@arc@bor@NE}{\tcb@arc@bor@SE}%
}

\def\tcb@border@first#1#2#3{%
  \tcb@border@prepare{#1}{#2}%
  \tcb@pathboundary{draw,line width=#1,#3}{%
    \tcb@gettikzxy{([xshift=\tcb@border@ts]frame.south west)}{\tcb@xa}{\tcb@ya}%
    \tcb@gettikzxy{([xshift=-\tcb@border@ts,yshift=-\tcb@border@ts]frame.north east)}{\tcb@xb}{\tcb@yb}%
    \pgfpathmoveto{\pgfqpoint{\tcb@xa}{\tcb@ya}}%
    \tcb@arc@bor@NW\pgfpathlineto{\pgfqpoint{\tcb@xa}{\tcb@yb}}%
    \tcb@arc@bor@NE\pgfpathlineto{\pgfqpoint{\tcb@xb}{\tcb@yb}}%
    \tcb@arc@zpt\pgfpathlineto{\pgfqpoint{\tcb@xb}{\tcb@ya}}%
  }%
}

\def\tcb@border@middle#1#2#3{%
  \tcb@border@prepare{#1}{#2}%
  \draw[line width=#1,#3]
    ([xshift=\tcb@border@ts]frame.north west) -- ([xshift=\tcb@border@ts]frame.south west);%
  \draw[line width=#1,#3]
    ([xshift=-\tcb@border@ts]frame.north east) -- ([xshift=-\tcb@border@ts]frame.south east);%
}

\def\tcb@border@last#1#2#3{%
  \tcb@border@prepare{#1}{#2}%
  \tcb@pathboundary{draw,line width=#1,#3}{%
    \tcb@gettikzxy{([xshift=\tcb@border@ts,yshift=\tcb@border@ts]frame.south west)}{\tcb@xa}{\tcb@ya}%
    \tcb@gettikzxy{([xshift=-\tcb@border@ts]frame.north east)}{\tcb@xb}{\tcb@yb}%
    \pgfpathmoveto{\pgfqpoint{\tcb@xa}{\tcb@yb}}%
    \tcb@arc@bor@SW\pgfpathlineto{\pgfqpoint{\tcb@xa}{\tcb@ya}}%
    \tcb@arc@bor@SE\pgfpathlineto{\pgfqpoint{\tcb@xb}{\tcb@ya}}%
    \tcb@arc@zpt\pgfpathlineto{\pgfqpoint{\tcb@xb}{\tcb@yb}}%
  }%
}

\def\tcb@draw@border@unbroken{%
  \let\tcb@border=\tcb@border@unbroken%
  \kvtcb@borderline%
}

\def\tcb@draw@border@first{%
  \let\tcb@border=\tcb@border@first%
  \kvtcb@borderline%
}

\def\tcb@draw@border@middle{%
  \let\tcb@border=\tcb@border@middle%
  \kvtcb@borderline%
}

\def\tcb@draw@border@last{%
  \let\tcb@border=\tcb@border@last%
  \kvtcb@borderline%
}

\def\tcb@bordernorth@draw#1#2#3{%
  \tcbdimto\tcb@border@ts{#2+(#1)/2}%
  \draw[line width=#1,#3] ([yshift=-\tcb@border@ts]frame.north west) -- ([yshift=-\tcb@border@ts]frame.north east);%
}

\def\tcb@bordernorth{%
  \ifdefstring{\tcb@split@state}{unbroken}{\tcb@bordernorth@draw}{%
    \ifdefstring{\tcb@split@state}{first}{\tcb@bordernorth@draw}{}}%
}

\def\tcb@bordersouth@draw#1#2#3{%
  \tcbdimto\tcb@border@ts{#2+(#1)/2}%
  \draw[line width=#1,#3] ([yshift=\tcb@border@ts]frame.south west) -- ([yshift=\tcb@border@ts]frame.south east);%
}

\def\tcb@bordersouth{%
  \ifdefstring{\tcb@split@state}{unbroken}{\tcb@bordersouth@draw}{%
    \ifdefstring{\tcb@split@state}{last}{\tcb@bordersouth@draw}{}}%
}

\def\tcb@borderwest#1#2#3{%
  \tcbdimto\tcb@border@ts{#2+(#1)/2}%
  \draw[line width=#1,#3] ([xshift=\tcb@border@ts]frame.north west) -- ([xshift=\tcb@border@ts]frame.south west);%
}

\def\tcb@bordereast#1#2#3{%
  \tcbdimto\tcb@border@ts{#2+(#1)/2}%
  \draw[line width=#1,#3] ([xshift=-\tcb@border@ts]frame.north east) -- ([xshift=-\tcb@border@ts]frame.south east);%
}

\tcbset{%
  border@line app/.code={\appto\kvtcb@borderline{#1}},%
  borderline/.style args={#1#2#3}{border@line app={\tcb@border{#1}{#2}{#3}}},%
  no borderline/.code={\def\kvtcb@borderline{}},%
  borderline north/.style args={#1#2#3}{border@line app={\tcb@bordernorth{#1}{#2}{#3}}},%
  borderline south/.style args={#1#2#3}{border@line app={\tcb@bordersouth{#1}{#2}{#3}}},%
  borderline west/.style args={#1#2#3}{border@line app={\tcb@borderwest{#1}{#2}{#3}}},%
  borderline east/.style args={#1#2#3}{border@line app={\tcb@bordereast{#1}{#2}{#3}}},%
  borderline horizontal/.style args={#1#2#3}{borderline north={#1}{#2}{#3},borderline south={#1}{#2}{#3}},%
  borderline vertical/.style args={#1#2#3}{borderline west={#1}{#2}{#3},borderline east={#1}{#2}{#3}},%
}


\def\tcb@shadow@comp@ts@smart#1#2{%
  \ifdim#2>0pt\relax\tcbdimto\tcb@shadow@ts{#1-#2/2}%%
  \else\tcbdimto\tcb@shadow@ts{#1+#2/2}\fi%
}

\def\tcb@shadow@comp@ts@copy#1#2{%
  \tcbdimto\tcb@shadow@ts{#1}%
}

\def\tcb@shadow@comp@arc{%
  \ifdim\dimexpr\tcb@outer@arc>\tcb@arc@scale\dimexpr\tcb@shadow@ts\relax%
    \tcbdimto\tcb@shadow@arc{\tcb@outer@arc-\tcb@arc@scale\dimexpr\tcb@shadow@ts\relax}%
  \else%
    \let\tcb@shadow@arc=\tcb@zpt%
  \fi%
}

\def\tcb@arc@sha{\pgfsetcornersarced{\pgfqpoint{\tcb@shadow@arc}{\tcb@shadow@arc}}}%

\def\tcb@arc@sha@NW{\csname tcb@arc@sha@NW@\tcb@corner@mode@NW\endcsname}
\def\tcb@arc@sha@NE{\csname tcb@arc@sha@NE@\tcb@corner@mode@NE\endcsname}
\def\tcb@arc@sha@SW{\csname tcb@arc@sha@SW@\tcb@corner@mode@SW\endcsname}
\def\tcb@arc@sha@SE{\csname tcb@arc@sha@SE@\tcb@corner@mode@SE\endcsname}

\let\tcb@arc@sha@NW@sharp\tcb@arc@zpt
\let\tcb@arc@sha@NE@sharp\tcb@arc@zpt
\let\tcb@arc@sha@SW@sharp\tcb@arc@zpt
\let\tcb@arc@sha@SE@sharp\tcb@arc@zpt

\let\tcb@arc@sha@NW@rounded\tcb@arc@sha
\let\tcb@arc@sha@NE@rounded\tcb@arc@sha
\let\tcb@arc@sha@SW@rounded\tcb@arc@sha
\let\tcb@arc@sha@SE@rounded\tcb@arc@sha

\def\tcb@shadow@unbroken#1#2#3#4{%
  \tcb@shadow@comp@ts{#3}{#1}%
  \tcb@shadow@comp@arc%
  \tcb@pathbase{fill,#4}{[xshift=#1+#3,yshift=#2+#3]frame.south west}{[xshift=#1-#3,yshift=#2-#3]frame.north east}%
    {\tcb@arc@sha@SW}{\tcb@arc@sha@NW}{\tcb@arc@sha@NE}{\tcb@arc@sha@SE}%
}

\def\tcb@shadow@first#1#2#3#4{%
  \tcb@shadow@comp@ts{#3}{#1}%
  \tcb@shadow@comp@arc%
  \tcb@pathbase{fill,#4}{[xshift=#1+#3,yshift=#2+#3]frame.south west}{[xshift=#1-#3,yshift=#2-#3]frame.north east}%
    {\tcb@arc@zpt}{\tcb@arc@sha@NW}{\tcb@arc@sha@NE}{\tcb@arc@zpt}%
}

\def\tcb@shadow@middle#1#2#3#4{%
  \tcb@shadow@comp@ts{#3}{#1}%
  \tcb@shadow@comp@arc%
  \tcb@pathbase{fill,#4}{[xshift=#1+#3,yshift=#2+#3]frame.south west}{[xshift=#1-#3,yshift=#2-#3]frame.north east}%
    {\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}%
}

\def\tcb@shadow@last#1#2#3#4{%
  \tcb@shadow@comp@ts{#3}{#1}%
  \tcb@shadow@comp@arc%
  \tcb@pathbase{fill,#4}{[xshift=#1+#3,yshift=#2+#3]frame.south west}{[xshift=#1-#3,yshift=#2-#3]frame.north east}%
    {\tcb@arc@sha@SW}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@sha@SE}%
}


\tcbset{%
  shad@w app/.code={\appto\kvtcb@shadow{#1}},%
  shadow/.style args={#1#2#3#4}{shad@w app={\csuse{tcb@shadow@\tcb@shapeofskin}{#1}{#2}{#3}{#4}}},%
  no shadow/.code={\def\kvtcb@shadow{}},%
  fuzzy shadow/.style args={#1#2#3#4#5}{shad@w app={%
    \begin{scope}[#5]%
      \letcs\tcb@shadow{tcb@shadow@\tcb@shapeofskin}%
      \tcb@shadow{#1}{#2}{\the\dimexpr#3-4\dimexpr#4\relax}{opacity=0.01}%
      \tcb@shadow{#1}{#2}{\the\dimexpr#3-3\dimexpr#4\relax}{opacity=0.02}%
      \tcb@shadow{#1}{#2}{\the\dimexpr#3-2\dimexpr#4\relax}{opacity=0.04}%
      \tcb@shadow{#1}{#2}{\the\dimexpr#3-#4\relax}{opacity=0.07}%
      \tcb@shadow{#1}{#2}{#3}{opacity=0.11}%
      \tcb@shadow{#1}{#2}{\the\dimexpr#3+#4\relax}{opacity=0.11}%
      \tcb@shadow{#1}{#2}{\the\dimexpr#3+2\dimexpr#4\relax}{opacity=0.07}%
      \tcb@shadow{#1}{#2}{\the\dimexpr#3+3\dimexpr#4\relax}{opacity=0.04}%
      \tcb@shadow{#1}{#2}{\the\dimexpr#3+4\dimexpr#4\relax}{opacity=0.02}%
      \tcb@shadow{#1}{#2}{\the\dimexpr#3+5\dimexpr#4\relax}{opacity=0.01}%
  \end{scope}}},%
  %
  drop shadow/.style={shadow={0.9mm}{-0.9mm}{0mm}{opacity=0.5,#1}},
  drop shadow/.default={black!50!white},%
  drop midday shadow/.style={shadow={0mm}{-0.8mm}{-0.4mm}{opacity=0.5,#1}},
  drop midday shadow/.default={black!50!white},%
  halo/.style args={#1 with #2}{shadow={0mm}{0mm}{-#1}{opacity=0.5,#2}},
  halo/.default={0.9mm with yellow},%
  drop fuzzy shadow/.style={fuzzy shadow={1.0mm}{-1.0mm}{0mm}{0.12mm}{#1}},
  drop fuzzy shadow/.default={black!50!white},%
  drop fuzzy midday shadow/.style={fuzzy shadow={0mm}{-1.0mm}{-0.5mm}{0.12mm}{#1}},
  drop fuzzy midday shadow/.default={black!50!white},%
  fuzzy halo/.style args={#1 with #2}{fuzzy shadow={0mm}{0mm}{-#1}{0.12mm}{#2}},
  fuzzy halo/.default={1.0mm with yellow},%
  %
  drop shadow southeast/.style={shadow={0.9mm}{-0.9mm}{0mm}{opacity=0.5,#1}},%
  drop shadow southeast/.default={black!50!white},%
  drop shadow south/.style={shadow={0mm}{-0.8mm}{-0.4mm}{opacity=0.5,#1}},%
  drop shadow south/.default={black!50!white},%
  drop shadow southwest/.style={shadow={-0.9mm}{-0.9mm}{0mm}{opacity=0.5,#1}},%
  drop shadow southwest/.default={black!50!white},%
  drop shadow west/.style={shadow={-0.8mm}{0mm}{-0.4mm}{opacity=0.5,#1}},%
  drop shadow west/.default={black!50!white},%
  drop shadow northwest/.style={shadow={-0.9mm}{0.9mm}{0mm}{opacity=0.5,#1}},%
  drop shadow northwest/.default={black!50!white},%
  drop shadow north/.style={shadow={0mm}{0.8mm}{-0.4mm}{opacity=0.5,#1}},%
  drop shadow north/.default={black!50!white},%
  drop shadow northeast/.style={shadow={0.9mm}{0.9mm}{0mm}{opacity=0.5,#1}},%
  drop shadow northeast/.default={black!50!white},%
  drop shadow east/.style={shadow={0.8mm}{0mm}{-0.4mm}{opacity=0.5,#1}},%
  drop shadow east/.default={black!50!white},%
  drop fuzzy shadow southeast/.style={fuzzy shadow={1.0mm}{-1.0mm}{0mm}{0.12mm}{#1}},
  drop fuzzy shadow southeast/.default={black!50!white},%
  drop fuzzy shadow south/.style={fuzzy shadow={0mm}{-1.0mm}{-0.5mm}{0.12mm}{#1}},
  drop fuzzy shadow south/.default={black!50!white},%
  drop fuzzy shadow southwest/.style={fuzzy shadow={-1.0mm}{-1.0mm}{0mm}{0.12mm}{#1}},
  drop fuzzy shadow southwest/.default={black!50!white},%
  drop fuzzy shadow west/.style={fuzzy shadow={-1.0mm}{0mm}{-0.5mm}{0.12mm}{#1}},
  drop fuzzy shadow west/.default={black!50!white},%
  drop fuzzy shadow northwest/.style={fuzzy shadow={-1.0mm}{1.0mm}{0mm}{0.12mm}{#1}},
  drop fuzzy shadow northwest/.default={black!50!white},%
  drop fuzzy shadow north/.style={fuzzy shadow={0mm}{1.0mm}{-0.5mm}{0.12mm}{#1}},
  drop fuzzy shadow north/.default={black!50!white},%
  drop fuzzy shadow northeast/.style={fuzzy shadow={1.0mm}{1.0mm}{0mm}{0.12mm}{#1}},
  drop fuzzy shadow northeast/.default={black!50!white},%
  drop fuzzy shadow east/.style={fuzzy shadow={1.0mm}{0mm}{-0.5mm}{0.12mm}{#1}},
  drop fuzzy shadow east/.default={black!50!white},%
  %
  smart shadow arc/.is choice,
  smart shadow arc/true/.code={\let\tcb@shadow@comp@ts=\tcb@shadow@comp@ts@smart},
  smart shadow arc/false/.code={\let\tcb@shadow@comp@ts=\tcb@shadow@comp@ts@copy},
  smart shadow arc/.default=true,
}

\def\tcb@boundary@tikzbendedbase#1#2#3#4#5#6#7#8{%
  \tcb@gettikzxy{(#1)}{\tcb@xa}{\tcb@ya}%
  \tcb@gettikzxy{(#2)}{\tcb@xb}{\tcb@yb}%
  \pgfpathmoveto{\pgfqpoint{\tcb@xa}{\tcb@yb}}%
  #5\pgfpathquadraticcurveto{\pgfqpoint{\dimexpr0.5\dimexpr\tcb@xa+\tcb@xb\relax}{\dimexpr\tcb@yb+#8}}{\pgfqpoint{\tcb@xb}{\tcb@yb}}%
  #6\pgfpathlineto{\pgfqpoint{\tcb@xb}{\tcb@ya}}%
  #3\pgfpathquadraticcurveto{\pgfqpoint{\dimexpr0.5\dimexpr\tcb@xa+\tcb@xb\relax}{\dimexpr\tcb@ya+#7}}{\pgfqpoint{\tcb@xa}{\tcb@ya}}%
  #4\pgfpathclose%
}

\def\tcb@pathbendedbase#1#2#3#4#5#6#7#8#9{\tcb@pathboundary{#1}{\tcb@boundary@tikzbendedbase{#2}{#3}{#4}{#5}{#6}{#7}{#8}{#9}}}

\def\tcb@shadowbended@prepare#1{%
  \tcbdimto\tcb@shadow@arc{\tcb@outer@arc-\tcb@arc@scale\dimexpr#1\relax}%
  \ifdim\dimexpr\tcb@shadow@arc<0pt\relax%
    \let\tcb@shadow@arc=\tcb@zpt%
  \fi%
}

\def\tcb@shadowlifted@unbroken#1#2#3#4#5{%
  \tcb@shadowbended@prepare{#3}%
  \tcb@pathbendedbase{fill,#5}{[xshift=#1+#3,yshift=#2+#3]frame.south west}{[xshift=-#1-#3,yshift=#2-#3]frame.north east}%
    {\tcb@arc@sha@SW}{\tcb@arc@sha@NW}{\tcb@arc@sha@NE}{\tcb@arc@sha@SE}{#4}{0pt}%
}

\def\tcb@shadowlifted@first#1#2#3#4#5{%
  \tcb@shadowbended@prepare{#3}%
  \tcb@pathbendedbase{fill,#5}{[xshift=#1+#3,yshift=#2+#3]frame.south west}{[xshift=-#1-#3,yshift=#2-#3]frame.north east}%
    {\tcb@arc@zpt}{\tcb@arc@sha@NW}{\tcb@arc@sha@NE}{\tcb@arc@zpt}{#4}{0pt}%
}

\def\tcb@shadowlifted@middle#1#2#3#4#5{%
  \tcb@shadowbended@prepare{#3}%
  \tcb@pathbendedbase{fill,#5}{[xshift=#1+#3,yshift=#2+#3]frame.south west}{[xshift=-#1-#3,yshift=#2-#3]frame.north east}%
    {\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}{#4}{0pt}%
}

\def\tcb@shadowlifted@last#1#2#3#4#5{%
  \tcb@shadowbended@prepare{#3}%
  \tcb@pathbendedbase{fill,#5}{[xshift=#1+#3,yshift=#2+#3]frame.south west}{[xshift=-#1-#3,yshift=#2-#3]frame.north east}%
    {\tcb@arc@sha@SW}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@sha@SE}{#4}{0pt}%
}

\tcbset{
  lifted shadow/.style n args={5}{shad@w app={%
    \begin{scope}[#5]%
      \letcs\tcb@shadowlifted{tcb@shadowlifted@\tcb@shapeofskin}%
      \tcb@shadowlifted{#1}{#2}{\dimexpr-4\dimexpr#4}{#3}{opacity=0.01}%
      \tcb@shadowlifted{#1}{#2}{\dimexpr-3\dimexpr#4}{#3}{opacity=0.02}%
      \tcb@shadowlifted{#1}{#2}{\dimexpr-2\dimexpr#4}{#3}{opacity=0.04}%
      \tcb@shadowlifted{#1}{#2}{\dimexpr-#4}{#3}{opacity=0.07}%
      \tcb@shadowlifted{#1}{#2}{0pt}{#3}{opacity=0.11}%
      \tcb@shadowlifted{#1}{#2}{\dimexpr+#4}{#3}{opacity=0.11}%
      \tcb@shadowlifted{#1}{#2}{\dimexpr+2\dimexpr#4}{#3}{opacity=0.07}%
      \tcb@shadowlifted{#1}{#2}{\dimexpr+3\dimexpr#4}{#3}{opacity=0.04}%
      \tcb@shadowlifted{#1}{#2}{\dimexpr+4\dimexpr#4}{#3}{opacity=0.02}%
      \tcb@shadowlifted{#1}{#2}{\dimexpr+5\dimexpr#4}{#3}{opacity=0.01}%
  \end{scope}}},%
  drop small lifted shadow/.style={lifted shadow={1mm}{-0.75mm}{1.3mm}{0.1mm}{#1}},
  drop small lifted shadow/.default={black!50!white},%
  drop lifted shadow/.style={lifted shadow={1.5mm}{-1.5mm}{2.7mm}{0.12mm}{#1}},
  drop lifted shadow/.default={black!50!white},%
  drop large lifted shadow/.style={lifted shadow={2mm}{-3mm}{5.7mm}{0.16mm}{#1}},
  drop large lifted shadow/.default={black!50!white},%
}

\newif\iftcb@isindraft
\def\tcb@draftmode{\tcbset{spartan,spartan@fit}}
\def\tcbstartdraftmode{\let\tcb@afteroptions@hook=\tcb@draftmode\tcb@isindrafttrue}
\def\tcbstopdraftmode{\let\tcb@afteroptions@hook=\@empty\tcb@isindraftfalse}

\def\tcbinterruptdraftmode{%
  \iftcb@isindraft%
    \tcbstopdraftmode%
    \let\tcbcontinuedraftmode=\tcbstartdraftmode%
  \else%
    \let\tcbcontinuedraftmode=\@empty%
  \fi}

\tcbset{%
  draftmode/.is choice,%
  draftmode/.default=true,%
  draftmode/true/.code=\tcbstartdraftmode,%
  draftmode/false/.code=\tcbstopdraftmode,%
}


\def\tcb@include@graphics{%
  \ifdefstring{\kvtcb@capture}{hbox}{%
    \tcbox{%
      \begingroup\edef\x{\endgroup\noexpand\includegraphics[\expandonce\kvtcb@graphics@options]}%
      \x{\imagepath}%
    }%
  }{%
    \iftcb@fixedheight%
      \begin{tcolorbox}%
        \begingroup\edef\x{\endgroup\noexpand\includegraphics[\expandonce\kvtcb@graphics@options,height=\tcbtextheight]}%
        \x{\imagepath}%
      \end{tcolorbox}%
    \else%
      \begin{tcolorbox}%
        \begingroup\edef\x{\endgroup\noexpand\includegraphics[\expandonce\kvtcb@graphics@options,width=\linewidth]}%
        \x{\imagepath}%
      \end{tcolorbox}%
    \fi%
  }%
}

\def\tcb@scanfilename#1#2{%
  \begingroup%
    \everyeof{\noexpand}%
    \endlinechar -1%
    \catcode`\_=11%
    \catcode`\~=11%
    \edef\x{\scantokens\expandafter{#2}}%
  \expandafter\endgroup%
  \expandafter\def\expandafter #1\expandafter{\x}%
}%


\def\tcb@include@graphics@preparefile#1{%
  \tcb@scanfilename\tcb@temp{#1}%
  \filename@parse{\tcb@temp}%
  \ifx\filename@ext\relax%
    \let\imagename\filename@base%
  \else%
    \def\imagename{\filename@base\Gin@sepdefault\filename@ext}%
  \fi%
  \ifdefined\grffile@Ginclude@graphics%
    % grffile package loaded
    \ifx\kvtcb@graphics@directory\@empty%
      \def\imagepath{#1}%
    \else%
      \def\imagepath{\kvtcb@graphics@directory/#1}%
    \fi%
  \else%
    \ifx\kvtcb@graphics@directory\@empty%
      \edef\imagepath{#1}%
    \else%
      \edef\imagepath{\kvtcb@graphics@directory/#1}%
    \fi%
  \fi%
}

\newcommand{\tcbincludegraphics}[2][]{%
  \begingroup%
  \tcb@layer@pushup%
  \tcb@apply@box@options{enhanced,clip upper=true,valign=center,center upper,#1}%
  \tcb@include@graphics@preparefile{#2}%
  \edef\imagepage{1}%
  \tcb@include@graphics%
  \endgroup%
}

\def\tcb@set@pdfpages#1#2{%
  \IfFileExists{#2}{%
    \ifdef{\pdfximage}{%
      \pdfximage{#2}%
      \edef#1{\the\pdflastximagepages}%
    }{%
      \ifdef{\XeTeXpdfpagecount}{%
        \edef#1{\the\XeTeXpdfpagecount #2 }%
        \ifnum#1=0 %
          \edef#1{1}%
        \fi%
      }{\tcb@error{For PDF support run pdflatex, xelatex, or lualatex}{%
        Your compiler seems not to support PDF include files.}}%
    }%
  }{\tcb@error{PDF file `#2' not found}{The PDF file `#2' was not found}}%
  \relax%
}

\newcommand{\tcbincludepdf}[2][]{%
  \begingroup%
  \tcb@layer@pushup%
  \tcb@apply@box@options{enhanced,clip upper=true,valign=center,center upper,#1}%
  \appto\kvtcb@graphics@options{,page=\imagepage}%
  \tcb@include@graphics@preparefile{#2}%
  \tcb@set@pdfpages\pdfpages{\imagepath}%
  \foreach \imagepage in \kvtcb@graphics@pages%
  {%
    \tcb@include@graphics%
  }%
  \endgroup%
}

\tcbset{%
  graphics options/.store in=\kvtcb@graphics@options,
  graphics pages/.store in=\kvtcb@graphics@pages,
  graphics directory/.store in=\kvtcb@graphics@directory,
}


\tcbset{%
  reset@skins/.style={%
    frame style=,interior style=,segmentation style=,@title style=,%
    colbacklower=black!15!white,%
    extend freelance=,extend freelancefirst=,extend freelancemiddle=,extend freelancelast=,%
    clear@spec,%
    watermark opacity=1.00,watermark color=tcbcol@back!85!tcbcol@frame,%
    watermark zoom=0.75,clip watermark,%
    clip title=false,clip upper=false,clip lower=false,%
    no borderline,smart shadow arc,no shadow,no underlay,no finish,tikz reset,at begin tikz reset,at end tikz reset,%
    boxed title size=title,no boxed title style,hbox boxed title,code={\let\tcb@specialgeonodes@hook\relax},%
    graphics options=,graphics pages={1,...,\pdfpages},graphics directory=,%
  },
  initialize@reset=reset@skins,
}

\tcbuselibrary{skins@jigsaw}


==> tcbskinsjigsaw.code.tex <==
%% The LaTeX package tcolorbox - version 3.90 (2016/02/29)
%% tcbskinsjigsaw.code.tex: Code for colorboxes with different skins
%%
%% -------------------------------------------------------------------------------------------
%% Copyright (c) 2006-2016 by Prof. Dr. Dr. Thomas F. Sturm <thomas dot sturm at unibw dot de>
%% -------------------------------------------------------------------------------------------
%%
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either version 1.3
%% of this license or (at your option) any later version.
%% The latest version of this license is in
%%   http://www.latex-project.org/lppl.txt
%% and version 1.3 or later is part of all distributions of LaTeX
%% version 2005/12/01 or later.
%%
%% This work has the LPPL maintenance status `author-maintained'.
%%
%% This work consists of all files listed in README
%%
\tcb@set@library@version{3.90}

\tcbuselibrary{skins}

\def\tcb@drawframe@pathjigsaw{%
  \tcb@pathboundary{tcb fill frame}{\tcb@boundaryframe@standardjigsaw}%
}

\def\tcb@boundary@pathfirstjigsaw@A{%
  \tcbdimto\tcb@xa{\tcb@width-\kvtcb@right@rule}%
  \tcbdimto\tcb@ya{\tcb@height-\kvtcb@top@rule}%
  \pgfpathmoveto{\pgfpointorigin}%
  \tcb@arc@out@NW\pgfpathlineto{\pgfqpoint{0pt}{\tcb@height}}%
  \tcb@arc@out@NE\pgfpathlineto{\pgfqpoint{\tcb@width}{\tcb@height}}%
  \tcb@arc@zpt\pgfpathlineto{\pgfqpoint{\tcb@width}{0pt}}%
  \pgfpathlineto{\pgfqpoint{\tcb@xa}{0pt}}%
  \tcb@arc@ins@NE\pgfpathlineto{\pgfqpoint{\tcb@xa}{\tcb@ya}}%
  \tcb@arc@ins@NW\pgfpathlineto{\pgfqpoint{\kvtcb@left@rule}{\tcb@ya}}%
  \tcb@arc@zpt\pgfpathlineto{\pgfqpoint{\kvtcb@left@rule}{0pt}}%
  \pgfpathclose%
}

\def\tcb@boundary@pathfirstjigsaw@B{%
  \tcbdimto\tcb@xa{\tcb@width-\kvtcb@right@rule}%
  \tcbdimto\tcb@ya{\kvtcb@bottom@rule+\tcb@innerheight}%
  \pgfpathmoveto{\pgfpointorigin}%
  \tcb@arc@out@NW\pgfpathlineto{\pgfqpoint{0pt}{\tcb@height}}%
  \tcb@arc@out@NE\pgfpathlineto{\pgfqpoint{\tcb@width}{\tcb@height}}%
  \tcb@arc@zpt\pgfpathlineto{\pgfqpoint{\tcb@width}{0pt}}%
  \pgfpathlineto{\pgfqpoint{\tcb@xa}{0pt}}%
  \pgfpathlineto{\pgfqpoint{\tcb@xa}{\tcb@ya}}%
  \pgfpathlineto{\pgfqpoint{\kvtcb@left@rule}{\tcb@ya}}%
  \pgfpathlineto{\pgfqpoint{\kvtcb@left@rule}{0pt}}%
  \pgfpathclose%
}

\def\tcb@drawframe@pathfirstjigsaw{%
  \tcb@pathboundary{tcb fill frame}{%
    \pgfseteorule%
    \iftcb@hasTitle%
      \iftcb@titlefilled%
        \ifdim\dimexpr\kvtcb@title@rule>0pt\relax%
          \tcb@boundary@pathfirstjigsaw@B%
          \tcb@boundarytitle@standard%
        \else%
          \tcb@boundary@pathfirstjigsaw@A%
        \fi%
      \else%
        \tcb@boundary@pathfirstjigsaw@B%
      \fi%
    \else%
      \tcb@boundary@pathfirstjigsaw@A%
    \fi%
  }%
}

\def\tcb@boundary@pathmiddlejigsaw@A{%
  \tcbdimto\tcb@xa{\tcb@width-\kvtcb@right@rule}%
  \pgfpathrectangle{\pgfpointorigin}{\pgfqpoint{\kvtcb@left@rule}{\tcb@height}}%
  \pgfpathrectangle{\pgfqpoint{\tcb@xa}{0pt}}{\pgfqpoint{\kvtcb@right@rule}{\tcb@height}}%
}

\def\tcb@boundary@pathmiddlejigsaw@B{%
  \tcbdimto\tcb@xa{\tcb@width-\kvtcb@right@rule}%
  \tcbdimto\tcb@ya{\tcb@height-\kvtcb@top@rule}%
  \pgfpathmoveto{\pgfpointorigin}%
  \tcb@arc@zpt\pgfpathlineto{\pgfqpoint{0pt}{\tcb@height}}%
  \pgfpathlineto{\pgfqpoint{\tcb@width}{\tcb@height}}%
  \pgfpathlineto{\pgfqpoint{\tcb@width}{0pt}}%
  \pgfpathlineto{\pgfqpoint{\tcb@xa}{0pt}}%
  \pgfpathlineto{\pgfqpoint{\tcb@xa}{\tcb@ya}}%
  \pgfpathlineto{\pgfqpoint{\kvtcb@left@rule}{\tcb@ya}}%
  \pgfpathlineto{\pgfqpoint{\kvtcb@left@rule}{0pt}}%
  \pgfpathclose%
}

\def\tcb@boundary@pathmiddlejigsaw@C{%
  \tcbdimto\tcb@xa{\tcb@width-\kvtcb@right@rule}%
  \tcbdimto\tcb@ya{\kvtcb@bottom@rule+\tcb@innerheight}%
  \pgfpathmoveto{\pgfpointorigin}%
  \tcb@arc@zpt\pgfpathlineto{\pgfqpoint{0pt}{\tcb@height}}%
  \pgfpathlineto{\pgfqpoint{\tcb@width}{\tcb@height}}%
  \pgfpathlineto{\pgfqpoint{\tcb@width}{0pt}}%
  \pgfpathlineto{\pgfqpoint{\tcb@xa}{0pt}}%
  \pgfpathlineto{\pgfqpoint{\tcb@xa}{\tcb@ya}}%
  \pgfpathlineto{\pgfqpoint{\kvtcb@left@rule}{\tcb@ya}}%
  \pgfpathlineto{\pgfqpoint{\kvtcb@left@rule}{0pt}}%
  \pgfpathclose%
}

\def\tcb@drawframe@pathmiddlejigsaw{%
  \tcb@pathboundary{tcb fill frame}{%
    \pgfseteorule%
    \iftcb@hasTitle%
      \iftcb@titlefilled%
        \ifdim\dimexpr\kvtcb@title@rule>0pt\relax%
          \tcb@boundary@pathmiddlejigsaw@C%
          \tcb@arc@zpt%
          \tcbdimto\tcb@ya{\kvtcb@bottom@rule+\tcb@innerheight+\kvtcb@title@rule}%
          \tcbdimto\tcb@xb{\tcb@width-\kvtcb@right@rule}%
          \tcbdimto\tcb@yb{\tcb@height-\kvtcb@top@rule}%
          \pgfpathrectanglecorners{\pgfqpoint{\kvtcb@left@rule}{\tcb@ya}}{\pgfqpoint{\tcb@xb}{\tcb@yb}}%
        \else%
          \tcb@boundary@pathmiddlejigsaw@B%
        \fi%
      \else%
        \tcb@boundary@pathmiddlejigsaw@C%
      \fi%
    \else%
      \tcb@boundary@pathmiddlejigsaw@A%
    \fi%
  }%
}

\def\tcb@drawframe@pathlastjigsaw{%
  \tcb@pathboundary{tcb fill frame}{%
    \pgfseteorule%
    \iftcb@hasTitle%
      \iftcb@titlefilled%
        \ifdim\dimexpr\kvtcb@title@rule>0pt\relax%
          \tcb@boundaryframe@pathlast%
          \tcb@arc@zpt%
          \tcbdimto\tcb@ya{\kvtcb@bottom@rule+\tcb@innerheight+\kvtcb@title@rule}%
          \tcbdimto\tcb@xb{\tcb@width-\kvtcb@right@rule}%
          \tcbdimto\tcb@yb{\tcb@height-\kvtcb@top@rule}%
          \pgfpathrectanglecorners{\pgfqpoint{\kvtcb@left@rule}{\tcb@ya}}{\pgfqpoint{\tcb@xb}{\tcb@yb}}%
          \tcb@boundaryinterior@title@standard%
        \else%
          \tcb@boundaryframe@pathlast%
          \tcb@boundary@base{\kvtcb@left@rule}{\kvtcb@bottom@rule}%
            {\tcb@width-\kvtcb@right@rule}{\tcb@height-\kvtcb@top@rule}%
            {\tcb@arc@ins@SW}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@ins@SE}%
        \fi%
      \else%
        \tcb@boundaryframe@pathlast%
      \fi%
    \else%
      \tcbdimto\tcb@xa{\tcb@width-\kvtcb@right@rule}%
      \pgfpathmoveto{\pgfpointorigin}%
      \tcb@arc@zpt\pgfpathlineto{\pgfqpoint{0pt}{\tcb@height}}%
      \pgfpathlineto{\pgfqpoint{\kvtcb@left@rule}{\tcb@height}}%
      \tcb@arc@ins@SW\pgfpathlineto{\pgfqpoint{\kvtcb@left@rule}{\kvtcb@bottom@rule}}%
      \tcb@arc@ins@SE\pgfpathlineto{\pgfqpoint{\tcb@xa}{\kvtcb@bottom@rule}}%
      \tcb@arc@zpt\pgfpathlineto{\pgfqpoint{\tcb@xa}{\tcb@height}}%
      \pgfpathlineto{\pgfqpoint{\tcb@width}{\tcb@height}}%
      \tcb@arc@out@SE\pgfpathlineto{\pgfqpoint{\tcb@width}{0pt}}%
      \tcb@arc@out@SW\pgfpathclose%
    \fi%
  }%
}


\def\tcb@draw@shadowjigsaw@unbroken{%
  \let\tcb@shadow=\tcb@shadow@unbroken%
  \begin{tcbinvclipframe}%
  \kvtcb@shadow%
  \end{tcbinvclipframe}%
}

\def\tcb@draw@shadowjigsaw@first{%
  \let\tcb@shadow=\tcb@shadow@first%
  \begin{tcbinvclipframe}%
  \kvtcb@shadow%
  \end{tcbinvclipframe}%
}

\def\tcb@draw@shadowjigsaw@middle{%
  \let\tcb@shadow=\tcb@shadow@middle%
  \begin{tcbinvclipframe}%
  \kvtcb@shadow%
  \end{tcbinvclipframe}%
}

\def\tcb@draw@shadowjigsaw@last{%
  \let\tcb@shadow=\tcb@shadow@last%
  \begin{tcbinvclipframe}%
  \kvtcb@shadow%
  \end{tcbinvclipframe}%
}

\tcb@new@skin{enhanced jigsaw}{base@unbroken,%
  frame engine=pathjigsaw,interior titled engine=path,interior engine=path,segmentation engine=path,title engine=path,%
  set@extensions@preframe={\tcb@draw@shadowjigsaw@unbroken},%
  skin first=enhancedfirst jigsaw,skin middle=enhancedmiddle jigsaw,skin last=enhancedlast jigsaw}

\tcb@new@skin{enhancedfirst jigsaw}{base@first,%
  frame engine=pathfirstjigsaw,interior titled engine=pathfirst,interior engine=pathfirst,segmentation engine=path,title engine=pathfirst,%
  set@extensions@preframe={\tcb@draw@shadowjigsaw@first},%
  skin first=enhancedfirst jigsaw,skin middle=enhancedmiddle jigsaw,skin last=enhancedmiddle jigsaw}

\tcb@new@skin{enhancedmiddle jigsaw}{base@middle,%
  frame engine=pathmiddlejigsaw,interior titled engine=pathmiddle,interior engine=pathmiddle,segmentation engine=path,title engine=pathmiddle,%
  set@extensions@preframe={\tcb@draw@shadowjigsaw@middle},%
  skin first=enhancedmiddle jigsaw,skin middle=enhancedmiddle jigsaw,skin last=enhancedmiddle jigsaw}

\tcb@new@skin{enhancedlast jigsaw}{base@last,%
  frame engine=pathlastjigsaw,interior titled engine=pathlast,interior engine=pathlast,segmentation engine=path,title engine=pathlast,%
  set@extensions@preframe={\tcb@draw@shadowjigsaw@last},%
  skin first=enhancedmiddle jigsaw,skin middle=enhancedmiddle jigsaw,skin last=enhancedlast jigsaw}

\tcbset{%
  enhanced jigsaw/.style={skin=enhanced jigsaw},%
  frame engine/pathjigsaw/.style={frame code=\tcb@drawframe@pathjigsaw},
  frame engine/pathfirstjigsaw/.style={frame code=\tcb@drawframe@pathfirstjigsaw},
  frame engine/pathmiddlejigsaw/.style={frame code=\tcb@drawframe@pathmiddlejigsaw},
  frame engine/pathlastjigsaw/.style={frame code=\tcb@drawframe@pathlastjigsaw},
}



==> tcbtheorems.code.tex <==
%% The LaTeX package tcolorbox - version 3.90 (2016/02/29)
%% tcbtheorems.code.tex: Code for theorems in colorboxes
%%
%% -------------------------------------------------------------------------------------------
%% Copyright (c) 2006-2016 by Prof. Dr. Dr. Thomas F. Sturm <thomas dot sturm at unibw dot de>
%% -------------------------------------------------------------------------------------------
%%
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either version 1.3
%% of this license or (at your option) any later version.
%% The latest version of this license is in
%%   http://www.latex-project.org/lppl.txt
%% and version 1.3 or later is part of all distributions of LaTeX
%% version 2005/12/01 or later.
%%
%% This work has the LPPL maintenance status `author-maintained'.
%%
%% This work consists of all files listed in README
%%
%\makeatletter
\tcb@set@library@version{3.90}

\RequirePackage{amsmath}

\def\tcb@hack@amsmath{\tcb@hack@currenvir\vskip-\abovedisplayskip}

\def\tcb@theo@form@namenumber#1#2{\hbox{#1~#2}}
\def\tcb@theo@form@numbername#1#2{\hbox{#2~#1}}
\def\tcb@theo@form@name#1#2{\hbox{#1}}

\def\tcb@theo@desc@form@std#1{\tcb@desc@col\kvtcb@desc@font\kvtcb@desc@delim@left#1\kvtcb@desc@delim@right}

\def\tcb@theo@title#1#2#3{%
  \ifdefempty{#2}{\setbox\z@=\color@hbox#1\color@endbox}{\setbox\z@=\tcb@theo@form{#1}{#2}}%
  \def\temp@a{#3}%
  \ifx\temp@a\@empty\relax%
    \unhbox\z@\kvtcb@terminatorsign%
  \else%
    \setbox\z@=\hbox{\unhbox\z@\kvtcb@separatorsign\ }%
    \hangindent\wd\z@%
    \hangafter=1%
    \mbox{\unhbox\z@}{\tcb@theo@desc@form{#3}}\kvtcb@terminatorsign%
  \fi%
}

\def\tcb@theo@listentry#1#2#3{%
  \def\kvtcb@listentry{\protect\numberline{#2}#3}%
}

\def\tcb@theo@label#1#2{%
  \def\temp@a{#2}%
  \ifx\temp@a\@empty%
  \else%
    \tcbset{label={#1:#2}}%
  \fi%
}

\if@fleqn%
\tcbset{%
  ams equation upper/.style={before upper=\tcb@hack@amsmath\equation,after upper=\endequation},%
  ams equation lower/.style={before lower=\tcb@hack@amsmath\equation,after lower=\endequation},%
  ams equation* upper/.style={before upper=\tcb@hack@amsmath\csname equation*\endcsname,after upper=\endequation},%
  ams equation* lower/.style={before lower=\tcb@hack@amsmath\csname equation*\endcsname,after lower=\endequation}%
}%
\else%
\tcbset{%
  ams equation upper/.style={before upper=\tcb@hack@currenvir\equation,after upper=\endequation},%
  ams equation lower/.style={before lower=\tcb@hack@currenvir\equation,after lower=\endequation},%
  ams equation* upper/.style={before upper=\tcb@hack@currenvir\csname equation*\endcsname,after upper=\endequation},%
  ams equation* lower/.style={before lower=\tcb@hack@currenvir\csname equation*\endcsname,after lower=\endequation},%
}%
\fi

\tcbset{
  theorem/.style args={#1#2#3#4}{%
    step and label={#2}{#4},%
    title={\letcs\tcb@temp{the#2}\tcb@theo@title{#1}{\tcb@temp}{#3}}},%
  math upper/.style={before upper=$\displaystyle,after upper=$},%
  math lower/.style={before lower=$\displaystyle,after lower=$},%
  math/.style={math upper,math lower},%
  ams equation/.style={ams equation upper,ams equation lower},%
  ams equation*/.style={ams equation* upper,ams equation* lower},%
  ams align upper/.style={before upper=\tcb@hack@amsmath\align,after upper=\endalign},%
  ams align lower/.style={before lower=\tcb@hack@amsmath\align,after lower=\endalign},%
  ams align/.style={ams align upper,ams align lower},%
  ams align* upper/.style={before upper=\tcb@hack@amsmath\csname align*\endcsname,after upper=\endalign},%
  ams align* lower/.style={before lower=\tcb@hack@amsmath\csname align*\endcsname,after lower=\endalign},%
  ams align*/.style={ams align* upper,ams align* lower},%
  ams gather upper/.style={before upper=\tcb@hack@amsmath\gather,after upper=\endgather},%
  ams gather lower/.style={before lower=\tcb@hack@amsmath\gather,after lower=\endgather},%
  ams gather/.style={ams gather upper,ams gather lower},%
  ams gather* upper/.style={before upper=\tcb@hack@amsmath\csname gather*\endcsname,after upper=\endgather},%
  ams gather* lower/.style={before lower=\tcb@hack@amsmath\csname gather*\endcsname,after lower=\endgather},%
  ams gather*/.style={ams gather* upper,ams gather* lower},%
  ams nodisplayskip upper/.style={before upper=\vskip-\abovedisplayskip},%
  ams nodisplayskip lower/.style={before lower=\vskip-\abovedisplayskip},%
  ams nodisplayskip/.style={ams nodisplayskip upper,ams nodisplayskip lower},%
  highlight math style/.style={highlight math/.style={notitle,nophantom,#1}},%
  separator sign/.store in=\kvtcb@separatorsign,%
  separator sign colon/.style={separator sign={:}},%
  separator sign dash/.style={separator sign={\ --}},%
  separator sign none/.style={separator sign=},%
  terminator sign/.store in=\kvtcb@terminatorsign,%
  terminator sign colon/.style={terminator sign={:}},%
  terminator sign dash/.style={terminator sign={\ --}},%
  terminator sign none/.style={terminator sign=},%
  description delimiters/.code 2 args={\def\kvtcb@desc@delim@left{#1}\def\kvtcb@desc@delim@right{#2}},%
  description delimiters parenthesis/.style={description delimiters=()},
  description delimiters none/.style={description delimiters={}{}},
  description color/.code={\def\temp@a{#1}\ifx\temp@a\@empty\relax%
    \def\tcb@desc@col{}\else\def\tcb@desc@col{\color{#1}}\fi},%
  description color/.default=,
  description font/.store in=\kvtcb@desc@font,
  description font/.default=,
  description formatter/.code={\let\tcb@theo@desc@form=#1},%
  description formatter/.default={\tcb@theo@desc@form@std},%
  theorem name and number/.code={\let\tcb@theo@form=\tcb@theo@form@namenumber},
  theorem number and name/.code={\let\tcb@theo@form=\tcb@theo@form@numbername},
  theorem name/.code={\let\tcb@theo@form=\tcb@theo@form@name},
  theorem style/.is choice,
  theorem style/standard/.style={separator sign colon,description delimiters none,
    terminator sign none,theorem name and number,attach title},
  theorem style/change standard/.style={theorem style=standard,theorem number and name},
  theorem style/plain/.style={separator sign none,description delimiters parenthesis,
    terminator sign colon,theorem name and number,attach title to upper={\ }},
  theorem style/plain apart/.style={separator sign none,description delimiters parenthesis,
    terminator sign none,theorem name and number,attach title},
  theorem style/break/.style={theorem style=plain,attach title to upper={\par}},
  theorem style/change/.style={theorem style=plain,theorem number and name},
  theorem style/change apart/.style={theorem style=plain apart,theorem number and name},
  theorem style/change break/.style={theorem style=break,theorem number and name},
  theorem style/margin/.style={theorem style=plain,theorem name,before title=\makebox[0pt][r]{\thetcbcounter\ }},
  theorem style/margin apart/.style={theorem style=margin,attach title,terminator sign none},
  theorem style/margin break/.style={theorem style=margin,attach title to upper={\par}},
}

\newcommand{\new@tcbtheorem}[5][]{%
  \@@newtcolorbox[auto counter,#1]{#2}[3][]{#4,%
    title={\tcb@theo@title{#3}{\thetcbcounter}{##2}},%
    list entry={\protect\numberline{\thetcbcounter}##2},%
    code={\tcb@theo@label{#5}{##3}},%
    ##1}%
  \@@newtcolorbox[#1,no counter,list inside=]{#2*}[2][]{#4,%
    title={\tcb@theo@title{#3}{\@empty}{##2}},%
    ##1}%
}

\def\newtcbtheorem{\let\@@newtcolorbox\newtcolorbox%
  \new@tcbtheorem}

\def\renewtcbtheorem{\let\@@newtcolorbox\renewtcolorbox%
  \new@tcbtheorem}

\newcommand{\tcbmaketheorem}[5]{%
  \newtcolorbox{#1}[3][]{#3,theorem={#2}{#4}{##2}{#5:##3},##1}%
}

\newtcbox{\tcboxmath}[1][]{nobeforeafter,math upper,tcbox raise base,#1}
\newtcbox{\tcbhighmath}[1][]{highlight math,nobeforeafter,math upper,tcbox raise base,#1}

\tcbset{%
  reset@theorems/.style={%
    description formatter,description color,description font,
    highlight math style={colframe=red,colback=yellow!25!white},%
    theorem style=standard,%
  },
  initialize@reset=reset@theorems,
}



==> tcbxparse.code.tex <==
%% The LaTeX package tcolorbox - version 3.90 (2016/02/29)
%% tcbxparse.code.tex: Code for xparse features
%%
%% -------------------------------------------------------------------------------------------
%% Copyright (c) 2006-2016 by Prof. Dr. Dr. Thomas F. Sturm <thomas dot sturm at unibw dot de>
%% -------------------------------------------------------------------------------------------
%%
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either version 1.3
%% of this license or (at your option) any later version.
%% The latest version of this license is in
%%   http://www.latex-project.org/lppl.txt
%% and version 1.3 or later is part of all distributions of LaTeX
%% version 2005/12/01 or later.
%%
%% This work has the LPPL maintenance status `author-maintained'.
%%
%% This work consists of all files listed in README
%%
%\makeatletter
\tcb@set@library@version{3.90}

\RequirePackage{xparse}[2013/12/31]

\tcbset{%
  IfNoValueTF/.code args={#1#2#3}{\IfNoValueTF{#1}{\pgfkeysalso{#2}}{\pgfkeysalso{#3}}},
  IfValueTF/.code args={#1#2#3}{\IfValueTF{#1}{\pgfkeysalso{#2}}{\pgfkeysalso{#3}}},
  IfBooleanTF/.code args={#1#2#3}{\IfBooleanTF{#1}{\pgfkeysalso{#2}}{\pgfkeysalso{#3}}},
  verbatim/.style={fontupper=\ttfamily,nobeforeafter,tcbox raise base,top=0pt,bottom=0pt,left=1mm,right=1mm,boxrule=0.3mm}
}

%-- tcolorbox --
\long\def\tcb@New@TColorBox#1#2#3{%
  \tcb@newenvironment{#1}{#2}{\tcolorbox[#3,options@for=#1]}{\endtcolorbox}}

\def\DeclareTColorBox{%
  \let\tcb@newenvironment\DeclareDocumentEnvironment%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TColorBox%
  \tcb@process@newenvironment}

\def\NewTColorBox{%
  \let\tcb@newenvironment\NewDocumentEnvironment%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TColorBox%
  \tcb@process@newenvironment}

\def\RenewTColorBox{%
  \let\tcb@newenvironment\RenewDocumentEnvironment%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TColorBox%
  \tcb@process@newenvironment}

\def\ProvideTColorBox{%
  \let\tcb@newenvironment\ProvideDocumentEnvironment%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TColorBox%
  \tcb@process@newenvironment}

%-- tcolorbox (total) --
\long\def\tcb@New@TotalTColorBox#1#2#3#4{%
  \expandafter\tcb@newcommand\csname#1\endcsname{#2}{\begin{tcolorbox}[#3,options@for=#1]#4\end{tcolorbox}}}

\def\DeclareTotalTColorBox{%
  \let\tcb@newcommand\DeclareDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TotalTColorBox%
  \tcb@process@newcommand}

\def\NewTotalTColorBox{%
  \let\tcb@newcommand\NewDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TotalTColorBox%
  \tcb@process@newcommand}

\def\RenewTotalTColorBox{%
  \let\tcb@newcommand\RenewDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TotalTColorBox%
  \tcb@process@newcommand}

\def\ProvideTotalTColorBox{%
  \let\tcb@newcommand\ProvideDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TotalTColorBox%
  \tcb@process@newcommand}

%-- tcbox --
\long\def\tcb@New@TCBox#1#2#3{%
  \expandafter\tcb@newcommand\csname#1\endcsname{#2}{\tcbox[#3,options@for=#1]}}

\def\DeclareTCBox{%
  \let\tcb@newcommand\DeclareDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TCBox%
  \tcb@process@newcommand}

\def\NewTCBox{%
  \let\tcb@newcommand\NewDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TCBox%
  \tcb@process@newcommand}

\def\RenewTCBox{%
  \let\tcb@newcommand\RenewDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TCBox%
  \tcb@process@newcommand}

\def\ProvideTCBox{%
  \let\tcb@newcommand\ProvideDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TCBox%
  \tcb@process@newcommand}

%-- tcbox (total) --
\long\def\tcb@New@TotalTCBox#1#2#3#4{%
  \expandafter\tcb@newcommand\csname#1\endcsname{#2}{\tcbox[#3,options@for=#1]{#4}}}

\def\DeclareTotalTCBox{%
  \let\tcb@newcommand\DeclareDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TotalTCBox%
  \tcb@process@newcommand}

\def\NewTotalTCBox{%
  \let\tcb@newcommand\NewDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TotalTCBox%
  \tcb@process@newcommand}

\def\RenewTotalTCBox{%
  \let\tcb@newcommand\RenewDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TotalTCBox%
  \tcb@process@newcommand}

\def\ProvideTotalTCBox{%
  \let\tcb@newcommand\ProvideDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TotalTCBox%
  \tcb@process@newcommand}

\DeclareTotalTCBox{\tcboxverb}{ O{} v }{verbatim,#1}{#2}

%-- tcboxfit --
\long\def\tcb@New@TCBoxFit#1#2#3{%
  \expandafter\tcb@newcommand\csname#1\endcsname{#2}{\tcboxfit[#3,options@for=#1]}}

\def\DeclareTCBoxFit{%
  \let\tcb@newcommand\DeclareDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TCBoxFit%
  \tcb@process@newcommand}

\def\NewTCBoxFit{%
  \let\tcb@newcommand\NewDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TCBoxFit%
  \tcb@process@newcommand}

\def\RenewTCBoxFit{%
  \let\tcb@newcommand\RenewDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TCBoxFit%
  \tcb@process@newcommand}

\def\ProvideTCBoxFit{%
  \let\tcb@newcommand\ProvideDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TCBoxFit%
  \tcb@process@newcommand}

\long\def\tcb@New@TotalTCBoxFit#1#2#3#4{%
  \expandafter\tcb@newcommand\csname#1\endcsname{#2}{\tcboxfit[#3,options@for=#1]{#4}}}

\def\DeclareTotalTCBoxFit{%
  \let\tcb@newcommand\DeclareDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TotalTCBoxFit%
  \tcb@process@newcommand}

\def\NewTotalTCBoxFit{%
  \let\tcb@newcommand\NewDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TotalTCBoxFit%
  \tcb@process@newcommand}

\def\RenewTotalTCBoxFit{%
  \let\tcb@newcommand\RenewDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TotalTCBoxFit%
  \tcb@process@newcommand}

\def\ProvideTotalTCBoxFit{%
  \let\tcb@newcommand\ProvideDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TotalTCBoxFit%
  \tcb@process@newcommand}


%-- tcblisting --
\long\def\tcb@New@TCBListing#1#2#3{%
  \tcb@newenvironment{#1}{#2}{\tcblisting{#3,options@for=#1}}{\endtcblisting}}

\def\DeclareTCBListing{%
  \let\tcb@newenvironment\DeclareDocumentEnvironment%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TCBListing%
  \tcb@process@newenvironment}

\def\NewTCBListing{%
  \let\tcb@newenvironment\NewDocumentEnvironment%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TCBListing%
  \tcb@process@newenvironment}

\def\RenewTCBListing{%
  \let\tcb@newenvironment\RenewDocumentEnvironment%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TCBListing%
  \tcb@process@newenvironment}

\def\ProvideTCBListing{%
  \let\tcb@newenvironment\ProvideDocumentEnvironment%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TCBListing%
  \tcb@process@newenvironment}

%-- tcbinputlisting --
\long\def\tcb@New@TCBInputListing#1#2#3{%
  \expandafter\tcb@newcommand\csname#1\endcsname{#2}{\tcbinputlisting{#3,options@for=#1}}%
}

\def\DeclareTCBInputListing{%
  \let\tcb@newcommand\DeclareDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TCBInputListing%
  \tcb@process@newcommand}

\def\NewTCBInputListing{%
  \let\tcb@newcommand\NewDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TCBInputListing%
  \tcb@process@newcommand}

\def\RenewTCBInputListing{%
  \let\tcb@newcommand\RenewDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TCBInputListing%
  \tcb@process@newcommand}

\def\ProvideTCBInputListing{%
  \let\tcb@newcommand\ProvideDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TCBInputListing%
  \tcb@process@newcommand}


%-- sidebyside --

\def\tcb@sbs@content@none{\tcb@sbs@text@left\tcblower\tcb@sbs@text@right}
\def\tcb@sbs@content@left{\box\tcb@upperbox\tcblower\tcb@sbs@text@right}
\def\tcb@sbs@content@right{\tcb@sbs@text@left\tcblower\box\tcb@lowerbox}
\def\tcb@sbs@content@both{\box\tcb@upperbox\tcblower\box\tcb@lowerbox}

\tcbset{%
  sidebyside adapt/.is choice,
  sidebyside adapt/none/.style={%
    sidebyside@adapt@process/.style={%
      code={\let\tcb@sbs@content\tcb@sbs@content@none},
    }%
  },
  sidebyside adapt/left/.style={%
    sidebyside@adapt@process/.style={%
      code={\sbox{\tcb@upperbox}{\tcb@sbs@text@left}\let\tcb@sbs@content\tcb@sbs@content@left},
      lefthand width=\wd\tcb@upperbox,
    }%
  },
  sidebyside adapt/right/.style={%
    sidebyside@adapt@process/.style={%
      code={\sbox{\tcb@lowerbox}{\tcb@sbs@text@right}\let\tcb@sbs@content\tcb@sbs@content@right},
      righthand width=\wd\tcb@lowerbox,
    }%
  },
  sidebyside adapt/both/.style={%
    sidebyside@adapt@process/.style={%
      code={\sbox{\tcb@upperbox}{\tcb@sbs@text@left}\sbox{\tcb@lowerbox}{\tcb@sbs@text@right}\let\tcb@sbs@content\tcb@sbs@content@both},
      text width=\wd\tcb@upperbox+\kvtcb@sbs@gap+\wd\tcb@lowerbox,
      lefthand width=\wd\tcb@upperbox,
    }%
  },
  %
  sidebyside switch/.is choice,
  sidebyside switch/true/.style={%
    sidebyside@switch/.code={%
      \tcb@swap{\tcb@sbs@text@left}{\tcb@sbs@text@right}
    }%
  },
  sidebyside switch/false/.style={%
    sidebyside@switch/.style=%
  },
  sidebyside switch/.default=true
}


\DeclareTotalTColorBox{\tcbsidebyside}{ +O{} +m +m }{%
  code={\long\def\tcb@sbs@text@left{#2}\long\def\tcb@sbs@text@right{#3}},%
  #1,%
  sidebyside,%
  sidebyside@switch,sidebyside@adapt@process%
}{\tcb@sbs@content}


\tcbset{%
  reset@xparse/.style={%
    sidebyside adapt=none,sidebyside switch=false,%
  },
  initialize@reset=reset@xparse,
}

